Resilient Federated LQR over Noisy and Lossy Uplinks via Scalar Communication

This paper studies model-free federated learning of a common LQR controller for a fleet of similar systems that communicate with a server over an uplink subject to limited bandwidth, packet dropout, and additive noise. We propose \textsc{ResiFedLQR}, a scalar communication scheme in which each agent sends one real number per packet, with redundancy, instead of full gradient estimates. The scalars can be gradient coordinates, projections of the gradient onto random directions reproduced at the server from a shared seed, or the rollout costs themselves. For the projection encoding, we prove that, with high probability, every iterate stabilizes all agents and the fleet-average cost converges linearly to a neighborhood of the optimum whose radius separates heterogeneity, sampling, and communication effects, and we derive a rule for choosing the number of transmissions from the channel parameters and the fleet size. We then compare the encodings with full-gradient transmission under the same uplink budget and identify the signal-to-noise regime and power constraint under which each is preferable. Numerical experiments on a heterogeneous fleet \reza{of BlueROV2 underwater vehicles} evaluate stability and convergence under varying noise levels and dropout probabilities.

==> Prob_def1.tex <==
\section{Problem Formulation and Objective}\label{sec:prob_def_object}

\begin{figure}[t]
    \centering
        \includegraphics[width=0.9\linewidth]{Fig/FL_LQR2.png}
    \caption{\small
    Federated LQR. (this is just a sketch, Reza can create a better one if we want to include one:)}
    \label{fig:FL_LQR}
\end{figure}
We consider a network of $M$ agents that communicate
through a server in a federated learning paradigm. Each agent is governed
by discrete-time linear time-invariant (LTI) dynamics 
\begin{equation}\label{eq:dynamics}
  x^{(n)}_{t+1} = A^{(n)}x^{(n)}_t + B^{(n)}u^{(n)}_t,
  ~n \in \mathcal{A} := [M]=\{1,\ldots,M\},
\end{equation}
where $x^{(n)}_t\in\mathbb{R}^{n_x}$ and $u^{(n)}_t\in\mathbb{R}^{n_u}$
are the state and~control input of agent~$n$.
The system matrices $(A^{(n)},B^{(n)})$ are unknown and may vary across
agents, while all agents share the same state and input dimensions. The agents objective is to obtain an LQR controller that minimizes
\begin{equation}\label{eq:individual_cost}
  J^{(n)}(K)
  := \mathbb{E}_{\substack{x_0\sim\mathcal{D}_0}}\!\left[\,\sum\nolimits_{t=0}^{\infty}
       x^{(n)\top}_t Q\,x^{(n)}_t
       + u^{(n)\top}_t R\,u^{(n)}_t\right],
\end{equation} where $\mathcal{D}_0$ is the set the initial condition drawn from, and $Q\succeq 0$ and $R\succ 0$ are cost matrices shared across agents.

There agents have
distinct but closely related dynamics, preforming under the following assumption.
\begin{assumption}[Similarity of dynamics]\label{ass:similarity}
There exists a nominal model $(A,B)$ such that, for all $n\in\mathcal{A}$,
\begin{equation}\label{eq:system_bound}
  \|A^{(n)}-A\|_2 \le \epsilon_1,\qquad
  \|B^{(n)}-B\|_2 \le \epsilon_2,
\end{equation}
for some heterogeneity parameters $\epsilon_1,\epsilon_2\ge 0$. \hfill$\square$
\end{assumption}
This similarity and common objective matrices $Q$ and $R$ in~\eqref{eq:individual_cost} make it meaningful to learn in cooperation with each other. This objective is pursued by learning a  single common policy. Thus, each agent applies the static state-feedback law
$u^{(n)}_t = -Kx^{(n)}_t$, where $K\in\mathbb{R}^{n_u\times n_x}$ is
a common gain learned cooperatively, translating to the 
The objective, which is to find a single gain $K$ minimizing the
fleet-average cost
\begin{equation}\label{eq:avg_cost}
  J_{\mathrm{avg}}(K) := \frac{1}{M}\sum\nolimits_{n=1}^{M} J^{(n)}(K).
\end{equation}

Unlike classical distributed control, where each agent learns its own
controller, we seek one common policy across the fleet. Such a policy
need not be individually optimal for every agent, but it provides a robust
shared baseline that can be learned efficiently through data aggregation
and locally fine-tuned if needed. The central challenge is
\emph{stability}: a gain that stabilizes one agent may destabilize another.
We therefore define the per-agent stabilizing set
\[
  \mathcal{S}^{(n)} := \bigl\{K : A^{(n)}-B^{(n)}K
                        \text{ is Schur stable}\bigr\},
\]
and let $\mathcal{S} := \bigcap_{n=1}^{M}\mathcal{S}^{(n)}$ denote the
set of gains that stabilize all agents simultaneously.

\begin{assumption}[Initial stabilizing policy]\label{ass:init}
There exists $K_0\in\mathcal{S}$ that stabilizes all agents
simultaneously. \hfill$\square$
\end{assumption}

This assumption is standard in policy optimization (see e.g.~[XXX])\margin{please add ref} and
can be satisfied via a conservative model-based baseline, an offline
design, or a simple stabilizing controller $K_0=0$ when the systems are open-loop
stable. Fully online stabilization is beyond the scope of this work.

The nominal federated LQR problem is
\begin{equation}\label{eq:fedlqr}
  \min_{K\in\mathcal{S}}\; J_{\mathrm{avg}}(K),
\end{equation}
\margin{we should mention stat dynamics}
where data exchange and coordination are facilitated by the server.
Starting from a common $K_0\in\mathcal{S}$, the server orchestrates
the entire learning process across the fleet of $M$ agents. At each
round $t$, the server broadcasts the current shared policy
$K_t \in \mathbb{R}^{n_u \times n_x}$ to all agents. Each agent $n$
independently executes local trajectory rollouts under a perturbed
version of $K_t$ and uses the resulting cost observations to form a
local zeroth-order gradient estimate $\tilde{g}_{t,n} \in \mathbb{R}^{d}$,
where $d = n_u n_x$ is the policy dimension after vectorizing $K_t$.
These local estimates are then communicated to the server over the
uplink channel. The server aggregates the received gradient information
across the active agents, computes a global descent direction
$\widehat{g}_t$, and performs a zeroth-order policy update
\begin{equation}\label{eq:policy_update}
  K_{t+1} = K_t - \eta\,\widehat{g}_t,
\end{equation}
where $\eta > 0$ is the stepsize. The updated policy $K_{t+1}$
is then broadcast back to all agents for the next round. 


In the setting we consider, the two communication directions are
fundamentally asymmetric. The downlink (the server broadcasting
$K_{t+1}$) is assumed reliable and is not a communication bottleneck.
The uplink, however, is constrained by limited transmission power,
bandwidth, and hardware capabilities of the agents. Consequently,
uplink transmissions are affected by packet loss and additive channel
noise. The impact of these impairments depends strongly on the message
dimension. When a full gradient $\tilde{g}_{t,n}\in\mathbb{R}^{d}$ is
transmitted, channel noise perturbs all $d$ coordinates and a dropped
packet removes an entire gradient estimate. This motivates the
communication strategy developed in this paper, which replaces
high-dimensional gradient transmissions with low-dimensional scalar
information. The stochastic channel model used throughout the paper
is stated next.

\begin{assumption}[Uplink channel noise and dropout]\label{assump:noise}
Each attempted uplink transmission is independently delivered with
probability $1-p_{\rm drop}$ and dropped with probability
$p_{\rm drop}\in[0,1)$. Let $\mathcal{R}_{t,n}(N)$ denote the set of
successfully received packets among $N$ transmission attempts.
Conditional on delivery, the received message satisfies
\[
  y = m + w,
\]
where the channel noise $w$ has zero mean and bounded second moment,
$$
  \mathbb{E}[w]=0,\qquad\mathbb{E}[w^2]\le\sigma_{\rm ch}^2.$$
For vector-valued messages, the same conditions hold componentwise.
Channel noises are independent across agents, transmissions,
coordinates, and rounds, and are independent of the dropout process
and the zeroth-order estimation randomness. \hfill$\square$
\end{assumption}

In this work, we solve~\eqref{eq:fedlqr} under the uplink model above.
The design is complicated by a fundamental stability challenge: ensuring
that each updated policy $K_{t+1}$ remains in the common stabilizing
set~$\mathcal{S}$ throughout learning, so that no agent is destabilized
during the optimization process.

\begin{comment}
In the setting we consider, the two communication directions
are fundamentally asymmetric. The \emph{downlink} (
the server broadcasting $K_{t+1}$ to all agents) is not
assumed to be a bottleneck: servers are typically
well-resourced infrastructure nodes with reliable, high-bandwidth
links, and transmitting a single $n_u\times n_x$ matrix
to the fleet is a low-overhead operation. The \emph{uplink},
by contrast, is the critical constraint. Agents are physical
dynamical systems (drones, ground vehicles, robotic
manipulators, or grid-connected actuators) deployed with
limited onboard battery, low-cost radio hardware, and
restricted transmission power. Their uplink channels are
consequently subject to bandwidth limitations, additive
channel noise, and packet dropout. Moreover, each local
gradient estimate $\tilde{g}_{t,n}$ is an $O(n_x n_u)$-dimensional
object: transmitting it faithfully is expensive, and a single
dropped packet destroys $O(d)$ bits of gradient information.
It is therefore the uplink, not the downlink, that
constitutes the communication bottleneck and the central
design challenge of this work. We model the channel impairments as follows.

\medskip
\noindent\textit{Channel noise model.}
Each delivered message $m_{n,s}^t$ is received at the server
as
\begin{equation}\label{eq:general_channel_model}
  y_{n,s}^t = m_{n,s}^t + w_{n,s}^t,
  \qquad s\in\mathcal{R}_{t,n}(N),
\end{equation}
where $w_{n,s}^t$ is additive uplink channel noise. When
the transmitted message is a $d$-dimensional vector,
$m_{n,s}^t\in\mathbb{R}^d$ and independent componentwise noise $w_{n,s}^t\in \mathbb{R}^d$ corrupts all $d$
components simultaneously, deflecting the entire received
direction. When the message is a scalar,
$m_{n,s}^t\in\mathbb{R}$ and a single real number is
corrupted. %In either case the server averages received copies to suppress the noise contribution.

\medskip
\noindent\textit{Dropout model.}
Uplink transmissions are subject to packet dropout:
each transmission is treated as an atomic packet and,
regardless of its payload size, is either delivered
in full or lost entirely. Formally, each packet is
independently delivered with probability $1-p_{\rm drop}$
and dropped with probability $p_{\rm drop}\in[0,1)$.
For $N$ attempted transmissions from client~$n$ at
round~$t$, let $\mathcal{R}_{t,n}(N)\subseteq\{1,\ldots,N\}$
denote the random index set of received packets, so that
$\mathbb{E}|\mathcal{R}_{t,n}(N)|=(1-p_{\rm drop})N$.
A client is excluded from the server's aggregation at
round~$t$ when all of its packets are lost.
A single common dropout probability is used across all
agents and rounds for simplicity; agent- or time-dependent
models can be accommodated by replacing $N$ with the
appropriate effective received count.

\begin{assumption}[Uplink channel noise and
dropout]\label{assump:noise}
Each attempted uplink transmission is independently
delivered with probability $1-p_{\rm drop}$ and dropped
with probability $p_{\rm drop}$. Conditional on delivery,
each channel noise entry $w$ satisfies
\begin{equation}
  \mathbb{E}[w]=0,\qquad\mathbb{E}[w^2]\le\sigma_{\rm ch}^2.
\end{equation}
For vector-valued messages, the same model holds
componentwise. Channel noises are independent across
agents, transmissions, coordinates, and rounds, and are
independent of the dropout process and the zeroth-order
estimation randomness. \hfill$\square$
\end{assumption}
\end{comment}

==> into_origional.tex <==
\section{Introduction}
\label{sec:introduction}
In recent years, federated learning (FL) has emerged as a powerful paradigm for large-scale collaborative learning across distributed agents \cite{mcmahan_communication-efficient_2017,konevcny_federated_2016}. 
By enabling multiple agents to learn a shared model without transmitting raw local data, FL provides a principled framework for scalable learning under communication, privacy, and data locality constraints. 
This paradigm has naturally extended to the reinforcement learning setting, giving rise to federated reinforcement learning (FRL), where multiple agents interacting with similar environments collaboratively learn shared value functions or policies \cite{wang_federated_2023,lim_federated_2020,yu_federated_2020}. 
Such collaborative learning frameworks have demonstrated strong empirical gains in sample efficiency and generalization in applications including autonomous driving, robotics, IoT systems, and large-scale cyber-physical infrastructures.

At the same time, there has been growing interest in applying learning-based methods to classical control problems, where safety, stability, and reliability are fundamental requirements. 
In particular, the Linear Quadratic Regulator (LQR) problem has emerged as a canonical benchmark for data-driven control, providing a structured setting in which learning-based policy optimization methods can be rigorously analyzed.


Policy optimization (PO) has proved to be a promising approach for data-driven optimal control in various settings \cite{hu_toward_2023,talebi_policy_2026}. Despite the lack of convexity in simple control settings, policy gradient (PG) methods have been shown to be globally convergent for structured settings such as the Linear Quadratic Regulator (LQR) problem. However, deploying these methods on physical hardware is currently intractable due to three converging bottlenecks \cite{}:
\begin{enumerate}
    \item \textbf{Communication Overload:} Transmitting high-dimensional gradients or weight matrices is not feasible under the tight bandwidth constraints of distributed autonomous swarms.
    \item \textbf{Privacy Leakage:} Gradients shared in federated settings can be inverted to reveal sensitive local system data.
    \item \textbf{Sample Inefficiency:} Model-free reinforcement learning typically requires millions of interactions, which is incompatible with the limited lifespan and safety requirements of physical systems.
\end{enumerate}


To address these challenges, Alemzadeh et al. (2024) proposes \texttt{D2SPI}, a data-driven geometric policy iteration that utilizes the algebraic structures of interactions to learn an optimal policy for all homogeneous agents in the network \cite{alemzadeh_data-driven_2024}. It utilizes temporary “auxiliary” communication links on a (much smaller) subnetwork during the “learning phase” to handle the coupling in the costs—links that will be removed subsequently for the final distributed feedback synthesis. 
%
In absence of coupling in the costs, Wang et al. (2023) introduced \texttt{FedLQR}, a framework where $M$ agents with unknown, distinct yet similar dynamics collaboratively learn an optimal policy \cite{wang_model-free_2023}. While \texttt{FedLQR} provides a rigorous foundation for stability and sample complexity reduction, it still relies on sharing full matrix updates. 




In this work, we propose \texttt{ScalarFedLQR}, which fundamentally rethinks the trade-off between communication and performance. 
By utilizing projection masking and scalar streams, we realize the vision of large-scale distributed autonomy while simultaneously solving for efficiency and privacy. 
Instead of transmitting the full policy gain $K$ or the gradient of the cost $\nabla J(K)$ which incurs an $\mathcal{O}(d)$ communication cost per agent per round, each client first computes a local zeroth-order (ZO) gradient estimate $\hat{\nabla} J(K)$ and samples a random vector $v$ locally, then uploads only the single scalar inner product $\langle v, \hat{\nabla} J(K)\rangle$. 
This reduces uplink communication from $\mathcal{O}(d)$ to $\mathcal{O}(1)$, independent of the system dimension.

Beyond communication efficiency, this projection-based mechanism provides intrinsic structural privacy. 
Since the server observes only a rank-one projection of the ZO gradient estimator, all components lying in the null space of $vv^\top$ remain completely unobservable, effectively masking the gradient geometry and preventing direct reconstruction of local system information. 
This null-space masking effect provides a principled form of privacy preservation, analogous to the scalar-communication mechanisms in recent federated learning frameworks that enable learning using only scalar-valued information exchange rather than dimension-dependent variables \cite{rostami_fedscalar_2024}.







==> intro1.tex <==
Here is the full rewritten introduction as a LaTeX section ready to paste into Overleaf:

```latex
\section{Introduction}

The deployment of policy gradient methods for model-free optimal control of physical dynamical systems faces a bottleneck that is often underappreciated in theoretical treatments but is decisive in real-world operation: the physical cost of a single gradient sample. In the zeroth-order (ZO) optimization framework that underlies model-free LQR \cite{fazel_global_2018, malik_derivative-free_2019}, estimating the gradient of the LQR cost $C(K)$ with respect to the policy gain $K$ requires physically executing a perturbed policy $\widehat{K}_s = K + U_s$ on the dynamical system, recording the resulting state trajectory $x_0, x_1, \ldots, x_\tau$, computing the finite-horizon accumulated cost $\widehat{C}_s = \sum_{t=0}^{\tau-1}(x_t^\top Q x_t + u_t^\top R u_t)$, and repeating this for $n_s$ independently sampled perturbation directions $U_1, \ldots, U_{n_s}$. The resulting estimator
\begin{equation*}
    \widehat{\nabla}C(K) = \frac{1}{n_s}\sum_{s=1}^{n_s} \frac{n_x n_u}{r^2} \widehat{C}_s U_s
\end{equation*}
converges to the true gradient as $n_s$ grows, but each sample is not a floating-point operation: it is a physical trajectory rollout lasting $\tau$ real-time steps on a live system \cite{dulac-arnold_challenges_2019}. For a drone executing a surveillance mission, each sample means interrupting the mission for an exploratory maneuver lasting potentially thousands of milliseconds while burning battery. For a power grid controller, each sample means applying a deliberately perturbed input that transiently stresses transformer insulation or causes frequency excursions. For a robotic arm on a manufacturing line, it means a measurable interruption to production. The single-agent sample complexity requirement $n_s = \mathcal{O}(1/\epsilon^2)$ translates directly into operational downtime, energy expenditure, and physical wear on safety-critical hardware. This is what makes reducing sample complexity not merely a theoretical desideratum but a practical necessity for continuous, live deployment of model-free control.

A large fleet of heterogeneous autonomous agents offers a natural and powerful solution: if $M$ agents with distinct but similar dynamics collectively pool their trajectory information, each agent's per-round sampling burden decreases proportionally. This is the central insight formalized by Wang et al.~\cite{wang_model-free_2023} in the \texttt{FedLQR} framework, which proves that through federation the required sample size per agent per gradient step decreases from $\mathcal{O}(1/\epsilon^2)$ to $\mathcal{O}(1/(M\epsilon^2))$, a factor-of-$M$ reduction achieved by exploiting the conditional independence of ZO gradient noise across distinct agents (Lemma~4 of \cite{wang_model-free_2023}). The physical interpretation is striking: a fleet of $M = 1000$ heterogeneous robots, each of which would normally require $1000$ trajectory rollouts per gradient step operating alone, now needs only a single trajectory per agent per round to achieve the same gradient accuracy. As $M$ grows further, the required per-agent sample count approaches zero, opening the door to a regime in which the majority of agents remain dormant during any given learning round---contributing no trajectory samples at all---while still benefiting from policy updates driven by the small activated subset. This is the vision of live, large-scale distributed learning: the shared policy improves continuously from collective experience, and the physical disruption imposed on each agent per round becomes vanishingly small.

The mechanism underlying this gain is the $1/(ML)$ scaling in the sample complexity denominator of \cite{wang_model-free_2023}, where $L$ is the number of local updates per round. The variance of the federated ZO gradient estimator decreases as $1/(ML)$ because the estimation errors from distinct agents are conditionally independent given the common filtration---a statistical property that holds even when agents have heterogeneous dynamics, since independence is a property of the trajectory sampling noise, not of the system structure itself. Heterogeneity does introduce an irreducible bias of order $\mathcal{O}(\epsilon_1 + \epsilon_2)$ between the federated gradient direction and each agent's local gradient (Lemma~3 of \cite{wang_model-free_2023}), where $\epsilon_1$ and $\epsilon_2$ bound pairwise differences in state transition and input matrices across the fleet. In the low-heterogeneity regime this bias is small, and the sample efficiency gain dominates: the collaboration is genuinely beneficial precisely because diverse agents contribute statistically independent gradient information, making their collective estimate more efficient than any single agent's data stream alone.

This motivating picture is, however, incomplete in one critical dimension. The sample complexity reduction requires large $M$, but the \texttt{FedLQR} framework requires each of the $M$ agents to upload its full gradient difference $\Delta^{(i)} \in \mathbb{R}^{q \times p}$ at every round, incurring an uplink communication cost of $\mathcal{O}(qp)$ per agent per round. The total server-side reception burden therefore scales as $\mathcal{O}(M \cdot qp)$, growing linearly with the fleet size and quadratically with the system dimension. In precisely the large-$M$ regime where sample efficiency is most attractive---drone swarms of thousands, smart grid networks spanning thousands of nodes, robotic fleets in large-scale warehouses---this communication overhead becomes the binding constraint that prevents realizing the near-zero per-agent sampling benefit. The tension is fundamental and cannot be resolved by addressing communication and sampling separately: realizing vanishingly small per-agent sample counts requires making $M$ large, but doing so with full gradient transmission generates prohibitive uplink load. A framework that scales $M$ upward must simultaneously compress per-agent communication downward, and the compression must be sufficient to keep total uplink cost independent of system dimension.

An additional consideration that reinforces the necessity of local data processing is the distributed, heterogeneous nature of the systems themselves. Each agent's trajectory data encodes information about its specific system matrices $(A^{(n)}, B^{(n)})$, which in many deployment contexts---heterogeneous robot fleets, vehicles from different manufacturers, industrial actuators with proprietary calibration data---represent operationally sensitive system characteristics. The federated learning paradigm \cite{mcmahan_communication-efficient_2017, konevcny_federated_2016} was designed precisely for such settings: agents process their trajectory data locally and transmit only distilled gradient information to a central coordinator, respecting the natural data locality that is inherent to distributed physical systems. By keeping raw trajectories on-device, federation aligns with this locality constraint and enables large-scale collaboration without requiring centralized access to each agent's raw operational data.

At the same time, there has been growing interest in applying learning-based methods to classical control problems, where safety, stability, and reliability are fundamental requirements. In particular, the Linear Quadratic Regulator (LQR) problem has emerged as a canonical benchmark for data-driven control, providing a structured setting in which learning-based policy optimization methods can be rigorously analyzed. Policy optimization (PO) has proved to be a promising approach for data-driven optimal control in various settings \cite{hu_toward_2023, talebi_policy_2026}. Despite the lack of convexity in simple control settings, policy gradient (PG) methods have been shown to be globally convergent for structured settings such as the LQR problem \cite{fazel_global_2018}. However, deploying these methods on physical hardware at scale is currently intractable due to two converging bottlenecks:
\begin{enumerate}
    \item \textbf{Communication Overload:} Transmitting high-dimensional gradients at each learning round is infeasible under the tight bandwidth constraints of distributed autonomous systems, and the total uplink burden grows with fleet size precisely when large fleets are needed to reduce per-agent sample cost.
    \item \textbf{Sample Inefficiency:} Model-free policy gradient methods require $\mathcal{O}(1/\epsilon^2)$ physical trajectory rollouts per gradient step, which is incompatible with the limited operational availability and safety requirements of physical systems operating in live environments.
\end{enumerate}

To address these challenges, Alemzadeh et al.~(2024) proposes \texttt{D2SPI}, a data-driven geometric policy iteration that utilizes the algebraic structures of interactions to learn an optimal policy for all homogeneous agents in the network \cite{alemzadeh_data-driven_2024}. It utilizes temporary ``auxiliary'' communication links on a (much smaller) subnetwork during the learning phase to handle the coupling in the costs---links that will be removed subsequently for the final distributed feedback synthesis. In absence of coupling in the costs, Wang et al.~(2023) introduced \texttt{FedLQR}, a framework where $M$ agents with unknown, distinct yet similar dynamics collaboratively learn an optimal policy \cite{wang_model-free_2023}. While \texttt{FedLQR} provides a rigorous foundation for stability and sample complexity reduction proportional to $M$, it still relies on sharing full matrix updates at each round. This leaves the communication overhead unsolved at the very scale where the sample efficiency gains become most significant: activating $M$ agents to drive per-agent sample cost toward a single trajectory is theoretically possible, but uploading $M$ full gradient matrices per round is operationally infeasible in bandwidth-constrained deployments.

In this work, we propose \texttt{ScalarFedLQR}, which resolves this tension by fundamentally compressing the uplink. Instead of transmitting the full policy gradient $\nabla J(K) \in \mathbb{R}^d$, each participating agent computes a local zeroth-order gradient estimate $\hat{\nabla}J(K)$, samples a random Rademacher direction $v$ locally, and uploads only the single scalar inner product $\langle v, \hat{\nabla}J(K)\rangle$ together with the random seed. This reduces uplink communication from $\mathcal{O}(d)$ to $\mathcal{O}(1)$, independent of system dimension, making the total server reception burden $\mathcal{O}(m)$ for $m$ active clients rather than $\mathcal{O}(m \cdot d)$. Because per-agent uplink cost is now constant, arbitrarily large fleets can participate without communication constraints, which in turn allows $m$ to grow freely and drives each agent's per-round sample requirement toward the near-zero regime that large-scale live learning demands.

Critically, the quality of gradient reconstruction does not degrade as $m$ grows---it improves. The server aggregates $m$ scalar projections, each encoding a rank-one view of a local gradient estimate, and reconstructs a global descent direction through averaging. The projection error from this compression scales as $1/\sqrt{m}$ with the number of active clients (Lemmas~III.6 and~III.7), directly mirroring \texttt{FedLQR}'s $1/M$ variance reduction for zeroth-order noise. More participating agents means better gradient recovery from scalar information alone, providing a compounding benefit: larger active sets simultaneously reduce per-agent sample requirements and reduce projection reconstruction error.

Beyond communication efficiency, this scalar projection mechanism provides structural privacy as a natural consequence of the encoding. Since the server observes only the rank-one projection $vv^\top \hat{\nabla}J(K)$, all gradient components in the null space of $vv^\top$ remain completely unobservable, preventing direct reconstruction of local system dynamics or trajectory data. This null-space masking provides a principled form of privacy preservation without requiring explicit noise injection, analogous to the scalar-communication mechanisms in recent federated learning frameworks \cite{rostami_fedscalar_2024}. Taken together, \texttt{ScalarFedLQR} realizes the vision of continuous, large-scale distributed autonomy: fleets of heterogeneous physical systems each contributing at most one trajectory per learning round---and often none---while a shared stabilizing policy converges through lightweight scalar exchanges.
```

==> intro2.tex <==
\section{Introduction}

The deployment of policy gradient methods for model-free optimal control of physical dynamical systems faces a bottleneck that is often underappreciated in theoretical treatments but is decisive in real-world operation: the physical cost of a single gradient sample. In the zeroth-order (ZO) optimization framework that underlies model-free LQR \cite{fazel_global_2018, malik_derivative-free_2019}, estimating the gradient of the LQR cost $C(K)$ with respect to the policy gain $K$ requires physically executing a perturbed policy $\widehat{K}_s = K + U_s$ on the dynamical system, recording the resulting state trajectory $x_0, x_1, \ldots, x_\tau$, computing the finite-horizon accumulated cost $\widehat{C}_s = \sum_{t=0}^{\tau-1}(x_t^\top Q x_t + u_t^\top R u_t)$, and repeating this for $n_s$ independently sampled perturbation directions $U_1, \ldots, U_{n_s}$. The resulting estimator
\begin{equation*}
    \widehat{\nabla}C(K) = \frac{1}{n_s}\sum_{s=1}^{n_s} \frac{n_x n_u}{r^2} \widehat{C}_s U_s
\end{equation*}
converges to the true gradient as $n_s$ grows, but each sample is not a floating-point operation: it is a physical trajectory rollout lasting $\tau$ real-time steps on a live system \cite{dulac-arnold_challenges_2019}.

A subtlety worth noting is why $n_s$ samples are required rather than the $d = n_x n_u$ samples that would suffice for exact coordinate-wise finite differences. In classical deterministic optimization, perturbing each of the $d$ coordinates of $K$ independently recovers the full gradient with exactly $d$ exact function evaluations. In the ZO LQR setting this assumption fails entirely: the cost $C(K) = \mathbb{E}_{x_0 \sim \mathcal{D}}\bigl[\sum_{t=0}^{\infty} x_t^\top Q x_t + u_t^\top R u_t\bigr]$ is an expectation over random initial conditions, and each trajectory rollout returns a single noisy realization $\widehat{C}_s$ of this expectation. Repeating the identical perturbation direction yields a different cost estimate because $x_0$ is redrawn each time. The requirement $n_s = \mathcal{O}(1/\epsilon^2)$ is therefore a purely statistical variance-reduction requirement---the Monte Carlo price of estimating an expectation from samples---entirely independent of the need to cover $d$ gradient directions. Dimension does enter the sample complexity, but only through the noise level of the estimator: the $n_x n_u / r^2$ prefactor in $\widehat{\nabla}C(K)$ and the $\min(n_x, n_u)\log[(n_x + n_u)/\delta]$ factor in Lemma~14 of~\cite{wang_model-free_2023} quantify the variance of the stochastic cost oracle rather than a coverage requirement. Crucially, the random smoothing estimator simultaneously probes all $d$ gradient components through the random outer product $\widehat{C}_s U_s$, so each physical rollout contributes information about every direction at once \cite{nesterov_random_2017}---an efficiency property that coordinate-wise perturbations do not share when the oracle is stochastic.

For a drone executing a surveillance mission, each sample means interrupting the mission for an exploratory maneuver lasting potentially thousands of milliseconds while burning battery. For a power grid controller, each sample means applying a deliberately perturbed input that transiently stresses transformer insulation or causes frequency excursions. For a robotic arm on a manufacturing line, it means a measurable interruption to production. The single-agent sample complexity requirement $n_s = \mathcal{O}(1/\epsilon^2)$ translates directly into operational downtime, energy expenditure, and physical wear on safety-critical hardware. This is what makes reducing sample complexity not merely a theoretical desideratum but a practical necessity for continuous, live deployment of model-free control.

A large fleet of heterogeneous autonomous agents offers a natural and powerful solution: if $M$ agents with distinct but similar dynamics collectively pool their trajectory information, each agent's per-round sampling burden decreases proportionally. This is the central insight formalized by Wang et al.~\cite{wang_model-free_2023} in the \texttt{FedLQR} framework, which proves that through federation the required sample size per agent per gradient step decreases from $\mathcal{O}(1/\epsilon^2)$ to $\mathcal{O}(1/(M\epsilon^2))$, a factor-of-$M$ reduction achieved by exploiting the conditional independence of ZO gradient noise across distinct agents (Lemma~4 of \cite{wang_model-free_2023}). The physical interpretation is striking: a fleet of $M = 1000$ heterogeneous robots, each of which would normally require $1000$ trajectory rollouts per gradient step operating alone, now needs only a single trajectory per agent per round to achieve the same gradient accuracy. As $M$ grows further, the required per-agent sample count approaches zero, opening the door to a regime in which the majority of agents remain dormant during any given learning round---contributing no trajectory samples at all---while still benefiting from policy updates driven by the small activated subset. This is the vision of live, large-scale distributed learning: the shared policy improves continuously from collective experience, and the physical disruption imposed on each agent per round becomes vanishingly small.

It is important to distinguish between the cost of operating under a policy and the cost of contributing a gradient sample. A dormant agent running under the current shared policy $K_t$ incurs only its baseline operational cost---burning fuel on its mission, regulating its load, executing its task---regardless of whether a learning round is taking place. An active agent, by contrast, must deviate from this nominal behavior for $\tau$ real-time steps by applying the deliberately perturbed policy $K_t + U_s$, absorbing additional energy expenditure, actuator stress, and mission disruption beyond what nominal operation demands. This contrast defines the true price of participation, and it is both context-dependent and system-dependent. A drone in open airspace can tolerate an exploratory maneuver; one navigating a tight corridor cannot. A grid node during off-peak hours can absorb a perturbed input; one under peak demand cannot. From a learning-theoretic standpoint, activating more agents is always beneficial---the projection error in \texttt{ScalarFedLQR} scales as $\mathcal{O}(1/\sqrt{m})$ with the number of active clients (Lemmas~III.6 and~III.7), so each additional participant directly tightens gradient reconstruction and accelerates convergence. Yet when agents have the operational flexibility to sit out a round, there is every reason to let them: a dormant agent avoids all exploration cost, receives the updated policy $K_{t+1}$ from the server broadcast at zero physical cost, and continues its mission uninterrupted. In large-scale deployments where $m$ need only be a small fraction of $M$ to achieve sufficient gradient accuracy, the exploration burden can be distributed across a rotating subset of the fleet, keeping the per-agent disruption as infrequent as the system can afford.

The mechanism underlying this gain is the $1/(ML)$ scaling in the sample complexity denominator of \cite{wang_model-free_2023}, where $L$ is the number of local updates per round. The variance of the federated ZO gradient estimator decreases as $1/(ML)$ because the estimation errors from distinct agents are conditionally independent given the common filtration---a statistical property that holds even when agents have heterogeneous dynamics, since independence is a property of the trajectory sampling noise, not of the system structure itself. Heterogeneity does introduce an irreducible bias of order $\mathcal{O}(\epsilon_1 + \epsilon_2)$ between the federated gradient direction and each agent's local gradient (Lemma~3 of \cite{wang_model-free_2023}), where $\epsilon_1$ and $\epsilon_2$ bound pairwise differences in state transition and input matrices across the fleet. In the low-heterogeneity regime this bias is small, and the sample efficiency gain dominates: the collaboration is genuinely beneficial precisely because diverse agents contribute statistically independent gradient information, making their collective estimate more efficient than any single agent's data stream alone.

This motivating picture is, however, incomplete in one critical dimension. The sample complexity reduction requires large $M$, but the \texttt{FedLQR} framework requires each of the $M$ agents to upload its full gradient difference $\Delta^{(i)} \in \mathbb{R}^{q \times p}$ at every round, incurring an uplink communication cost of $\mathcal{O}(qp)$ per agent per round. The total server-side reception burden therefore scales as $\mathcal{O}(M \cdot qp)$, growing linearly with the fleet size and quadratically with the system dimension. In precisely the large-$M$ regime where sample efficiency is most attractive---drone swarms of thousands, smart grid networks spanning thousands of nodes, robotic fleets in large-scale warehouses---this communication overhead becomes the binding constraint that prevents realizing the near-zero per-agent sampling benefit. The tension is fundamental and cannot be resolved by addressing communication and sampling separately: realizing vanishingly small per-agent sample counts requires making $M$ large, but doing so with full gradient transmission generates prohibitive uplink load. A framework that scales $M$ upward must simultaneously compress per-agent communication downward, and the compression must be sufficient to keep total uplink cost independent of system dimension.

An additional consideration that reinforces the necessity of local data processing is the distributed, heterogeneous nature of the systems themselves. Each agent's trajectory data encodes information about its specific system matrices $(A^{(n)}, B^{(n)})$, which in many deployment contexts---heterogeneous robot fleets, vehicles from different manufacturers, industrial actuators with proprietary calibration data---represent operationally sensitive system characteristics. The federated learning paradigm \cite{mcmahan_communication-efficient_2017, konevcny_federated_2016} was designed precisely for such settings: agents process their trajectory data locally and transmit only distilled gradient information to a central coordinator, respecting the natural data locality that is inherent to distributed physical systems. By keeping raw trajectories on-device, federation aligns with this locality constraint and enables large-scale collaboration without requiring centralized access to each agent's raw operational data.

At the same time, there has been growing interest in applying learning-based methods to classical control problems, where safety, stability, and reliability are fundamental requirements. In particular, the Linear Quadratic Regulator (LQR) problem has emerged as a canonical benchmark for data-driven control, providing a structured setting in which learning-based policy optimization methods can be rigorously analyzed. Policy optimization (PO) has proved to be a promising approach for data-driven optimal control in various settings \cite{hu_toward_2023, talebi_policy_2026}. Despite the lack of convexity in simple control settings, policy gradient (PG) methods have been shown to be globally convergent for structured settings such as the LQR problem \cite{fazel_global_2018}. However, deploying these methods on physical hardware at scale is currently intractable due to two converging bottlenecks:
\begin{enumerate}
    \item \textbf{Communication Overload:} Transmitting high-dimensional gradients at each learning round is infeasible under the tight bandwidth constraints of distributed autonomous systems, and the total uplink burden grows with fleet size precisely when large fleets are needed to reduce per-agent sample cost.
    \item \textbf{Sample Inefficiency:} Model-free policy gradient methods require $\mathcal{O}(1/\epsilon^2)$ physical trajectory rollouts per gradient step, which is incompatible with the limited operational availability and safety requirements of physical systems operating in live environments.
\end{enumerate}

To address these challenges, Alemzadeh et al.~(2024) proposes \texttt{D2SPI}, a data-driven geometric policy iteration that utilizes the algebraic structures of interactions to learn an optimal policy for all homogeneous agents in the network \cite{alemzadeh_data-driven_2024}. It utilizes temporary ``auxiliary'' communication links on a (much smaller) subnetwork during the learning phase to handle the coupling in the costs---links that will be removed subsequently for the final distributed feedback synthesis. In absence of coupling in the costs, Wang et al.~(2023) introduced \texttt{FedLQR}, a framework where $M$ agents with unknown, distinct yet similar dynamics collaboratively learn an optimal policy \cite{wang_model-free_2023}. While \texttt{FedLQR} provides a rigorous foundation for stability and sample complexity reduction proportional to $M$, it still relies on sharing full matrix updates at each round. This leaves the communication overhead unsolved at the very scale where the sample efficiency gains become most significant: activating $M$ agents to drive per-agent sample cost toward a single trajectory is theoretically possible, but uploading $M$ full gradient matrices per round is operationally infeasible in bandwidth-constrained deployments.

In this work, we propose \texttt{ScalarFedLQR}, which resolves this tension by fundamentally compressing the uplink. Instead of transmitting the full policy gradient $\nabla J(K) \in \mathbb{R}^d$, each participating agent computes a local zeroth-order gradient estimate $\hat{\nabla}J(K)$, samples a random Rademacher direction $v$ locally, and uploads only the single scalar inner product $\langle v, \hat{\nabla}J(K)\rangle$ together with the random seed. This reduces uplink communication from $\mathcal{O}(d)$ to $\mathcal{O}(1)$, independent of system dimension, making the total server reception burden $\mathcal{O}(m)$ for $m$ active clients rather than $\mathcal{O}(m \cdot d)$. Because per-agent uplink cost is now constant, arbitrarily large fleets can participate without communication constraints, which in turn allows $m$ to grow freely and drives each agent's per-round sample requirement toward the near-zero regime that large-scale live learning demands.

Critically, the quality of gradient reconstruction does not degrade as $m$ grows---it improves. The server aggregates $m$ scalar projections, each encoding a rank-one view of a local gradient estimate, and reconstructs a global descent direction through averaging. The projection error from this compression carries a dimension-dependent factor of $(d-1)$ in the worst-case bound (Corollary~III.5), reflecting the algebraic cost of discarding all but one scalar degree of freedom per agent. However, under client averaging this dimension dependence is tamed: the high-probability bound on the projection error scales as $\mathcal{O}\!\left(\sqrt{(d-1)\log(2d/\delta)/m}\right)$ with the number of active clients $m$ (Lemmas~III.6 and~III.7), directly mirroring \texttt{FedLQR}'s $1/M$ variance reduction for zeroth-order noise. More participating agents means better gradient recovery from scalar information alone, providing a compounding benefit: larger active sets simultaneously reduce per-agent sample requirements and reduce projection reconstruction error, and in the large-fleet regime the $(d-1)$ dimension factor is effectively neutralized by the $1/\sqrt{m}$ decay.

A subtlety worth addressing is why $n_s$ samples are required rather than the $d = n_x n_u$
samples that would suffice for exact coordinate-wise finite differences. In classical deterministic
optimization, perturbing each coordinate of $K$ independently recovers the full gradient with
exactly $d$ oracle queries. In the ZO LQR setting this logic fails entirely: the cost
$C(K) = \mathbb{E}_{x_0 \sim \mathcal{D}}\bigl[\sum_{t=0}^{\infty} x_t^\top Q x_t + u_t^\top R
u_t\bigr]$ is an \emph{expectation} over random initial conditions, so each trajectory rollout
returns a noisy realization of this expectation. Repeating the identical perturbation direction
yields a different cost estimate because $x_0$ is redrawn each time. The requirement
$n_s = \mathcal{O}(1/\epsilon^2)$ is therefore a purely statistical variance-reduction
requirement---the Monte Carlo price of estimating a stochastic oracle---entirely separate from
the need to cover $d$ gradient directions. Dimension enters only through the noise level of the
estimator: the $n_x n_u / r^2$ prefactor in $\widehat{\nabla}C(K)$ reflects the variance of the
smoothed cost oracle rather than a coverage requirement. Crucially, the random smoothing
estimator simultaneously probes all $d$ gradient components through the outer product
$\widehat{C}_s U_s$, so each physical rollout contributes information about every direction at
once \cite{nesterov_random_2017}---an efficiency property that coordinate-wise perturbations do
not share when the oracle is stochastic.


Beyond communication efficiency, this scalar projection mechanism provides structural privacy as a natural consequence of the encoding. Since the server observes only the rank-one projection $vv^\top \hat{\nabla}J(K)$, all gradient components in the null space of $vv^\top$ remain completely unobservable, preventing direct reconstruction of local system dynamics or trajectory data. This null-space masking provides a principled form of privacy preservation without requiring explicit noise injection, analogous to the scalar-communication mechanisms in recent federated learning frameworks \cite{rostami_fedscalar_2024}. Taken together, \texttt{ScalarFedLQR} realizes the vision of continuous, large-scale distributed autonomy: fleets of heterogeneous physical systems each contributing at most one trajectory per learning round---and often none---while a shared stabilizing policy converges through lightweight scalar exchanges.

==> intro3.tex <==
\section{Introduction}

The deployment of policy gradient methods for model-free optimal LQR control of physical dynamical systems
faces a bottleneck that is often underappreciated in theoretical treatments but is decisive in
real-world operation: the physical cost of a single gradient sample. In the zeroth-order (ZO)
optimization framework that underlies model-free LQR \cite{fazel_global_2018, malik_derivative-free_2019} for an LTI system with $n_x$ states and $n_u$ control,
estimating the gradient of the LQR cost $C(K)$ with respect to the policy gain $K\in\mathbb{R}^{n_x\times n_u}$ requires
physically executing a perturbed policy $\widehat{K}_s = K + U_s$ on the dynamical system,
recording the resulting state trajectory $x_0, x_1, \ldots, x_\tau$, computing the finite-horizon
accumulated cost $\widehat{C}_s = \sum_{t=0}^{\tau-1}(x_t^\top Q x_t + u_t^\top R u_t)$, and
repeating this for $n_s$ independently sampled perturbation directions $U_1, \ldots, U_{n_s}$.
The resulting estimator
\begin{equation*}
    \widehat{\nabla}C(K) = \frac{1}{n_s}\sum_{s=1}^{n_s} \frac{n_x n_u}{r^2} \widehat{C}_s U_s
\end{equation*}
converges to the true gradient as $n_s$ grows, but each sample is not a floating-point
operation---it is a physical trajectory rollout lasting $\tau$ real-time steps on a live system
\cite{dulac-arnold_challenges_2019}.

Unlike coordinate-wise finite differences---which recover the full gradient
with exactly $d = n_x n_u$ deterministic oracle queries---the ZO LQR estimator
requires $n_s \gg d$ rollouts. The reason is that
\begin{equation*}
  C(K) = \mathbb{E}_{x_0 \sim \mathcal{D}}\!\left[\sum_{t=0}^{\infty}
  x_t^{\top} Q x_t + u_t^{\top} R u_t\right]
\end{equation*}
is an \emph{expectation} over random initial conditions, so each rollout
returns only a noisy realization; repeating the identical perturbation
direction yields a different cost estimate because $x_0$ is redrawn each
time. The required sample count of $n_s = \mathcal{O}(1/\epsilon^2)$ is therefore a purely statistical
variance-reduction requirement---the Monte Carlo price of estimating a
stochastic oracle---entirely separate from the need to probe $d$ gradient
directions, where $\epsilon > 0$ denotes the target gradient estimation
accuracy, i.e., the maximum allowable deviation
$\|\widehat{\nabla}C(K) - \nabla C(K)\|_F \leq \epsilon$
between the zeroth-order estimator and the true policy gradient. Dimension enters only through the $n_x n_u / r^2$ noise
prefactor in $\widehat{\nabla}C(K)$, not as a coverage
requirement~\cite{nesterov_random_2017}. In practice, for a drone, generating each sample means
interrupting a surveillance mission for an exploratory maneuver while
burning battery; for a power grid controller, it means applying a perturbed
input that stresses transformer insulation; for a robotic arm, it means
measurable production downtime. This is what makes reducing sample
complexity not merely a theoretical desideratum but a practical necessity
for continuous, live deployment of model-free control.


An interesting avenue, however, exists for reducing sampling cost in
large-scale multi-agent operations. In many practical
deployments---drone swarms, robotic fleets, or networks of industrial
controllers---agents are nominally identical but exhibit slightly
distinct dynamics due to manufacturing tolerances, actuator wear, or
environmental calibration differences. No two units are exactly alike,
yet their dynamics share the same underlying structure. Formally, when the fleet is modeled as $M$ agents with \emph{distinct but similar} dynamics, they can pool their trajectory information, reducing each agent's
per-round sampling burden proportionally. This is the central insight
formalized by Wang et al.~\cite{wang_model-free_2023} in the
\texttt{FedLQR} framework, which proves that the required sample size
per agent decreases from $\mathcal{O}(1/\epsilon^2)$ to
$\mathcal{O}(1/(M\epsilon^2))$, a factor-of-$M$ reduction achieved by
exploiting the conditional independence of ZO gradient noise across
distinct agents (Lemma~4 of \cite{wang_model-free_2023}). The practical implication is striking: consider a fleet of $M = 1000$ robots, each of which
would require $1000$ trajectory rollouts per gradient step operating
alone; under \texttt{FedLQR}, the same gradient accuracy is achieved
with only a single rollout per agent per round. 

In a large-scale operation, as $M$ grows, the required per-agent sample
count approaches zero. This naturally points to a regime that goes
\emph{beyond} \texttt{FedLQR}: rather than requiring all $M$ agents to
participate at every round, only an active subset
$\mathcal{A}^t \subseteq [M]$ of size $m = |\mathcal{A}^t|$ need
contribute gradient samples---precisely the partial-participation
setting that federated learning was originally designed
for~\cite{mcmahan_communication-efficient_2017, konevcny_federated_2016}.
The remaining $M - m$ agents stay dormant, free to recharge, offload
local computation, or dedicate their communication resources to other
onboard tasks, while still receiving the updated policy $K_{t+1}$ from
the server broadcast at zero physical cost.

This active--dormant distinction reflects a fundamental asymmetry in
participation cost. A dormant agent running under the current shared
policy $K_t$ incurs only its baseline operational cost. An active agent,
by contrast, must deviate from nominal behavior for $\tau$ real-time
steps by executing the deliberately perturbed policy $K_t + U_s$,
absorbing additional energy expenditure, actuator stress, and mission
disruption. This contrast is context- and system-dependent: a drone in
open airspace can tolerate an exploratory maneuver; one in a tight
corridor cannot. From a learning-theoretic standpoint, activating more
agents is always beneficial---each additional participant directly
tightens gradient reconstruction and accelerates convergence---yet when
agents have the operational flexibility to sit out a round, there is
every reason to let them. Realizing this partial-participation regime at
scale, however, exposes a second bottleneck that sample-complexity
analysis alone does not capture: the communication cost incurred by
each agent that does participate.

Indeed, this motivating picture is incomplete in one critical dimension.
While the sample complexity reduction justifies scaling $M$ upward and
activating only a subset $m \ll M$ of agents per round,
\texttt{FedLQR} requires each agent to upload its full gradient
difference $\Delta^{(i)} \in \mathbb{R}^{n_u \times n_x}$ at every
round, incurring an uplink cost of $\mathcal{O}(n_u n_x)$ per agent
per round. The total server-side reception burden therefore scales as
$\mathcal{O}(M \cdot n_u n_x)$, growing linearly with fleet size and
quadratically with system dimension---precisely the regime where the sample-efficiency gains of
large-$M$ collaboration are most attractive. A framework that scales $M$
upward and activates a subset downward must simultaneously compress
per-agent communication to a constant-size message. An additional
consideration reinforces this need: each agent's trajectory data encodes
its specific system matrices $(A^{(n)}, B^{(n)})$, which in many
deployment contexts represent operationally sensitive characteristics.
Transmitting full gradient matrices enables gradient inversion and system
identification attacks, exposing local dynamics to the server. These two
requirements---constant-size uplink and structural privacy---call for a
communication mechanism that decouples transmission cost from system
dimension while masking the gradient geometry by design. Addressing both
simultaneously, alongside the partial-participation structure motivated
above, is the central contribution of \texttt{ScalarFedLQR}.

At the same time, there has been growing interest in applying learning-based methods to classical
control problems, where safety, stability, and reliability are fundamental requirements.
Policy optimization (PO) has proved to be a promising approach for data-driven optimal control
in various settings \cite{hu_toward_2023, talebi_policy_2026}. Despite the lack of convexity
in simple control settings, policy gradient (PG) methods have been shown to be globally convergent
for structured settings such as the LQR problem \cite{fazel_global_2018}. However, deploying
these methods on physical hardware at scale is currently intractable due to two converging
bottlenecks:
\begin{enumerate}
    \item \textbf{Communication Overload:} Transmitting high-dimensional gradients at each
    learning round is infeasible under the tight bandwidth constraints of distributed autonomous
    systems, and the total uplink burden grows with fleet size precisely when large fleets are
    needed to reduce per-agent sample cost.
    \item \textbf{Sample Inefficiency:} Model-free policy gradient methods require
    $\mathcal{O}(1/\epsilon^2)$ physical trajectory rollouts per gradient step, which is
    incompatible with the limited operational availability and safety requirements of physical
    systems operating in live environments.
\end{enumerate}

To address these challenges, Alemzadeh et al.~(2024) proposes \texttt{D2SPI}, a data-driven
geometric policy iteration that utilizes the algebraic structures of interactions to learn an
optimal policy for all homogeneous agents in the network \cite{alemzadeh_data-driven_2024}.
In absence of coupling in the costs, Wang et al.~(2023) introduced \texttt{FedLQR}, a framework
where $M$ agents with unknown, distinct yet similar dynamics collaboratively learn an optimal
policy \cite{wang_model-free_2023}. While \texttt{FedLQR} provides a rigorous foundation for
stability and sample complexity reduction proportional to $M$, it still relies on sharing full
matrix updates at each round, leaving the communication overhead unsolved at precisely the scale
where the sample efficiency gains become most significant.

In this work, we propose \texttt{ScalarFedLQR}, which resolves this tension by fundamentally
compressing the uplink. Instead of transmitting the full policy gradient
$\nabla J(K) \in \mathbb{R}^d$, each participating agent computes a local zeroth-order gradient
estimate $\hat{\nabla}J(K)$, samples a random Rademacher direction $v$ locally, and uploads only
the single scalar inner product $\langle v, \hat{\nabla}J(K)\rangle$ together with the random
seed. This reduces uplink communication from $\mathcal{O}(d)$ to $\mathcal{O}(1)$, independent
of system dimension, making the total server reception burden $\mathcal{O}(m)$ for $m$ active
clients rather than $\mathcal{O}(m \cdot d)$. The server aggregates $m$ scalar projections and
reconstructs a global descent direction through averaging; the high-probability projection error
scales as $\mathcal{O}\!\left(\sqrt{(d-1)\log(2dT/\delta)/m}\right)$ (Lemmas~III.6
and~III.7), so larger active sets simultaneously reduce per-agent sample requirements and tighten
gradient reconstruction---a compounding benefit that neutralizes the dimension-dependent error
factor in the large-fleet regime. Beyond communication efficiency, since the server observes only
the rank-one projection $vv^\top \hat{\nabla}J(K)$, all gradient components in the null space of
$vv^\top$ remain completely unobservable, providing structural privacy through projection masking
without requiring explicit noise injection, analogous to recent scalar-communication federated
learning frameworks \cite{rostami_fedscalar_2024}. Taken together, \texttt{ScalarFedLQR}
realizes the vision of continuous, large-scale distributed autonomy: fleets of heterogeneous
physical systems each contributing at most one trajectory per learning round---and often
none---while a shared stabilizing policy converges through lightweight scalar exchanges.

==> intro4.tex <==
\section{Introduction}

The deployment of policy gradient methods for model-free optimal LQR
control of physical dynamical systems faces a bottleneck that is often
underappreciated in theoretical treatments but is decisive in real-world
operation: the physical cost of a single gradient sample. In the
zeroth-order (ZO) optimization framework that underlies model-free
LQR~\cite{fazel_global_2018, malik_derivative-free_2019}, estimating
the gradient of the LQR cost $C(K)$ with respect to the policy gain
$K \in \mathbb{R}^{n_u \times n_x}$ requires physically executing a
perturbed policy $\widehat{K}_s = K + U_s$ on the dynamical system,
recording the resulting state trajectory, computing the finite-horizon
accumulated cost, and repeating this for $n_s$ independently sampled
perturbation directions. The resulting estimator
\begin{equation*}
    \widehat{\nabla}C(K) = \frac{1}{n_s}\sum_{s=1}^{n_s}
    \frac{n_x n_u}{r^2} \widehat{C}_s U_s
\end{equation*}
converges to the true gradient as $n_s$ grows, requiring $n_s = \mathcal{O}(1/\epsilon^2)$ samples to
reduce the gradient estimation error below $\epsilon > 0$. But each sample is not a
floating-point operation---it is a physical trajectory rollout lasting
$\tau$ real-time steps on a live system~\cite{dulac-arnold_challenges_2019}.

In practice, for a drone, generating each sample means interrupting a
surveillance mission for an exploratory maneuver while burning battery;
for a power grid controller, it means applying a perturbed input that
stresses transformer insulation; for a robotic arm, it means measurable
production downtime. This is what makes reducing sample complexity not merely a theoretical desideratum but a practical necessity for continuous, live deployment of model-free control.

An interesting avenue exists for reducing sampling cost in large-scale multi-agent operations. When a fleet of $M$ agents with \emph{distinct but similar} dynamics\footnote{In many practical deployments---drone swarms, robotic fleets, or networks of industrial controllers---agents are nominally identical but exhibit slightly distinct dynamics due to manufacturing tolerances, actuator wear, or environmental calibration differences.} can pool their trajectory information, each agent's per-round sampling burden reduces by a factor of $M$. This is the central insight formalized by Wang et al.~\cite{wang_model-free_2023} in the \texttt{FedLQR} framework, which proves that the required sample size per agent decreases from $\mathcal{O}(1/\epsilon^2)$ to $\mathcal{O}(1/(M\epsilon^2))$, a factor-of-$M$ reduction achieved by exploiting the conditional independence of ZO gradient noise across distinct agents (Lemma~4 of \cite{wang_model-free_2023}). The result is striking: consider a fleet of $M = 1000$ robots, each of which would require $1000$ trajectory rollouts per gradient step operating alone; under \texttt{FedLQR}, the same gradient accuracy is achieved with only a single rollout per agent per round.

Despite offering a compelling foundation for collaborative
model-free LQR, two concerns yet arise when deploying \texttt{FedLQR} of~\cite{wang_model-free_2023}  at scale.
The first is operational: requiring all $M$ agents to actively collect gradient samples at every round forces every unit into continuous exploratory excitation, regardless of whether its local conditions permit safe deviation from nominal behavior.
The second is informational: even with full participation, each active agent must transmit a full gradient matrix per round, incurring a communication cost that grows with both fleet size and system dimension. The first concern can  naturally be resolved within the federated learning paradigm itself. Since the per-agent sample requirement already scales as $\mathcal{O}(1/(M\epsilon^2))$, for any realistic fleet size $M$ this burden becomes small enough that only a subset $m=|\mathcal{A}_t|$ of agents need contribute gradient samples at each round. The inactive agents can use the disengagement window to recharge, offload local computation, or dedicate their communication resources to other onboard tasks and still receive the updated policy
$K_{t+1}$ from the server broadcast at zero cost. The second
concern, however, is not resolved by \texttt{FedLQR} and
becomes more acute precisely as $M$ grows.



 Concretely, \texttt{FedLQR} requires each participating agent to upload
its full gradient difference $\Delta^{(i)} \in \mathbb{R}^{n_u \times n_x}$,
incurring an uplink cost of $\mathcal{O}(n_u n_x)$ per agent per round.
The total server-side reception burden therefore scales as
$\mathcal{O}(m \cdot d)$ where $d = n_u n_x$, growing quadratically with
system dimension---precisely the regime where the sample-efficiency gains
of large-$M$ collaboration are most attractive. An additional consideration
reinforces this need: each agent's trajectory data encodes its specific
system matrices $(A^{(n)}, B^{(n)})$, which in many deployment contexts
represent operationally sensitive characteristics. Transmitting full gradient
matrices enables gradient inversion and system identification attacks,
exposing local dynamics to the server. These two requirements---constant-size
uplink and structural privacy---call for a communication mechanism that
decouples transmission cost from system dimension while masking the gradient
geometry by design.

At the same time, policy optimization (PO) has proved to be a promising
approach for data-driven optimal control in various
settings~\cite{hu_toward_2023, talebi_policy_2026}, and despite the
lack of convexity in simple control settings, policy gradient (PG)
methods have been shown to be globally convergent for structured
settings such as the LQR problem~\cite{fazel_global_2018}. However,
deploying these methods on physical hardware at scale remains
intractable due to two converging bottlenecks: \textbf{(i) Communication
Overload}, where transmitting high-dimensional gradients is infeasible
under tight bandwidth constraints and the total uplink burden grows with
fleet size precisely when large fleets are needed to reduce per-agent
sample cost; and \textbf{(ii) Sample Inefficiency}, where model-free
policy gradient methods require $\mathcal{O}(1/\epsilon^2)$ physical
trajectory rollouts per gradient step, incompatible with the limited
operational availability of physical systems in live environments. To
address these challenges, Alemzadeh et al.~(2024) propose \texttt{D2SPI}
for homogeneous networks~\cite{alemzadeh_data-driven_2024}, and Wang
et al.~(2023) introduced \texttt{FedLQR} for $M$ agents with unknown,
distinct yet similar dynamics~\cite{wang_model-free_2023}. While
\texttt{FedLQR} provides a rigorous foundation for stability and
sample complexity reduction proportional to $M$, it still relies on
sharing full matrix updates at each round, leaving the communication
overhead unsolved at precisely the scale where the sample efficiency
gains become most significant.

In this work, we propose \texttt{ScalarFedLQR}, which resolves this
tension by fundamentally compressing the uplink. Instead of transmitting
the full policy gradient $\nabla J(K) \in \mathbb{R}^d$, each
participating agent computes a local zeroth-order gradient estimate
$\hat{\nabla}J(K)$, samples a random Rademacher direction $v$ locally,
and uploads only the single scalar inner product
$\langle v, \hat{\nabla}J(K)\rangle$ together with the random seed.
This reduces uplink communication from $\mathcal{O}(d)$ to
$\mathcal{O}(1)$, independent of system dimension, making the total
server reception burden $\mathcal{O}(m)$ for $m$ active clients rather
than $\mathcal{O}(m \cdot d)$. The server aggregates $m$ scalar
projections and reconstructs a global descent direction through
averaging; the high-probability projection error scales as
$\mathcal{O}\!\left(\sqrt{(d-1)\log(2dT/\delta)/m}\right)$
(Lemmas~III.6 and~III.7), so larger active sets simultaneously reduce
per-agent sample requirements and tighten gradient
reconstruction---a compounding benefit that neutralizes the
dimension-dependent error factor in the large-fleet regime. Beyond
communication efficiency, since the server observes only the rank-one
projection $vv^\top \hat{\nabla}J(K)$, all gradient components in the
null space of $vv^\top$ remain completely unobservable, providing
structural privacy through projection masking without requiring explicit
noise injection, analogous to recent scalar-communication federated
learning frameworks~\cite{rostami_fedscalar_2024}. Taken together,
\texttt{ScalarFedLQR} realizes the vision of continuous, large-scale
distributed autonomy: fleets of heterogeneous physical systems each
contributing at most one trajectory per learning round---and often
none---while a shared stabilizing policy converges through lightweight
scalar exchanges.

==> intro5.tex <==
\section{Introduction}

Policy optimization (PO) is a promising paradigm for data-driven control~\cite{hu_toward_2023, talebi_policy_2026}. Despite nonconvexity, policy gradient (PG) methods enjoy global convergence in structured settings such as LQR~\cite{fazel_global_2018,bu_lqr_2019}. However, large-scale deployment on physical systems is constrained by two fundamental bottlenecks: (i) communication overload, as transmitting high-dimensional gradients under limited bandwidth becomes prohibitive and scales with fleet size~\cite{mcmahan_communication-efficient_2017, konevcny_federated_2016}; and (ii) sample inefficiency, since model-free PG requires $\mathcal{O}(1/\epsilon^2)$ trajectory rollouts per step—untenable in real-world operation~\cite{dean_sample_2020}. Recent work partially mitigates these challenges: \texttt{D2SPI} addresses homogeneous networks~\cite{alemzadeh_data-driven_2024}, while FedLQR extends to heterogeneous but similar agents~\cite{wang_model-free_2023}.

A central, often underemphasized limitation underlying these bottlenecks is the \emph{physical cost of each gradient sample}. In zeroth-order (ZO) model-free LQR~\cite{fazel_global_2018, malik_derivative-free_2019}, estimating $\nabla J(K)$ for $K \in \mathbb{R}^{n_u \times n_x}$ requires executing perturbed policies $\widehat{K}_s = K + U_s$, collecting trajectories, and averaging costs over $n_s$ perturbations. The estimator
\begin{equation}\label{eq:local-grad-estimate}
    \widehat{\nabla}J(K) = \frac{1}{n_s}\sum\nolimits_{s=1}^{n_s}
    \frac{n_x n_u}{r^2} \widehat{J}_s U_s 
\end{equation}
with $\widehat{J}_s = J(\widehat{K}_s)$, achieves $\epsilon$-accurate gradients with $n_s = \mathcal{O}(1/\epsilon^2)$. Crucially, each “sample” is not a cheap computation but a full trajectory rollout of length $\tau$ on a live system~\cite{dulac-arnold_challenges_2019}, making sample inefficiency a direct operational burden.

In practice, each sample carries real cost: a drone must interrupt its mission and expend battery on exploration, a power grid controller applies perturbations that stress equipment, and a robotic arm incurs production downtime. Reducing sample complexity is therefore not just theoretical—it is essential for safe, continuous deployment of learning for control and estimation \cite{mohammadi_learning_2020,zhao_global_2023,talebi_data-driven_2023,umenberger_globally_2022}.
A promising solution arises in large-scale multi-agent systems. When $M$ agents with similar (but not identical) dynamics pool their trajectory data, each agent’s sampling burden drops by a factor of $M$. As shown by Wang et al.~\cite{wang_model-free_2023} in FedLQR, the per-agent sample requirement improves from $\mathcal{O}(1/\epsilon^2)$ to $\mathcal{O}(1/(M\epsilon^2))$ by leveraging independent gradient noise across agents, and learning a policy that optimizes the average performance across the fleet.

% In practice, for a drone, generating each sample means interrupting a
% surveillance mission for an exploratory maneuver while burning battery;
% for a power grid controller, it means applying a perturbed input that
% stresses transformer insulation; for a robotic arm, it means measurable
% production downtime. This is what makes reducing sample complexity not merely a theoretical desideratum but a practical necessity for continuous, live deployment of model-free control.

% An interesting avenue exists for reducing sampling cost in large-scale multi-agent operations. When a fleet of $M$ agents with \emph{distinct but similar} dynamics\footnote{In many practical deployments---drone swarms, robotic fleets, or networks of industrial controllers---agents are nominally identical but exhibit slightly distinct dynamics due to manufacturing tolerances, actuator wear, or environmental calibration differences.} can pool their trajectory information, each agent's per-round sampling burden reduces by a factor of $M$. This is the central insight formalized by Wang et al.~\cite{wang_model-free_2023} in the FedLQR framework, which proves that the required sample size per agent decreases from $\mathcal{O}(1/\epsilon^2)$ to $\mathcal{O}(1/(M\epsilon^2))$, a factor-of-$M$ reduction achieved by exploiting the conditional independence of ZO gradient noise across distinct agents (Lemma~4 of \cite{wang_model-free_2023}). The result is striking: consider a fleet of $M = 1000$ robots, each of which would require $1000$ trajectory rollouts per gradient step operating alone; under FedLQR, the same gradient accuracy is achieved with only a single rollout per agent per round.

Despite offering a compelling foundation for collaborative
model-free LQR, two concerns yet arise when deploying FedLQR of~\cite{wang_model-free_2023}  at scale. First, requiring all $M$ agents to collect samples each round forces continuous exploration, even when local conditions make deviation unsafe. Second, each agent must transmit a full gradient matrix ($\Delta^{(i)} \in \mathbb{R}^{n_u \times n_x}$ with an uplink cost of $\mathcal{O}(n_u n_x)$ per agent per round), 
leading to a total server-side burden of $\mathcal{O}(M d)$ with $d = n_u n_x$. This communication cost grows with both fleet size and system dimension—precisely where large-scale collaboration is most beneficial.
The first issue is merely operational and can be mitigated within the federated framework \cite{qi_federated_2021}: since the per-agent sample complexity scales as $\mathcal{O}(1/(M\epsilon^2))$, only a subset of agents need participate each round. Others can remain idle—recharging or reallocating resources—while still receiving the updated policy $K_{t+1}$. The second issue, however, remains unresolved and worsens as $M$ increases. Moreover, transmitting full gradient matrices exposes sensitive information: each agent’s data implicitly encodes its local dynamics, enabling gradient inversion and system identification attacks~\cite{zhu_deep_2019}. Together, these concerns highlight the need for communication schemes with constant-size uplink and built-in structural privacy, decoupling transmission cost from system dimension while obscuring gradient geometry.



% Concretely, FedLQR requires each participating agent to upload
% its full gradient difference $\Delta^{(i)} \in \mathbb{R}^{n_u \times n_x}$,
% incurring an uplink cost of $\mathcal{O}(n_u n_x)$ per agent per round.
% The total server-side reception burden therefore scales as
% $\mathcal{O}(m \cdot d)$ where $d = n_u n_x$, growing quadratically with
% system dimension---precisely the regime where the sample-efficiency gains
% of large-$M$ collaboration are most attractive. 
% An additional consideration
% reinforces this need: each agent's trajectory data encodes its specific
% system matrices $(A^{(n)}, B^{(n)})$, which in many deployment contexts
% represent operationally sensitive characteristics. Transmitting full gradient
% matrices enables gradient inversion and system identification attacks,
% exposing local dynamics to the server. These two requirements---constant-size
% uplink and structural privacy---call for a communication mechanism that
% decouples transmission cost from system dimension while masking the gradient
% geometry by design.


We propose \textsc{ScalarFedLQR}, which resolves this tension by fundamentally compressing the uplink. Instead of transmitting the full gradient $\nabla J(K) \in \mathbb{R}^d$, We invoke the concept of the \emph{projected directional derivative}, which has been recently explored in optimization to reduce computational and memory costs in gradient-based learning~\cite{fournier2023can,silver2021learning,rostami2024projected}, as well as in zeroth-order optimization~\cite{nesterov2017random}, and adapt it to design a communication-efficient encoding mechanism for federated LQR. In this framework, each participating agent forms a local zeroth-order estimate $\widehat{\nabla}J(K)$, samples a random Rademacher direction $v \in {\pm1}^d$ using a shared pseudorandom generator, and uploads only the scalar projection $\langle v, \widehat{\nabla}J(K)\rangle$ together with the corresponding random seed (an integer). Using the received seeds, the server deterministically reconstructs the same directions $v$ and aggregates the scalar messages to form a global descent direction. This reduces per‑agent communication from $\mathcal{O}(d)$ to $\mathcal{O}(1)$ and the total server burden from $\mathcal{O}(Md)$ to $\mathcal{O}(M)$ for $M$ active agents, independent of system dimension. The resulting approximation error reflects both projection distortion and zeroth‑order estimation noise, capturing the joint effects of sample size, policy dimension, and fleet size.

We show that, under suitable conditions on $M$, $d$, and the local estimation error $\epsilon$, \textsc{ScalarFedLQR} achieves linear convergence to the average optimal policy:
\begin{thm}[Linear convergence—Informal]
Assume the average LQR cost satisfies standard regularity conditions (e.g., a Polyak--\L{}ojasiewicz condition with $\mu_c$ and locally Lipschitz condition with $L_c$) on a stabilizing $c$-sublevel set. If the local zeroth-order relative estimation errors are uniformly bounded by $\epsilon$ such that
\begin{gather*}
    \sqrt{\frac{(d-1)\log\!\bigl(2d/\delta\bigr)}{M}}
\Big(1 + \epsilon \Big) \lesssim \beta
\end{gather*}
for some $\beta \in (0,1)$
then, with an appropriate constant stepsize and a failure probability $\delta$, \textsc{ScalarFedLQR} the average cost gap decreases at a geometric rate \(
1-\frac{\mu_c(1-\beta)^2}{L_c(1+\beta)^2}\).
\end{thm}

This result reveals a favorable tradeoff unique to large federated fleets. While scalar projection introduces approximation error that depends on the policy dimension, this effect is mitigated through averaging across participating
agents. In particular, as the number of active agents $M$ grows relative to the
problem dimension $d$, the effective relative error decreases, so the stability
condition can be satisfied with a smaller admissible value of $\beta$. Since the allowable stepsize range
$
0<\eta<\frac{2(1-\beta)}{L_c(1+\beta)^2}
$
expands as $\beta$ becomes smaller, larger fleets permit larger stepsizes and therefore faster linear convergence, even in high-dimensional control problems. Conversely, when fewer agents participate or when local gradient estimates are noisy, a larger effective $\beta$ is needed to maintain stability, which forces more conservative updates. Thus, \textsc{ScalarFedLQR} exhibits a compounding advantage at scale: per-agent communication remains constant, while both stability and convergence improve as fleet size grows, effectively decoupling learning performance from system dimension.


The rest of the paper is organized as follows.  
\S II formulates the federated model-free LQR problem and introduces the stabilizing set and similarity assumptions.  
\S III presents the \textsc{ScalarFedLQR} algorithm and analyzes its stability and convergence properties, including high-probability bounds on the scalar-projection error and linear convergence under a PL condition.  
\S IV provides numerical experiments comparing \textsc{ScalarFedLQR} with FedLQR under varying levels of heterogeneity and communication budgets.  
\S V concludes the paper and outlines directions for future work. Due to page limit, the missing proofs are provided in the extended version this work \cite{MR-ST-SSK:26}.





\begin{comment}
We show that, under suitable conditions on $M$, $d$, and the local estimation error $\epsilon$, \textsc{ScalarFedLQR} achieves linear convergence to the average optimal policy with an appropriate stepsize:
\begin{thm}[Linear convergence—Informal]
Under 
\text{condition involving $M$,$d$, local gradient error $\epsilon$ and $\beta_t$} \textsc{ScalarFedLQR} converges to the average optimal policy at a linear rate of ( function of $\beta_t$).
\end{thm}%
This highlights the compounding advantage in large fleets. \st{depeding on the bound explain the tradeoff here.}

Moreover, since the server observes only the rank-one projection $vv^\top \widehat{\nabla}J(K)$, components in its null space remain hidden, providing structural privacy without explicit noise injection~\cite{rostami_fedscalar_2024}. Together, this enables continuous large-scale autonomy: heterogeneous agents contribute at most one trajectory per round—often none—while a shared stabilizing policy converges via lightweight scalar exchanges.


The rest of the paper is organized as follows: 
\end{comment}

==> intro6.tex <==
\section{Introduction}

Policy optimization (PO) is a promising paradigm for data-driven control~\cite{hu_toward_2023,talebi_policy_2026}. 
Despite nonconvexity, policy gradient (PG) methods enjoy global convergence guarantees in structured settings such as the linear quadratic regulator (LQR)~\cite{fazel_global_2018,bu_lqr_2019}. 
These properties make PO particularly attractive for large-scale autonomous systems, where accurate models are unavailable and controllers must be learned directly from interaction data.

In model-free LQR, policy gradients are commonly estimated using zeroth-order (ZO) methods that require multiple trajectory rollouts per update~\cite{malik_derivative-free_2019}. 
Since each rollout corresponds to a full execution on a physical system, sampling inefficiency directly translates into operational cost. 
Federated learning offers a principled mechanism to mitigate this burden by enabling multiple agents with similar dynamics to collaboratively learn a common policy while pooling their data. 
In particular, recent federated LQR methods show that averaging gradient estimates across $M$ agents reduces the required number of rollouts per agent by a factor of $M$, improving the per-agent sample complexity from $\mathcal{O}(1/\epsilon^2)$ to $\mathcal{O}(1/(M\epsilon^2))$~\cite{wang_model-free_2023}. 
This factor-$M$ reduction makes federated LQR a compelling approach for large fleets of resource-constrained systems.

Despite these gains in sample efficiency, existing federated LQR methods introduce a new bottleneck: communication. 
Current approaches require each agent to transmit full policy gradients or gain matrices at every communication round, resulting in uplink costs that scale with the policy dimension and server-side aggregation costs that grow with both system dimension and fleet size~\cite{mcmahan_communication-efficient_2017,konecny_federated_2016}. 
As a result, communication—not sampling—becomes the dominant limitation in large-scale deployments.

This paper addresses this challenge by proposing \emph{ScalarFedLQR}, a communication-efficient federated algorithm for model-free LQR control with heterogeneous agents. 
ScalarFedLQR builds on a decomposed projected gradient mechanism, in which each agent computes a local zeroth-order gradient estimate and communicates only a single scalar projection per round. 
The server aggregates these scalar messages to reconstruct a global descent direction, reducing the per-agent uplink communication cost from $\mathcal{O}(d)$ to $\mathcal{O}(1)$, independent of the policy dimension. 
The projected-gradient structure is inspired by related developments in directional and projected gradient methods in optimization~\cite{fournier2023can,silver2021learning,rostami2024projected,nesterov2017random}.

We show that this extreme communication compression preserves the core guarantees of federated LQR. 
Under standard stability and regularity conditions, all iterates remain within the common stabilizing set, and ScalarFedLQR converges linearly to the optimal average policy. 
Moreover, the approximation error introduced by scalar projection decreases with the number of participating agents, revealing a favorable scaling regime in large federated fleets.

The rest of the paper is organized as follows. 
Section~II formulates the federated model-free LQR problem and introduces the stabilizing set and similarity assumptions. 
Section~III presents the \textsc{ScalarFedLQR} algorithm. 
Section~IV establishes stability and convergence guarantees. 
Section~V reports numerical results, and Section~VI concludes the paper. 
Due to page limits, omitted proofs are provided in the extended version~\cite{MR-ST-SSK:26}.

==> intro7.tex <==
\section{Introduction}

Policy optimization (PO) is a promising paradigm for data-driven control~\cite{hu_toward_2023, talebi_policy_2026}. Despite nonconvexity, policy gradient (PG) methods enjoy global convergence in structured settings such as LQR~\cite{fazel_global_2018,bu_lqr_2019}. However, large-scale deployment on physical systems is constrained by two fundamental bottlenecks: (i) communication overload, as transmitting high-dimensional gradients under limited bandwidth becomes prohibitive and scales with fleet size~\cite{mcmahan_communication-efficient_2017, konevcny_federated_2016}; and (ii) sample inefficiency, since model-free PG requires $\mathcal{O}(1/\epsilon^2)$ trajectory rollouts per step—untenable in real-world operation~\cite{dean_sample_2020}. Recent work partially mitigates these challenges: \texttt{D2SPI} addresses homogeneous networks~\cite{alemzadeh_data-driven_2024}, while \texttt{FedLQR} extends to heterogeneous but similar agents~\cite{wang_model-free_2023}.

A central, often underemphasized limitation underlying these bottlenecks is the \emph{physical cost of each gradient sample}. In zeroth-order (ZO) model-free LQR~\cite{fazel_global_2018, malik_derivative-free_2019}, estimating $\nabla J(K)$ for $K \in \mathbb{R}^{n_u \times n_x}$ requires executing perturbed policies $\widehat{K}_s = K + U_s$, collecting trajectories, and averaging costs over $n_s$ perturbations via
\begin{equation}\label{eq:local-grad-estimate}
\textstyle \widehat{\nabla}J(K) = \frac{1}{n_s}\sum_{s=1}^{n_s}
\frac{n_x n_u}{r^2} \widehat{J}_s U_s,
\end{equation}
where $\widehat{J}_s = J(\widehat{K}_s)$, achieving $\epsilon$-accurate gradients with $n_s = \mathcal{O}(1/\epsilon^2)$. Crucially, each “sample” is not a cheap computation but a full trajectory rollout of length $\tau$ on a live system~\cite{dulac-arnold_challenges_2019}. 
In practice, this cost is tangible: a drone must interrupt its mission and expend battery, a power grid controller applies perturbations that stress equipment, and a robotic arm incurs production downtime. Reducing sample complexity is therefore not merely theoretical but essential for safe, continuous deployment of learning-based control~\cite{mohammadi_learning_2020,zhao_global_2023,talebi_data-driven_2023,umenberger_globally_2022}. 
A key opportunity arises in large-scale multi-agent systems: when $M$ agents with similar (but not necessarily identical) dynamics pool trajectory data, the per-agent sampling burden decreases by a factor of $M$. As shown by Wang et al.~\cite{wang_model-free_2023} in \texttt{FedLQR}, the requirement improves from $\mathcal{O}(1/\epsilon^2)$ to $\mathcal{O}(1/(M\epsilon^2))$ by exploiting independent gradient noise across agents while optimizing average fleet performance.

% In practice, for a drone, generating each sample means interrupting a
% surveillance mission for an exploratory maneuver while burning battery;
% for a power grid controller, it means applying a perturbed input that
% stresses transformer insulation; for a robotic arm, it means measurable
% production downtime. This is what makes reducing sample complexity not merely a theoretical desideratum but a practical necessity for continuous, live deployment of model-free control.

% An interesting avenue exists for reducing sampling cost in large-scale multi-agent operations. When a fleet of $M$ agents with \emph{distinct but similar} dynamics\footnote{In many practical deployments---drone swarms, robotic fleets, or networks of industrial controllers---agents are nominally identical but exhibit slightly distinct dynamics due to manufacturing tolerances, actuator wear, or environmental calibration differences.} can pool their trajectory information, each agent's per-round sampling burden reduces by a factor of $M$. This is the central insight formalized by Wang et al.~\cite{wang_model-free_2023} in the FedLQR framework, which proves that the required sample size per agent decreases from $\mathcal{O}(1/\epsilon^2)$ to $\mathcal{O}(1/(M\epsilon^2))$, a factor-of-$M$ reduction achieved by exploiting the conditional independence of ZO gradient noise across distinct agents (Lemma~4 of \cite{wang_model-free_2023}). The result is striking: consider a fleet of $M = 1000$ robots, each of which would require $1000$ trajectory rollouts per gradient step operating alone; under FedLQR, the same gradient accuracy is achieved with only a single rollout per agent per round.

% Despite offering a compelling foundation for collaborative
% model-free LQR, two concerns yet arise when deploying FedLQR of~\cite{wang_model-free_2023}  at scale. First, requiring all $M$ agents to collect samples each round forces continuous exploration, even when local conditions make deviation unsafe. Second, each agent must transmit a full gradient matrix ($\Delta^{(i)} \in \mathbb{R}^{n_u \times n_x}$ with an uplink cost of $\mathcal{O}(n_u n_x)$ per agent per round), 
% leading to a total server-side burden of $\mathcal{O}(M d)$ with $d = n_u n_x$. This communication cost grows with both fleet size and system dimension—precisely where large-scale collaboration is most beneficial.
% The first issue is merely operational and can be mitigated within the federated framework \cite{qi_federated_2021}: since the per-agent sample complexity scales as $\mathcal{O}(1/(M\epsilon^2))$, only a subset of agents need participate each round. Others can remain idle—recharging or reallocating resources—while still receiving the updated policy $K_{t+1}$. The second issue, however, remains unresolved and worsens as $M$ increases. Moreover, transmitting full gradient matrices exposes sensitive information: each agent’s data implicitly encodes its local dynamics, enabling gradient inversion and system identification attacks~\cite{zhu_deep_2019}. Together, these concerns highlight the need for communication schemes with constant-size uplink and built-in structural privacy, decoupling transmission cost from system dimension while obscuring gradient geometry.


Despite its strengths, \texttt{FedLQR} faces two limitations at scale. First, requiring all $M$ agents to sample each round enforces continuous exploration, though this can be mitigated by subsampling since per-agent sample complexity already scales as $\mathcal{O}(1/(M\epsilon^2))$\cite{qi_federated_2021}. Second, and more fundamentally, each agent must transmit a full gradient matrix $\Delta^{(i)} \in \mathbb{R}^{n_u \times n_x}$, incurring $\mathcal{O}(d)$ uplink cost and a total server burden of $\mathcal{O}(Md)$ with $d=n_u n_x$. This cost grows with both fleet size and system dimension—precisely where collaboration is most valuable—and additionally exposes sensitive local dynamics through gradient inversion attacks\cite{zhu_deep_2019}. These limitations motivate our approach: achieving constant-size uplink with built-in structural privacy, decoupling communication from system dimension while retaining guaranteed fast federated learning and iterative stability.
% \reza{we have privacy here, should we keep it?}


% Concretely, FedLQR requires each participating agent to upload
% its full gradient difference $\Delta^{(i)} \in \mathbb{R}^{n_u \times n_x}$,
% incurring an uplink cost of $\mathcal{O}(n_u n_x)$ per agent per round.
% The total server-side reception burden therefore scales as
% $\mathcal{O}(m \cdot d)$ where $d = n_u n_x$, growing quadratically with
% system dimension---precisely the regime where the sample-efficiency gains
% of large-$M$ collaboration are most attractive. 
% An additional consideration
% reinforces this need: each agent's trajectory data encodes its specific
% system matrices $(A^{(n)}, B^{(n)})$, which in many deployment contexts
% represent operationally sensitive characteristics. Transmitting full gradient
% matrices enables gradient inversion and system identification attacks,
% exposing local dynamics to the server. These two requirements---constant-size
% uplink and structural privacy---call for a communication mechanism that
% decouples transmission cost from system dimension while masking the gradient
% geometry by design.


% In this paper, we propose \textsc{ScalarFedLQR}, which resolves this tension by fundamentally compressing the uplink. Instead of transmitting the full gradient $\nabla J(K) \in \mathbb{R}^d$, We invoke the concept of the \emph{projected directional derivative}, which has been recently explored in optimization to reduce computational and memory costs in gradient-based learning~\cite{fournier2023can,silver2021learning,rostami2024projected}, as well as in zeroth-order optimization~\cite{nesterov2017random}, and adapt it to design a communication-efficient encoding mechanism for federated LQR. In this framework, each participating agent forms a local zeroth-order estimate $\widehat{\nabla}J(K)$, samples a random Rademacher direction $v \in {\pm1}^d$ using a shared pseudorandom generator, and uploads only the scalar projection $\langle v, \widehat{\nabla}J(K)\rangle$ together with the corresponding random seed (an integer). Using the received seeds, the server deterministically reconstructs the same directions $v$ and aggregates the scalar messages to form a global descent direction. This reduces per‑agent communication from $\mathcal{O}(d)$ to $\mathcal{O}(1)$ and the total server burden from $\mathcal{O}(Md)$ to $\mathcal{O}(M)$ for $M$ active agents, independent of system dimension. The resulting approximation error reflects both projection distortion and zeroth‑order estimation noise, capturing the joint effects of sample size, policy dimension, and fleet size.

We propose \textsc{ScalarFedLQR}, which resolves this tension by compressing the uplink via \emph{projected directional derivatives}. Rather than transmitting the full gradient $\nabla J(K) \in \mathbb{R}^d$, each participating agent computes a local zeroth-order estimate $\widehat{\nabla}J(K)$, samples a Rademacher direction $v \in {\pm1}^d$ using a shared pseudorandom generator, and sends only the scalar projection $\langle v, \widehat{\nabla}J(K)\rangle$ along with the seed. The server reconstructs $v$ deterministically from the seed and aggregates these scalar messages to obtain a global descent direction. This reduces per-agent communication from $\mathcal{O}(d)$ to $\mathcal{O}(1)$ and total server cost from $\mathcal{O}(Md)$ to $\mathcal{O}(M)$ for $M$ active agents, independent of system dimension. The induced error decomposes into projection distortion and zeroth-order estimation noise, jointly governed by sample size, dimension, and fleet size~\cite{fournier2023can,silver2021learning,rostami2024projected,nesterov2017random}.

Under standard regularity conditions on the average LQR cost (e.g., a Polyak–\L{}ojasiewicz condition with constant $\mu_c$ and local Lipschitz continuity with $L_c$ over a stabilizing sublevel set), we establish linear convergence:

\smallskip
\noindent\textbf{Theorem. }(Linear convergence—Informal)
\emph{If the local zeroth-order relative errors are bounded by $\epsilon$ and
\[\textstyle d \, \log(2d/\delta) \, M^{-1} \,(1+\epsilon)^2 \lesssim \beta^2 \quad \text{for some } \beta \in (0,1),\]
then, with a suitable constant stepsize and probability at least $1-\delta$, \textsc{ScalarFedLQR} achieves geometric decay of the average cost at rate
$1 - (\mu_c/L_c){(1-\beta)^2}/{(1+\beta)^2}.$\boxend}
\smallskip

\noindent This result highlights a key large-scale advantage: although scalar projection introduces dimension-dependent error, averaging across agents reduces its impact as $M$ grows. Consequently, larger fleets admit smaller $\beta$, enabling larger stepsizes and faster linear convergence—even in high dimensions. In contrast, smaller or noisier settings require more conservative updates. Thus, \textsc{ScalarFedLQR} achieves a compounding benefit at scale: scalar per-agent communication with improving stability and convergence as fleet size increases.

The rest of the paper is organized as follows.  
\S II formulates the federated model-free LQR problem and introduces the stabilizing set and similarity assumptions.  
\S III presents the \textsc{ScalarFedLQR} algorithm and \S IV analyzes its stability and convergence properties, including high-probability bounds on the scalar-projection error and linear convergence under a PL condition.  
\S V provides numerical experiments comparing \textsc{ScalarFedLQR} with \texttt{FedLQR} under varying levels of heterogeneity and communication budgets.  
\S VI concludes the paper and outlines directions for future work. 
% Due to page limit, the missing proofs are provided in the extended version this work \cite{MR-ST-SSK:26}.





\begin{comment}
We show that, under suitable conditions on $M$, $d$, and the local estimation error $\epsilon$, \textsc{ScalarFedLQR} achieves linear convergence to the average optimal policy with an appropriate stepsize:
\begin{thm}[Linear convergence—Informal]
Under 
\text{condition involving $M$,$d$, local gradient error $\epsilon$ and $\beta_t$} \textsc{ScalarFedLQR} converges to the average optimal policy at a linear rate of ( function of $\beta_t$).
\end{thm}%
This highlights the compounding advantage in large fleets. \st{depeding on the bound explain the tradeoff here.}

Moreover, since the server observes only the rank-one projection $vv^\top \widehat{\nabla}J(K)$, components in its null space remain hidden, providing structural privacy without explicit noise injection~\cite{rostami_fedscalar_2024}. Together, this enables continuous large-scale autonomy: heterogeneous agents contribute at most one trajectory per round—often none—while a shared stabilizing policy converges via lightweight scalar exchanges.


The rest of the paper is organized as follows: 
\end{comment}

==> intro8.tex <==
\section{Introduction}

Policy optimization (PO) is a promising paradigm for data-driven control of
cyber-physical systems (CPS)~\cite{hu_toward_2023, talebi_policy_2026}.
Despite nonconvexity, policy gradient (PG) methods enjoy global convergence
in structured settings such as LQR~\cite{fazel_global_2018, bu_lqr_2019}.
\added{A central bottleneck in deploying such methods on physical systems is
the cost of each gradient sample.}
In zeroth-order (ZO) model-free LQR~\cite{fazel_global_2018,
malik_derivative-free_2019}, estimating $\nabla J(K)$ for
$K \in \mathbb{R}^{n_{u} \times n_{x}}$ requires executing perturbed
rollouts $\widehat{K}_{s} = K + U_{s}$ and averaging costs over $n_{s}$
trajectories via \margin{let's update this discussion here to also include the improved oracles with $1/\epsilon$ complexity using the two point estimate, reduced variance using baseline and... ----( and the stepsize is missing}
\begin{equation}\label{eq:zo-grad}
  \textstyle
  \widehat{\nabla}J(K) = \frac{1}{n_{s}}\sum_{s=1}^{n_{s}}
  \frac{n_{x}n_{u}}{r^{2}}\,\widehat{J}_{s}\,U_{s},
\end{equation}
where $\widehat{J}_{s} = J(\widehat{K}_{s})$, achieving $\epsilon$-accurate
gradients with $n_{s} = \mathcal{O}(1/\epsilon^{2})$~\cite{dean_sample_2020}.
Each sample corresponds to a full trajectory rollout of length $\tau$ on a
live system~\cite{dulac-arnold_challenges_2019}: a drone must interrupt its
mission and expend battery, a grid controller applies perturbations that
stress equipment, and a robotic arm incurs production downtime.
\added{Reducing this per-agent rollout burden is therefore not merely a
theoretical concern but a practical requirement for safe, continuous
deployment of learning-based control~\cite{mohammadi_learning_2020,
zhao_global_2023, talebi_data-driven_2023, umenberger_globally_2022}.
In large-scale multi-agent CPS, cooperation offers a principled path toward
this goal: when $M$ agents with similar but not necessarily identical
dynamics execute independent rollouts and share information, the per-agent
sample complexity improves from $\mathcal{O}(1/\epsilon^{2})$ to
$\mathcal{O}(1/(M\epsilon^{2}))$, as shown in \texttt{FedLQR}~\cite{wang_model-free_2023}
by exploiting statistical independence of gradient noise across agents while
optimizing a common fleet-level performance objective.
This reduction is consequential precisely because each rollout carries a
tangible physical cost: pooling data across $M$ agents amortizes that cost
by a factor of $M$, making model-free LQR tractable at fleet scale.} \margin{let's report this factor M improvement more modular given any gradient oracle.}

\added{Cooperation, however, demands communication, and in realistic CPS
deployments communication channels are unreliable.
Two impairments are fundamental: \emph{message dropout}, where packets are
lost due to link failure, congestion, or interference; and \emph{channel
noise}, which corrupts transmitted values.
Both are acutely damaging when agents transmit high-dimensional gradient
matrices $\Delta^{(i)} \in \mathbb{R}^{n_{u} \times n_{x}}$, as in
\texttt{FedLQR}~\cite{wang_model-free_2023}: a single dropped packet
destroys $\mathcal{O}(d)$ bits of gradient information ($d = n_{u}n_{x}$),
and channel noise can deflect the entire descent direction, threatening
stability of the learning process.
Beyond reliability, high-dimensional transmissions also expose sensitive local
dynamics to gradient inversion attacks~\cite{zhu_deep_2019}.
These are not peripheral concerns; they are fundamental barriers to deploying
cooperative learning over real communication infrastructure.}

\added{We propose a different perspective: \emph{scalar directional
derivatives as a resilience mechanism for cooperative LQR}.
Reducing each agent's uplink to a single real number---a directional
derivative of its local gradient estimate along a shared random
direction---unlocks two resilience properties unavailable to high-dimensional
schemes.
\emph{(i) Dropout robustness via retransmission.}
A scalar message can be retransmitted multiple times within the same
communication budget.
Because each transmission is independent, the probability that at least one
copy is delivered grows with the number of redundant sends, converting a
fragile single-packet protocol into a robust multi-send one at negligible
extra cost.
\emph{(ii) Noise suppression via averaging.}
When multiple noisy copies of the same scalar arrive, averaging them directly
reduces channel noise in the gradient signal---a benefit that cannot be
obtained from a single high-dimensional vector without a dedicated
error-correction layer.
Both properties are enabled precisely by scalar structure: projecting onto a
Rademacher direction $v \in \{\pm 1\}^{d}$ collapses $\mathcal{O}(d)$
information to a single number that is cheap to retransmit and easy to
average, yet whose projection error diminishes as fleet size $M$
grows---exactly the regime where cooperation is most valuable.
Directional derivatives thus serve as the structural bridge between
communication resilience and cooperative learning efficiency.} \margin{why Rademacher directions? is it statistically optimal in some sense?]][\
}

We propose \textsc{ScalarFedLQR}, which realizes this resilient cooperative
scheme.
Rather than transmitting the full gradient $\nabla J(K) \in \mathbb{R}^{d}$,
each participating agent computes a local ZO estimate
$\widehat{\nabla}J(K)$, samples a Rademacher direction
$v \in \{\pm 1\}^{d}$ via a shared pseudorandom generator, and sends only
the scalar projection $\langle v, \widehat{\nabla}J(K)\rangle$ along with
the seed.
\added{The scalar nature of this message enables retransmission at negligible
overhead: under dropout, multiple copies increase delivery probability; under
channel noise, received copies are averaged before server aggregation,
directly suppressing noise in the gradient signal.}
The server reconstructs $v$ deterministically from the seed and aggregates
the received scalars into a global descent direction.
This reduces per-agent uplink from $\mathcal{O}(d)$ to $\mathcal{O}(1)$
and total server cost from $\mathcal{O}(Md)$ to $\mathcal{O}(M)$,
independent of system dimension.
The induced error decomposes into projection distortion and ZO estimation
noise, jointly governed by sample size, dimension, and fleet
size~\cite{fournier2023can, silver2021learning, rostami2024projected,
nesterov2017random}.

Under standard regularity conditions on the average LQR cost
(Polyak--\L{}ojasiewicz constant $\mu_{c}$, Lipschitz smoothness $L_{c}$
over a stabilizing sublevel set), we establish linear convergence:

\margin{before this summary of linear convergence we need to settle the challenge with heterogeneity. Also, the way it is stated it is not clear how the communication constraints/effects are coming into the picture}
\smallskip
\noindent\textbf{Theorem.}~(Linear convergence---Informal)
\emph{If the local ZO relative errors are bounded by $\epsilon$ and
\[
  \textstyle
  d\,\log(2d/\delta)\,M^{-1}(1+\epsilon)^{2} \lesssim \beta^{2}
  \quad \text{for some } \beta \in (0,1),
\]
then, with a suitable constant stepsize and probability at least $1-\delta$,
\textsc{ScalarFedLQR} achieves geometric cost decay at rate
$1-(\mu_{c}/L_{c})(1-\beta)^{2}/(1+\beta)^{2}$.}\hfill$\square$
\smallskip

\noindent
This result highlights the compounding benefit of scale: although scalar
projection introduces dimension-dependent error, averaging across $M$ agents
reduces its impact as the fleet grows, admitting smaller $\beta$, larger
stepsizes, and faster convergence even in high dimensions.
\added{Crucially, the same scalar structure that drives this scaling also
supports retransmission and noise averaging, so resilience to channel
impairments and convergence speed reinforce one another as $M$ increases.}
Thus, \textsc{ScalarFedLQR} turns communication-channel adversity from a
learning obstacle into a solvable design parameter.

The rest of the paper is organized as follows.
\S\ref{sec:problem} formulates the federated model-free LQR problem and
introduces the stabilizing set and similarity assumptions.
\S\ref{sec:algorithm} presents the \textsc{ScalarFedLQR} algorithm,
\added{including the retransmission and noise-averaging communication
protocol,} and \S\ref{sec:analysis} analyzes its stability and convergence,
including high-probability bounds on the scalar-projection error and linear
convergence under a PL condition.
\S\ref{sec:numerics} provides numerical experiments comparing
\textsc{ScalarFedLQR} with \texttt{FedLQR} under varying heterogeneity and
communication budgets.
\S\ref{sec:conclusion} concludes and outlines directions for future work.


==> intro9.tex <==
\section{Introduction}

\IEEEPARstart{P}{olicy} optimization has emerged as a practical route to
data-driven control: the controller is parameterized directly, and its
parameters are updated from the cost observed on the closed-loop
system~\cite{hu_toward_2023,talebi_policy_2026}. Despite the nonconvexity
of the resulting problem, policy gradient (PG) methods converge to the
global optimum in structured settings such as the linear quadratic
regulator (LQR)~\cite{fazel_global_2018,bu_lqr_2019}, which makes LQR the
natural benchmark for understanding what data-driven control costs. That
cost is not computational. In model-free PG, the gradient is estimated
by running the system under randomly perturbed gains and recording the
resulting costs~\cite{fazel_global_2018,malik_derivative-free_2019}, and
every such evaluation is a trajectory rollout on the physical
plant~\cite{dulac-arnold_challenges_2019}. The number of rollouts needed
for an $\epsilon$-accurate gradient depends on the oracle, from order
$1/\epsilon^2$ for one-point estimators to order $1/\epsilon$ for
two-point estimators~\cite{malik_derivative-free_2019}, but it is never
small.\margin{cite variance-reduced / baseline oracles if desired} For a drone, a rollout is a
detour from its mission and a draw on its battery; for a grid
controller, it is a perturbation that stresses equipment; for a robotic
arm, it is production downtime. This is the essential difference from
federated learning of statistical models, where a sample is a
computation on stored data and the binding constraint is
communication~\cite{mcmahan_communication-efficient_2017,konevcny_federated_2016}.
In learning-based control, the binding constraint is the energy and
time spent generating data on the plant.

Cooperation offers a principled way to share that burden. When $M$
agents with similar dynamics pool their rollouts to learn a common gain,
the estimation noise, which is independent across agents, averages out,
and whatever the oracle, the rollouts each agent must contribute drop by
a factor of $M$~\cite{ren_federated_2020,wang_model-free_2023}. This
reduction is what makes model-free control viable at fleet scale, and it
is the premise of federated LQR. It rests, however, on
communication: each round, every agent must send its local gradient
estimate to a server and receive the updated gain in return.

The same physical constraints that make rollouts expensive make this
communication unreliable. A small, battery-powered platform has limited
transmit power and bandwidth and low-cost radio hardware; its uplink is
subject to packet loss and additive noise, and every bit it sends costs
energy that competes with its mission. Existing federated LQR
schemes~\cite{wang_model-free_2023,alemzadeh_data-driven_2024} treat
the channel as ideal and transmit the full gradient, a vector of
dimension $d=n_un_x$. Over a real uplink, this is fragile in a specific
way. Channel noise corrupts all $d$ coordinates of the message at once
and deflects the descent direction; a single lost packet discards the
agent's entire contribution for that round; and the natural remedy,
retransmission, multiplies a cost that already scales with $d$. Worse,
the damage is not confined to slower convergence. In model-free control
the iterates are deployed on the plant as they are computed, so an
update corrupted by the channel can push the common gain outside the
set that stabilizes every agent. The gains that cooperation buys in
sample complexity can thus be returned, with interest, by the channel
through which cooperation happens.

This paper addresses that tension. Its starting point is the
observation that the uplink and downlink are asymmetric: the server is
provisioned and grid-powered, and broadcasting one gain matrix is cheap,
whereas each agent pays for its uplink in energy and airtime, over a
radio whose bandwidth is fixed by its hardware. Reliable learning must
therefore work within that bandwidth: the redundancy needed to
compensate for noise and dropout cannot be bought with more bits per
round, only with a better use of the bits the agent already has. The
question is what to put in those bits, and our answer is to change the
message rather than the channel. The solution we propose is to change the message rather than the
channel. Instead of its gradient estimate, each agent sends scalar
directional derivatives of that estimate along random directions
generated from a seed shared with the server. A scalar message has two
properties that a $d$-dimensional one lacks. It can be retransmitted
many times within the same budget, so the probability that at least one
copy survives dropout grows with the number of sends, turning a fragile
single-packet protocol into a robust multi-send one at negligible extra
cost. And when several noisy copies arrive, averaging them suppresses
channel noise in the gradient signal directly, without an
error-correction layer. Under a fixed uplink budget, an agent can
therefore transmit many independent scalars in place of a few copies of
a $d$-dimensional vector, and the server can recover a descent direction
from whatever subset of them arrives. The number of scalar
transmissions per round becomes a single design parameter that trades
uplink cost for resilience, turning the channel from an obstacle to
learning into a quantity that can be designed.

\emph{Related Work:} Policy gradient methods for LQR have been analyzed
in the model-based and model-free settings, establishing gradient
domination, iterate stability, and sample complexity
bounds~\cite{fazel_global_2018,malik_derivative-free_2019,mohammadi_convergence_2021,bu_lqr_2019,hu_toward_2023,talebi_policy_2026}.
Cooperative extensions include distributed policy iteration for
homogeneous networks~\cite{alemzadeh_data-driven_2024}, federated LQR
tracking for identical dynamics~\cite{ren_federated_2020}, and
\textsc{FedLQR}~\cite{wang_model-free_2023}, which handles similar but
heterogeneous agents and quantifies both the sample-complexity gain of
cooperation and the cost of heterogeneity. All of these assume
noiseless, lossless communication. In federated learning of statistical
models, communication is reduced by local updates, sparsification, or
quantization~\cite{mcmahan_communication-efficient_2017,konevcny_federated_2016},%
\margin{add 2--3 compression refs (e.g., Alistarh QSGD, Stich sparsified SGD, Bernstein signSGD)}
and the effect of noisy or lossy channels on convergence has been studied
for over-the-air aggregation and unreliable
clients;\margin{add 2--3 refs on FL over noisy/unreliable channels}
these analyses concern the optimization error of a statistical model and
do not address stability of a physical system during learning.
Directional derivatives along random directions have been used to
reduce computation and memory in gradient-based
learning~\cite{fournier2023can,silver2021learning,rostami2024projected},
in zeroth-order optimization~\cite{nesterov2017random}, and, in our
earlier work, as a communication primitive for federated learning of
statistical models~\cite{rostami_fedscalar_2024}, where the choice of
direction distribution was shown to affect the variance of the
reconstruction. We use Rademacher directions: their fixed norm gives the
smallest reconstruction variance among isotropic directions with the
same second moment, and they are reproduced exactly from an integer
seed.\margin{check: variance $(d-1)\|g\|^2$ for fixed norm vs.\ $(d+1)\|g\|^2$ for Gaussian} A preliminary
conference version of the present paper~\cite{MR-ST-SSK:26} introduced
scalar communication for federated LQR over an ideal channel and
analyzed homogeneous agents. The present paper treats the uplink as it
is: bandwidth-limited, noisy, and lossy.

\emph{Contribution:} We propose \textsc{ResiFedLQR}, a federated
model-free LQR algorithm in which each agent sends $N_{\rm sc}$ scalar
directional derivatives of its local gradient estimate over an uplink
with packet dropout and additive noise. Our contributions are:
\begin{itemize}
\item We show that all iterates of \textsc{ResiFedLQR} stabilize every
agent and that the fleet-average cost converges linearly to a
neighborhood of its optimum. The neighborhood has three parts with
different costs of removal: a heterogeneity floor, which we derive from
the similarity of the agents rather than assume; a rollout floor, set by
the accuracy of the local gradient estimates; and a communication floor.
\item We show that every communication-induced term, in the stability
condition, the admissible stepsize, the rate, and the floor, is governed
by a single quantity: the policy dimension divided by the expected
number of scalars the server receives per round. Increasing
$N_{\rm sc}$ or the fleet size $M$ shrinks it, so a fixed uplink budget
converts directly into resilience, and larger fleets need fewer
transmissions per agent.
\item We compare with full-gradient transmission over the same channel
and budget. Scalar communication reduces the channel-noise contribution
to the floor by a factor of $\sqrt d$ and increases the fraction of
agents whose messages survive dropout, at the price of a dimension-free
relative error that affects only the rate. This is why
\textsc{ResiFedLQR} remains stabilizing in noise and dropout regimes
where full-gradient transmission does not, which we confirm numerically
through empirical stability regions over stepsize, dropout probability,
and noise level.
\end{itemize}

\emph{Outline:} Section~\ref{sec:prob_def_object} formulates the
federated LQR problem and the uplink model. Section~\ref{sec:scalar}
introduces scalar gradient encoding, and Section~\ref{sec:resifedlqr}
presents \textsc{ResiFedLQR}. Section~\ref{sec:analysis} establishes
stability and convergence and discusses the roles of heterogeneity,
noise, dropout, and $N_{\rm sc}$. Section~\ref{sec:numerics} reports
numerical experiments, and Section~\ref{sec:conclusion} concludes.

==> stability0.tex <==
\section{Stability Analysis and Convergence of
\textsc{ResiFedLQR}}\label{sec:analysis}

This section presents the  the stability and convergence analysis of
Algorithm~\ref{alg:nc_scalarfedlqr_inline}. For technical
reasons that become clear below, the analysis is restricted
to the $c$-sublevel set $
  \mathcal{S}_c := \{K : J_{\rm avg}(K)\le c\}, $
which contains the initial gain $K_0$ and is contained in
the common stabilizing set $\mathcal{S}$ when $Q\succ 0$
and $R\succ 0$. Our goal is to show that, under suitable
stepsize and gradient-error conditions, the iterates generated
by Algorithm~\ref{alg:nc_scalarfedlqr_inline} remain in
$\mathcal{S}_c$ and converge toward a minimizer of the
average cost. 

Relative to an idealized \textsc{FedLQR} setting with perfect communication, the server in \textsc{ResiFedLQR} does not directly receives the local gradient estimates $\tilde g_{t,n}$. Instead, under the uplink model of Assumption~\ref{assump:noise}, it must reconstruct a descent direction from noisy scalar directional projections received from a random subset of agents. As a result, in addition to the zeroth-order gradient-estimation error, the server-side update direction deviates from the true gradient through three more distinct mechanisms: (i) scalar reconstruction error arising from the finite number of random directions, (ii) channel-noise error induced by the additive uplink corruption, and (iii) client-activation error caused by averaging only over the active set $\mathcal{A}_t$. The dropout probability $p_{\rm drop}$ affects the analysis through the random received counts $N_{t,n}^{\rm rec}$ and the resulting active-client set $\mathcal A_t$. The central goal of the analysis is therefore to quantify these error sources, establish conditions under which their combined effect remains sufficiently small relative to the true gradient, and characterize how the design parameter $N_{\rm sc}$ trades communication cost for statistical accuracy, dropout resilience, stability margin, and convergence speed.

\medskip
We begin by making the mathematical structure of
Algorithm~\ref{alg:nc_scalarfedlqr_inline}'s output
explicit, as this decomposition underlies every subsequent
result. The decoded direction for each active client at the server is
\begin{align}\label{eq:client_decode_dropout}
  \widehat{g}_{t,n}
  =\frac{1}{N_{t,n}^{\rm rec}}
  \sum\nolimits_{s\in\mathcal{R}_{t,n}}
  y_{n,s}^t\,v_{t,n,s},
  \qquad n\in\mathcal{A}_t,
\end{align}
and the server aggregate is
\begin{align}\label{eq:resifed_noisy_direction_dropout}
  \widehat{g}_t
  =\frac{1}{|\mathcal{A}_t|}
  \sum\nolimits_{n\in\mathcal{A}_t}\widehat{g}_{t,n}.
\end{align}
When there is no dropout, $\mathcal{A}_t=[M]$ and
$N_{t,n}^{\rm rec}=N_{\rm sc}$,
so~\eqref{eq:resifed_noisy_direction_dropout} reduces to
$\widehat{g}_t=\frac{1}{M}\sum_{n=1}^M\frac{1}{N_{\rm sc}}
\sum_{s=1}^{N_{\rm sc}}y_{n,s}^t\,v_{t,n,s}$.
Substituting $y_{n,s}^t=v_{t,n,s}^{\top}\tilde{g}_{t,n}
+w_{n,s}^t$ into~\eqref{eq:client_decode_dropout} gives
the client-side decomposition
\begin{align}\label{eq:client_decomposition_dropout}
  \widehat{g}_{t,n}
  =&\underbrace{
    \frac{1}{N_{t,n}^{\rm rec}}
    \sum\nolimits_{s\in\mathcal{R}_{t,n}}
    v_{t,n,s}v_{t,n,s}^{\top}\tilde{g}_{t,n}
  }_{\bar{g}_{t,n}}
 \, +\nonumber\\&~~~
  \underbrace{
    \frac{1}{N_{t,n}^{\rm rec}}
    \sum\nolimits_{s\in\mathcal{R}_{t,n}}
    w_{n,s}^t\,v_{t,n,s}
  }_{e_{t,n}^{\rm ch}},
  \quad n\in\mathcal{A}_t,
\end{align}
and therefore
\begin{align}\label{eq:server_decomposition_dropout}
  \widehat{g}_t = \bar{g}_t+e_t^{\rm ch},~
  \bar{g}_t:=\frac{1}{|\mathcal{A}_t|}
  \sum_{n\in\mathcal{A}_t}\bar{g}_{t,n},~
  e_t^{\rm ch}:=\frac{1}{|\mathcal{A}_t|}
  \sum_{n\in\mathcal{A}_t}e_{t,n}^{\rm ch}.
\end{align}
Here $\bar{g}_t$ is the clean scalar-reconstructed direction
from the received measurements and $e_t^{\rm ch}$ is the
reconstructed channel-noise error. For compact notation,
define
$
  V_{t,n}^{\rm rec}
  :=\bigl[v_{t,n,s}\bigr]_{s\in\mathcal{R}_{t,n}}
  \in\mathbb{R}^{d\times N_{t,n}^{\rm rec}},~
  y_{t,n}^{\rm rec}
  :=\bigl[y_{n,s}^t\bigr]_{s\in\mathcal{R}_{t,n}}
  \in\mathbb{R}^{N_{t,n}^{\rm rec}},$
  and $
  w_{t,n}^{\rm rec}
  :=\bigl[w_{n,s}^t\bigr]_{s\in\mathcal{R}_{t,n}}
  \in\mathbb{R}^{N_{t,n}^{\rm rec}},$
where $\mathcal{R}_{t,n}=\{s_1,\ldots,s_{N_{t,n}^{\rm rec}}\}$
is written in any fixed order. The channel observation
and client decode then read
$y_{t,n}^{\rm rec}=(V_{t,n}^{\rm rec})^{\top}\tilde{g}_{t,n}
+w_{t,n}^{\rm rec}$ and
\begin{align}\label{eq:vectorized_client_decode_dropout}
  \widehat{g}_{t,n}
  =&\frac{1}{N_{t,n}^{\rm rec}}V_{t,n}^{\rm rec}y_{t,n}^{\rm rec}\nonumber
 \\ =&\underbrace{
    \frac{1}{N_{t,n}^{\rm rec}}
    V_{t,n}^{\rm rec}(V_{t,n}^{\rm rec})^{\top}\tilde{g}_{t,n}
  }_{\bar{g}_{t,n}}
  +
  \underbrace{
    \frac{1}{N_{t,n}^{\rm rec}}
    V_{t,n}^{\rm rec}w_{t,n}^{\rm rec}
  }_{e_{t,n}^{\rm ch}}.
\end{align}
This decomposition preserves the client-wise averaging
structure of the algorithm under dropout. Dropout replaces
the deterministic count $N_{\rm sc}$ by the realized count
$N_{t,n}^{\rm rec}$ and the full client set $[M]$ by the
active set $\mathcal{A}_t$. Under independent per-scalar
dropout, $\mathbb{E}[N_{t,n}^{\rm rec}]=(1-p_{\rm drop})
N_{\rm sc}$ and $\mathbb{E}[|\mathcal{A}_t|]=M(1-p_{\rm
drop}^{N_{\rm sc}})$, so increasing $N_{\rm sc}$ enlarges
both the expected number of received scalars and the
expected active set, simultaneously improving scalar
reconstruction and channel-noise averaging.

\medskip
Next, let $g_t:=\nabla J_{\rm avg}(K_t)$ denote the exact
gradient and let $\tilde{g}_t:=\frac{1}{M}\sum_{n=1}^M
\tilde{g}_{t,n}$ denote the full average of the local
zeroth-order estimates:
\begin{align}\label{eq::zo_diff}
  g_t:=\nabla J_{\rm avg}(K_t),\qquad
  \tilde{g}_t:=\frac{1}{M}\sum\nolimits_{n=1}^M\tilde{g}_{t,n}.
\end{align}
Under dropout, the server aggregates only the active clients
$\mathcal{A}_t=\{n:N_{t,n}^{\rm rec}>0\}$. We therefore
also define the active-client ZO average
\begin{align}\label{eq:active_zo_average}
  \tilde{g}_t^{\mathcal{A}}
  :=\frac{1}{|\mathcal{A}_t|}
  \sum\nolimits_{n\in\mathcal{A}_t}\tilde{g}_{t,n},
  \qquad|\mathcal{A}_t|>0.
\end{align}
When there is no dropout, $\mathcal{A}_t=[M]$ and
$\tilde{g}_t^{\mathcal{A}}=\tilde{g}_t$.
From~\eqref{eq:server_decomposition_dropout}, the total
error between the server's update direction and the true
gradient is
\begin{align}\label{eq:total_error_resifed_dropout}
  e_t^{\rm tot}
  \!:=\!\widehat{g}_t-g_t
  =\underbrace{(\bar{g}_t-\tilde{g}_t^{\mathcal{A}})}_{e_t^{\rm proj}}
  +\underbrace{(\tilde{g}_t^{\mathcal{A}}-\tilde{g}_t)}_{e_t^{\rm drop}}
  +\underbrace{(\tilde{g}_t-g_t)}_{e_t^{\rm ZO}}
  +\!\!\!\!\!\underbrace{e_t^{\rm ch}}_{\!\!\!\!\!\!\!\!\text{channel noise}}\!\!\!\!\!.
\end{align}
Here $e_t^{\rm proj}$ is the scalar reconstruction error
over the received directions, $e_t^{\rm drop}$ is the
active-client dropout error, $e_t^{\rm ZO}$ is the
zeroth-order estimation error, and $e_t^{\rm ch}$ is the
reconstructed channel-noise error. Equivalently, grouping
all communication-layer errors as
$e_t^{\rm rec}:=\widehat{g}_t-\tilde{g}_t
=e_t^{\rm proj}+e_t^{\rm ch}+e_t^{\rm drop}$,
we write
\begin{align}\label{eq:total_error_resifed}
  e_t^{\rm tot}
  =\underbrace{(\widehat{g}_t-\tilde{g}_t)}_{e_t^{\rm rec}}
  +\underbrace{(\tilde{g}_t-g_t)}_{e_t^{\rm ZO}}.
\end{align}
If no scalar message is received in a round,
Algorithm~\ref{alg:nc_scalarfedlqr_inline} sets
$K_{t+1}=K_t$, so the cost does not increase. Otherwise,
the following results apply to the realized dropout and
channel-noise pattern.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\medskip
Our analysis relies on local smoothness and a local
Polyak--\L{}ojasiewicz (PL) condition for $J_{\rm avg}$
on $\mathcal{S}_c$.

\begin{assumption}[Local smoothness and local PL condition
on $\mathcal{S}_c$]\label{ass:pl}
There exist constants $L_c>0$ and $\mu_c>0$ such that for
all $K\in\mathcal{S}_c$,
\begin{equation}\label{eq:Lip}
  \|\nabla^2 J_{\rm avg}(K)\|_2\le L_c,
\end{equation}
\begin{equation}\label{eq:pl}
  \frac{1}{2}\|\nabla J_{\rm avg}(K)\|_2^2
  \ge\mu_c\bigl(J_{\rm avg}(K)-J_{\rm avg}^\star\bigr),
\end{equation}
where $J_{\rm avg}^\star:=\inf_{K\in\mathcal{S}_c}
J_{\rm avg}(K)$. \hfill$\square$
\end{assumption}

This assumption is known to hold in the homogeneous case \cite{talebi_policy_2026}, i.e., when $\epsilon_1=\epsilon_2=0$ in~\eqref{eq:system_bound}, provided $Q\succ0$ and $R\succ0$.
It is also expected to hold for sufficiently similar heterogeneous dynamics, but a detailed analysis is left for future work.\margin{this is tricky assertion,  building the paper based on a conjecture! cannot you explicitly show this or refer to FedLQR or other references?}

Referring to~\eqref{eq::zo_diff}, let $e_t^{\rm ZO}:=\tilde{g}_t-g_t$ and define the event $\mathcal{E}_t^{\rm ZO}:=\{\|e_t^{\rm ZO}\|_2\le\varepsilon\}$.
By Lemma~4 of~\cite{wang_model-free_2023}, this event can
be ensured with high probability under suitable sampling
parameters. It remains to control the communication-layer
error $e_t^{\rm rec}$. Unlike the zeroth-order error, which
comes from estimating local policy gradients through
rollouts, this error comes from reconstructing the averaged
zeroth-order gradient from noisy and intermittently received
scalar directional measurements. The next lemma gives a
high-probability bound on $\|e_t^{\rm rec}\|_2$. Combining
this with the zeroth-order event $\mathcal{E}_t^{\rm ZO}$
yields the total-error condition required by
Lemma~\ref{lem:federated_descent}. \margin{we should make this oracle condition precise, and also discuss the range of $\epsilon$ for which we can still handle the error.}

\begin{assumption}[Bounded gradient heterogeneity]
\label{ass:heterogeneity}
For each round $t$, let
$\Delta_{t,n}:=\tilde{g}_{t,n}-\tilde{g}_t$.
Assume there exist nonnegative quantities $\Gamma_t$ and
$B_t$ such that
\begin{align}
  \frac{1}{M}\sum\nolimits_{n=1}^{M}\|\Delta_{t,n}\|_2^2
  \le\Gamma_t^2,~
  \max_{1\le n\le M}\|\Delta_{t,n}\|_2\le B_t.
\end{align}
\hfill$\square$
\end{assumption} \margin{I'll be cautious about introducing this as an assumption; what does it mean for the agents? depending on what heterogeniety we are considering...}

Such bounded gradient heterogeneity assumptions are
standard in federated optimization~\cite{rostami2023federated}.
They quantify how much each client's local gradient estimate
can deviate from the full-client round average $\tilde{g}_t$.

\begin{lem}[One-step descent under scalar reconstruction,
dropout, and channel noise]\label{lem:federated_descent}
Fix $K_t\in\mathcal{S}_c$, let
$g_t:=\nabla J_{\rm avg}(K_t)\in\mathbb{R}^d$, and suppose
$|\mathcal{A}_t|>0$. Consider the update
$K_{t+1}=K_t-\eta\,\widehat{g}_t$,
where $\widehat{g}_t$ is the direction generated by
Algorithm~\ref{alg:nc_scalarfedlqr_inline}. Assume
$J_{\rm avg}$ is $L_c$-smooth on $\mathcal{S}_c$. If
$\|e_t^{\rm tot}\|_2\le\beta_t\|g_t\|_2$ for some
$\beta_t\in[0,1)$, with $e_t^{\rm tot}$ defined
in~\eqref{eq:total_error_resifed_dropout}, then
\begin{align}
  J_{\rm avg}(K_{t+1})
  \le J_{\rm avg}(K_t)
  -\eta\left[(1-\beta_t)-\frac{L_c\eta}{2}(1+\beta_t)^2
  \right]\|g_t\|_2^2.
  \label{eq:one_step_descent_beta}
\end{align}
Consequently, $J_{\rm avg}(K_{t+1})\le J_{\rm avg}(K_t)$
provided $0<\eta<\eta_{\max}:=2(1-\beta_t)/
(L_c(1+\beta_t)^2)$.
In particular, if $\beta_t\le\beta<1$ uniformly, a
sufficient uniform stepsize condition is
$0<\eta<2(1-\beta)/(L_c(1+\beta)^2)$.
Furthermore, with $\eta^\star=\eta_{\max}/2$,
\begin{align}
  J_{\rm avg}(K_{t+1})
  \le J_{\rm avg}(K_t)
  -\frac{(1-\beta_t)\eta_{\max}}{4}\|g_t\|_2^2.
  \label{eq:one_step_descent_eta_star}
\end{align}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:federated_descent}]
Since $J_{\rm avg}$ is $L_c$-smooth on $\mathcal{S}_c$,
\begin{align}
  J_{\rm avg}(K_{t+1})
  \le J_{\rm avg}(K_t)
  +\langle\nabla J_{\rm avg}(K_t),K_{t+1}-K_t\rangle
  \\ \nonumber+\frac{L_c}{2}\|K_{t+1}-K_t\|_2^2.
\end{align}
Using $g_t=\nabla J_{\rm avg}(K_t)$ and
$K_{t+1}=K_t-\eta\widehat{g}_t$,
\begin{align}
  J_{\rm avg}(K_{t+1})
  \le J_{\rm avg}(K_t)
  -\eta\langle g_t,\widehat{g}_t\rangle
  +\frac{L_c\eta^2}{2}\|\widehat{g}_t\|_2^2.
\end{align}
Writing $\widehat{g}_t=g_t+e_t^{\rm tot}$, applying
Cauchy--Schwarz and the triangle inequality, and using
$\|e_t^{\rm tot}\|_2\le\beta_t\|g_t\|_2$ yields the result.
Setting $\eta^\star=\eta_{\max}/2$ gives the
coefficient $(1-\beta_t)/2$, which
proves~\eqref{eq:one_step_descent_eta_star}.
\end{proof}

Lemma~\ref{lem:federated_descent} shows that $J_{\rm avg}$
decreases whenever $e_t^{\rm tot}$ is sufficiently small
relative to $\|g_t\|_2$. The parameter $\beta_t$
captures the admissible relative error in the server-side
update direction. To extend this to a full stability and
convergence guarantee, it remains to control
$e_t^{\rm rec}$.

\begin{rem}[Meaning of the relative-error parameter $\beta_t$] The parameter $\beta_t$ quantifies how accurately the server-side direction approximates the exact gradient. When $\beta_t=0$, the classical smooth-gradient descent stepsize bound $0<\eta<2/L_c$ is recovered. As $\beta_t$ increases, the admissible stepsize decreases, reflecting the fact that communication and estimation errors reduce the reliability of the descent direction. Consequently, improving gradient reconstruction directly enlarges the stability region of the algorithm. \end{rem}

\begin{lem}[High-probability bound for the noisy
reconstruction error under dropout]
\label{lem:hp_erec_resifed}
Fix a round $t$ with $|\mathcal{A}_t|>0$. Let
$q_{\rm sc}:=1-p_{\rm drop}$ and
$q_{\rm act}:=1-p_{\rm drop}^{N_{\rm sc}}$. Define
$\kappa_{\rm sc}:=\mathbb{E}[\mathbf{1}\{N_{t,n}^{\rm rec}
>0\}/N_{t,n}^{\rm rec}]$. Under
Assumptions~\ref{ass:heterogeneity} and~\ref{assump:noise},
for any $\delta\in(0,1)$, with probability at least
$1-\delta$,
\small
\begin{align}\label{eq:hp_erec_resifed}
  &\|e_t^{\rm rec}\|_2
  \le
  \underbrace{
    \!\frac{C\sqrt{M\kappa_{\rm sc}(d-1)\log(6d/\delta)}}
    {|\mathcal{A}_t|}
    \sqrt{\|\tilde{g}_t\|_2^2+\Gamma_t^2}
  }_{\text{projection error}}
  \\ \nonumber&+\!
  \underbrace{
    \frac{C\sqrt{M\kappa_{\rm sc}d\log(6d/\delta)}}
    {|\mathcal{A}_t|}\sigma_{\rm ch}
  }_{\text{channel-noise error}}
\!+
  \!\underbrace{
    \frac{C\sqrt{Mq_{\rm act}(1-q_{\rm act})
    \log(6d/\delta)}}{|\mathcal{A}_t|}\Gamma_t
  }_{\text{client-activation error}}
  \\ \nonumber &+
  \underbrace{
    \frac{C\log(6d/\delta)}{|\mathcal{A}_t|}
    \bigl[(d-1)(\|\tilde{g}_t\|_2+B_t)+B_t\bigr]
  }_{\text{lower-order Bernstein term}},
\end{align}
where $C>0$ is an absolute constant.
\end{lem}
The proof of Lemma~\ref{lem:hp_erec_resifed} is presented in the appendix.

\begin{rem}[Benefit of federation] The leading terms in~\eqref{eq:hp_erec_resifed} scale proportionally to $\sqrt{M}/|\mathcal A_t|$. When dropout is moderate, $|\mathcal A_t| \approx Mq_{\rm act}$, yielding an overall reconstruction error of order $1/\sqrt{M}$. Thus, increasing the number of participating agents improves not only statistical efficiency, as in classical federated learning, but also the accuracy of the scalar gradient reconstruction itself. \end{rem}

\begin{rem}[Role of dropout in the reconstruction bound]
The quantity $\kappa_{\rm sc}$ measures the effective
inverse number of received scalar samples. Since
$N_{t,n}^{\rm rec}\sim\mathrm{Binomial}(N_{\rm sc},
q_{\rm sc})$, splitting on the event
$N_{t,n}^{\rm rec}\ge q_{\rm sc}N_{\rm sc}/2$ and applying
a Chernoff bound gives
$\kappa_{\rm sc}\le 2/(q_{\rm sc}N_{\rm sc})
+\exp(-q_{\rm sc}N_{\rm sc}/8)$,
so $\kappa_{\rm sc}$ is of order $1/(q_{\rm sc}N_{\rm sc})$
when $q_{\rm sc}N_{\rm sc}$ is moderately large. In the
no-dropout case, $\kappa_{\rm sc}=1/N_{\rm sc}$ and
$q_{\rm act}=1$, recovering the usual
$1/\sqrt{MN_{\rm sc}}$-type scalar reconstruction scaling.
The term $q_{\rm act}(1-q_{\rm act})\Gamma_t^2$ captures
the additional error from random client activation; it
vanishes when all clients are active. \hfill$\square$
\end{rem}

We are now in a position to state the formal stability
guarantee. Combining Lemma~\ref{lem:federated_descent},
Assumption~\ref{ass:heterogeneity}, and the uniform
high-probability reconstruction bound from
Lemma~\ref{lem:hp_erec_uniform_T_resifed}, the following
theorem shows that the iterates remain in $\mathcal{S}_c$
provided the total direction error is uniformly controlled.

\begin{thm}[Stability of
\textsc{ResiFedLQR}]\label{thm:stability_resifed_fixed_beta}
Fix a horizon $T\ge 1$. Assume $K_0\in\mathcal{S}_c$ and
that for each round $t=0,\ldots,T-1$, whenever
$K_t\in\mathcal{S}_c$ and $|\mathcal{A}_t|>0$, the segment
$\{K_t-s\eta\widehat{g}_t:s\in[0,1]\}$ remains in
$\mathcal{S}_c$. Let $\mathcal{E}_T^{\rm ZO}:=
\bigcap_{t=0}^{T-1}\mathcal{E}_t^{\rm ZO}$. For every
active round, let $\zeta_t$ denote the right-hand side
of~\eqref{eq:hp_erec_uniformT_resifed}. Assume there exists
$\beta\in[0,1)$ such that
\begin{equation}\label{eq:fixed_beta_condition_resifed}
  \varepsilon+\zeta_t\le\beta\|g_t\|_2,
  \qquad\forall t=0,\ldots,T-1\ \text{with}\
  |\mathcal{A}_t|>0.
\end{equation}
If the stepsize satisfies
\begin{equation}\label{eq:fixed_stepsize_condition_resifed}
  0<\eta<\frac{2(1-\beta)}{L_c(1+\beta)^2},
\end{equation}
then, on $\mathcal{E}_T^{\rm ZO}$, with probability at
least $1-\delta$,
$J_{\rm avg}(K_{t+1})\le J_{\rm avg}(K_t)$ for
$t=0,\ldots,T-1$. Consequently, $K_t\in\mathcal{S}_c$
for $t=0,\ldots,T$, and all iterates are stabilizing.
\hfill$\square$
\end{thm}

\begin{proof}
By~\eqref{eq:total_error_resifed},
$e_t^{\rm tot}=e_t^{\rm rec}+e_t^{\rm ZO}$.
By Lemma~\ref{lem:hp_erec_uniform_T_resifed}, with
probability at least $1-\delta$,
$\|e_t^{\rm rec}\|_2\le\zeta_t$ simultaneously for all
active rounds. On $\mathcal{E}_T^{\rm ZO}$,
$\|e_t^{\rm ZO}\|_2\le\varepsilon$. Hence
$\|e_t^{\rm tot}\|_2\le\zeta_t+\varepsilon\le\beta\|g_t\|_2$
by~\eqref{eq:fixed_beta_condition_resifed}.
Lemma~\ref{lem:federated_descent} then
gives $J_{\rm avg}(K_{t+1})\le J_{\rm avg}(K_t)$ on every
active round. On inactive rounds $|\mathcal{A}_t|=0$, the
algorithm sets $K_{t+1}=K_t$. By induction,
$J_{\rm avg}(K_t)\le J_{\rm avg}(K_0)\le c$, so
$K_t\in\mathcal{S}_c\subseteq\mathcal{S}$ for all
$t=0,\ldots,T$.
\end{proof}


\begin{rem}[Comparison with full-gradient FedLQR] Theorem~\ref{thm:stability_resifed_fixed_beta} shows that stability depends on the aggregate direction error rather than on the communication protocol itself. The advantage of \textsc{ResiFedLQR} is therefore indirect: by allowing many more retransmissions within a fixed communication budget, it reduces the reconstruction term $\zeta_t$ and makes the stability condition \eqref{eq:fixed_beta_condition_resifed} easier to satisfy than under repeated full-gradient communication. \boxend\end{rem}

\subsection{Linear convergence under a PL condition}

Theorem~\ref{thm:stability_resifed_fixed_beta} establishes
that the iterates remain in $\mathcal{S}_c$ throughout the
horizon. Having secured this stability guarantee, we now
study convergence within $\mathcal{S}_c$. Combining
Lemma~\ref{lem:federated_descent} with the PL condition
on $J_{\rm avg}$, we obtain a linear convergence rate over
the active update rounds.

\begin{thm}[Linear convergence of
\textsc{ResiFedLQR}]\label{thm:pl_convergence_resifed}
Under the setup of
Theorem~\ref{thm:stability_resifed_fixed_beta}, assume
in addition that $J_{\rm avg}$ satisfies the PL condition in
Assumption~\ref{ass:pl} with parameter $\mu_c>0$. Let
$\eta^\star=(1-\beta)/(L_c(1+\beta)^2)$ and define the
number of active rounds up to time $t$ as
$N_t^{\rm up}:=\sum_{\tau=0}^{t-1}\mathbf{1}\{|\mathcal{A}_\tau|>0\}$.
Then, on $\mathcal{E}_T^{\rm ZO}$, with probability at
least $1-\delta$,
\small
\begin{align*}
  J_{\rm avg}(K_t)-J_{\rm avg}^\star
  \le\left(1-\frac{\mu_c(1-\beta)^2}{L_c(1+\beta)^2}
  \right)^{N_t^{\rm up}}
  \bigl(J_{\rm avg}(K_0)-J_{\rm avg}^\star\bigr),\\
  \forall ~t=0,\ldots,T.
\end{align*}
 In particular, if $|\mathcal{A}_t|>0$ for every
$t=0,\ldots,T-1$, then $N_t^{\rm up}=t$ and
\textsc{ResiFedLQR} converges linearly.
\hfill$\square$
\end{thm}

\begin{proof}
The total error satisfies
$\|e_t^{\rm tot}\|_2\le\zeta_t+\varepsilon\le\beta\|g_t\|_2$
on every active round by the same argument as in the proof
of Theorem~\ref{thm:stability_resifed_fixed_beta}. With
$\eta^\star=(1-\beta)/(L_c(1+\beta)^2)$,
Lemma~\ref{lem:federated_descent} gives
\[
  J_{\rm avg}(K_{t+1})
  \le J_{\rm avg}(K_t)
  -\frac{(1-\beta)^2}{2L_c(1+\beta)^2}\|g_t\|_2^2.
\]
Subtracting $J_{\rm avg}^\star$ and invoking the PL
condition $\|g_t\|_2^2\ge 2\mu_c(J_{\rm avg}(K_t)
-J_{\rm avg}^\star)$ yields a contraction by the factor
$\rho:=1-\mu_c(1-\beta)^2/(L_c(1+\beta)^2)$ on every
active round. Inactive rounds leave the gap unchanged.
Iterating gives the result.
\end{proof}

\begin{rem}[Impact of communication impairments on rate] The convergence factor depends on communication impairments only through $\beta$. Noise, dropout, and projection distortion do not alter the PL structure of the underlying optimization problem; instead, they increase the effective gradient error and thereby enlarge $\beta$. As $\beta$ approaches zero, the convergence rate approaches that of ideal federated policy gradient descent.\boxend \end{rem}

\medskip
\begin{rem}[Role of {$N_{\rm sc}$}{:} stability margin,
resilience, convergence speedup, and communication
efficiency]
The stability condition~\eqref{eq:fixed_beta_condition_resifed}
can be read as a certified relative-error condition: the
admissible $\beta$ must satisfy $\beta\ge\max_{t}(\varepsilon
+\zeta_t)/\|g_t\|_2$. Reducing $\zeta_t$ directly reduces
the smallest feasible $\beta$, enlarges the stability margin,
permits a larger stable stepsize, and decreases the
contraction factor $\rho$, yielding a faster certified linear
rate. Increasing $N_{\rm sc}$ reduces $\zeta_t$ through three
mechanisms. First, it decreases $\kappa_{\rm sc}$, reducing
the scalar projection error. Second, the same decrease in
$\kappa_{\rm sc}$ improves channel-noise averaging. Third,
it increases $q_{\rm act}=1-p_{\rm drop}^{N_{\rm sc}}$,
enlarging $\mathbb{E}[|\mathcal{A}_t|]=Mq_{\rm act}$ and
reducing the client-activation error. At equal communication
($N_{\rm sc}=dN_F$), \textsc{ResiFedLQR} has $d$~times
more scalar transmission opportunities than repeated
\textsc{FedLQR}, reducing the effective channel-noise
contribution by a factor of order $\sqrt{d}$ and enlarging
the active set in expectation.
\end{rem}
In summary, $N_{\rm sc}$
provides:
\begin{itemize}
  \item \emph{communication efficiency}: $N_{\rm sc}<dN_F$
  gives a strict bit reduction;
  \item \emph{stability-margin improvement}: larger
  $N_{\rm sc}$ reduces $\zeta_t$, making
  $\varepsilon+\zeta_t\le\beta\|g_t\|_2$ easier to satisfy;
  \item \emph{convergence speedup}: smaller feasible $\beta$
  gives a larger admissible stepsize and faster PL rate;
  \item \emph{noise resilience}: scalar averaging reduces
  the channel-noise contribution by order $\sqrt{d}$;
  \item \emph{dropout resilience}: larger $N_{\rm sc}$
  increases $q_{\rm act}$ and reduces the client-activation
  error.
\end{itemize}
Consequently, in noise- or dropout-dominated regimes where
repeated \textsc{FedLQR} admits no feasible $\beta<1$,
\textsc{ResiFedLQR} can still satisfy the stability condition
by increasing $N_{\rm sc}$, while retaining communication
efficiency whenever $N_{\rm sc}<dN_F$.

\begin{rem}[Dimension scaling] Although scalar projection introduces a dimension-dependent error through the factor $d$, the same scalar structure permits up to $d$ times more transmissions under an equal communication budget. Consequently, the dimension penalty introduced by projection is partially offset by the additional averaging that the scalar protocol enables. This tradeoff is the key mechanism underlying the communication-resilience advantages of \textsc{ResiFedLQR}. \end{rem}

\begin{rem}[Interpretation of the error decomposition] Equation~\eqref{eq:total_error_resifed_dropout} separates the effects of learning and communication. The zeroth-order error $e_t^{\rm ZO}$ is present even under perfect communication and reflects the finite-sample nature of model-free policy optimization. In contrast, $e_t^{\rm proj}$, $e_t^{\rm ch}$, and $e_t^{\rm drop}$ arise solely from the communication layer and vanish under ideal gradient exchange. This separation allows the stability analysis to distinguish limitations caused by gradient estimation from those caused by communication constraints. \end{rem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%



\clearpage

Define
$\bar h_{q,c}:=\sup_{K\in\mathcal S_c}h_{q,\mathrm{het}}(K)$,
$q\in\{1,2\}$, where $h_{1,\mathrm{het}}$ and $h_{2,\mathrm{het}}$
are the policy-gradient sensitivity quantities in Lemma~3
of~\cite{wang_model-free_2023}, and let
\begin{equation}\label{eq:b_het}
b_{\mathrm{het}}
:=
\bigl(\epsilon_1\bar h_{1,c}+\epsilon_2\bar h_{2,c}\bigr)^2.
\end{equation}
\st{can we include the full definition here? They also eventually use a $h_3$ that uniformly bounds this term. are we effectively using the same thing?}


\begin{lem}[Approximate PL condition for the average cost]
\label{lem:approximate_pl_average}
Define
$\mu_c:=\min_{n\in[M]}\mu_{n,c}$ and
$J_{\mathrm{avg}}^\star:=\inf_{K\in\mathcal S_c}J_{\mathrm{avg}}(K)$. Under Assumption~\ref{ass:pl} and the system heterogeneity condition
in~\eqref{eq::system_bound}, for every $K\in\mathcal S_c$,
\begin{subequations}
\begin{align}
&\|\nabla^2J_{\mathrm{avg}}(K)\|_2\le L_c,\label{eq:Lip}\\
&\frac{1}{2}\|\nabla J_{\mathrm{avg}}(K)\|_2^2
\ge
\mu_c\bigl(J_{\mathrm{avg}}(K)-J_{\mathrm{avg}}^\star\bigr)
-b_{\mathrm{het}}.\label{eq:pl}
\end{align}
\end{subequation}
\end{lem}

\begin{proof}
Let $g_n:=\nabla J^{(n)}(K)$ and
$g:=\frac{1}{M}\sum_{n=1}^Mg_n=\nabla J_{\mathrm{avg}}(K)$.
Averaging~\eqref{eq:individual_pl} gives
\begin{align}
\!\!\!\frac{1}{2M}\sum\nolimits_{n=1}^M\|g_n\|_2^2
&\ge
\mu_c\left(
J_{\mathrm{avg}}(K)-\frac{1}{M}\sum\nolimits_{n=1}^MJ_n^\star
\right).
\label{eq:average_individual_pl}
\end{align}
Using
\begin{align}
\frac{1}{M}\sum_{n=1}^M\|g_n\|_2^2
&=
\|g\|_2^2
+\frac{1}{2M^2}\sum_{i=1}^M\sum_{j=1}^M
\|g_i-g_j\|_2^2,
\end{align}
we obtain
\begin{align}
\frac{1}{2}\|g\|_2^2
&\ge
\mu_c\left(
J_{\mathrm{avg}}(K)-\frac{1}{M}\sum\nolimits_{n=1}^MJ_n^\star
\right)
\nonumber\\
&\quad-
\frac{1}{4M^2}\sum\nolimits_{i=1}^M\sum\nolimits_{j=1}^M
\|g_i-g_j\|_2^2.
\label{eq:average_pl_pairwise}
\end{align}
For every pair of agents $i,j\in[M]$, the system agents $i,j\in[M]$, the system heterogeneity
condition~\eqref{eq::system_bound} and the triangle inequality give
\begin{align}
\|A^{(i)}-A^{(j)}\|_2
&\le
\|A^{(i)}-A\|_2+\|A-A^{(j)}\|_2
\le 2\epsilon_1,
\nonumber\\
\|B^{(i)}-B^{(j)}\|_2
&\le
\|B^{(i)}-B\|_2+\|B-B^{(j)}\|_2
\le 2\epsilon_2.
\label{eq:pairwise_system_heterogeneity}
\end{align}
Therefore, Lemma~3 of~\cite{wang_model-free_2023} gives
\begin{align}
\|g_i-g_j\|_2
&\le
2\bigl(
\epsilon_1\bar h_{1,c}
+\epsilon_2\bar h_{2,c}
\bigr).
\end{align}
Consequently,
\begin{align}
\frac{1}{4M^2}\sum\nolimits_{i=1}^M\sum\nolimits_{j=1}^M
\|g_i-g_j\|_2^2
&\le b_{\mathrm{het}}.
\end{align}
Moreover,
$\frac{1}{M}\sum_{n=1}^MJ_n^\star\le J_{\mathrm{avg}}^\star$.
Substituting these bounds into~\eqref{eq:average_pl_pairwise}
proves~\eqref{eq:pl}.
\end{proof}

Thus, the exact PL condition is recovered when
$\epsilon_1=\epsilon_2=0$.
\hline



\hline

\begin{thm}[Linear convergence of \textsc{ScalarFedLQR} to a neighborhood]
\label{thm:pl_convergence_scalar}
Under the setup and assumptions of
Theorem~\ref{thm:stability_scalar_fixed_beta}, assume in addition that
Assumption~\ref{ass:pl} holds on $\mathcal S_c$. Let
$\eta^\star=\frac{1-\beta}{L_c(1+\beta)^2}$ and define
$
\rho:=1-\frac{\mu_c(1-\beta)^2}{L_c(1+\beta)^2}\in[0,1).
$
Then, on $\mathcal E_T^{\mathrm{ZO}}$, with probability at least
$1-\delta$,
\begin{align*}
J_{\mathrm{avg}}(K_t)-J_{\mathrm{avg}}^\star
&\le
\rho^t
\bigl(J_{\mathrm{avg}}(K_0)-J_{\mathrm{avg}}^\star\bigr)
+
(1-\rho^t)\frac{b_{\mathrm{het}}}{\mu_c}.
\end{align*}
Hence, \textsc{ScalarFedLQR} converges linearly to a
heterogeneity-dependent neighborhood of $J_{\mathrm{avg}}^\star$ with
radius $b_{\mathrm{het}}/\mu_c$. In particular,
$
\limsup_{t\rightarrow\infty}
J_{\mathrm{avg}}(K_t)-J_{\mathrm{avg}}^\star
\le b_{\mathrm{het}}/\mu_c.
$
\end{thm}

\begin{proof}
By Lemma~\ref{lem:hp_eproj_uniform_T_normalized}, with probability at
least $1-\delta$, we have
$
\|e_t^{\mathrm{proj}}\|_2\le\zeta_t
$
for all $t=0,\dots,T-1$. Also, on
$\mathcal E_T^{\mathrm{ZO}}$,
$
\|e_t^{\mathrm{ZO}}\|_2\le\varepsilon
$
for all $t=0,\dots,T-1$. Hence,
$
\|e_t^{\mathrm{tot}}\|_2
\le
\|e_t^{\mathrm{proj}}\|_2+\|e_t^{\mathrm{ZO}}\|_2
\le
\zeta_t+\varepsilon
\le
\beta\|g_t\|_2.
$
Therefore, Lemma~\ref{lem:federated_descent} applies with
$\beta_t=\beta$. With
$
\eta^\star=\eta_{\max}/2
=\frac{1-\beta}{L_c(1+\beta)^2},
$
we obtain
\begin{align}
J_{\mathrm{avg}}(K_{t+1})
&\le
J_{\mathrm{avg}}(K_t)
-\frac{(1-\beta)^2}
{2L_c(1+\beta)^2}\|g_t\|_2^2.
\label{eq:pl_pf_descent_beta}
\end{align}
Let
$
F_t:=J_{\mathrm{avg}}(K_t)-J_{\mathrm{avg}}^\star.
$
By Lemma~\ref{lem:approximate_pl_average},
\begin{align}
\|g_t\|_2^2
&\ge
2\mu_cF_t-2b_{\mathrm{het}}.
\end{align}
Substituting this inequality into
\eqref{eq:pl_pf_descent_beta} gives
\begin{align*}
F_{t+1}
&\le
F_t
-\frac{(1-\beta)^2}
{L_c(1+\beta)^2}
\bigl(\mu_cF_t-b_{\mathrm{het}}\bigr)
\\
&=
\rho F_t
+
(1-\rho)\frac{b_{\mathrm{het}}}{\mu_c}.
\end{align*}
Iterating this recursion yields
\begin{align*}
F_t
&\le
\rho^tF_0
+
(1-\rho^t)\frac{b_{\mathrm{het}}}{\mu_c},
\end{align*}
which proves the result.
\end{proof}


The above result uses the relative-error condition
$
\varepsilon+\zeta_t\le\beta\|g_t\|_2
$
from Theorem~\ref{thm:stability_scalar_fixed_beta}; hence, the
zeroth-order accuracy is absorbed into the relative-error requirement
and does not appear as a separate term in the final neighborhood.
Under the milder relative-plus-additive condition
$
\|e_t^{\mathrm{tot}}\|_2
\le
\beta\|g_t\|_2+\varepsilon_{\mathrm{eff}},
$
the convergence neighborhood is expected to contain both the
heterogeneity term $b_{\mathrm{het}}/\mu_c$ and an additional
gradient-accuracy term of order
$
\varepsilon_{\mathrm{eff}}^2/
\bigl(\mu_c(1-\beta)^2\bigr),
$
consistent with prior model-free FedLQR analysis
\cite{wang_model-free_2023}. A detailed treatment of this milder
condition is left for future work.


\clearpage


\appendices

\section{Technical Details}
% \begin{lem}[Johnson--Lindenstrauss Lemma \cite{matouvsek2008variants}]
% \label{lem:JL}
% Fix \(0<\varepsilon<1\) and \(0<\delta<1\). Let \(d\in\mathbb N\) be the ambient dimension and let \(N_{\mathrm{sc}}\) denote the embedding dimension. Suppose
% \[
% N_{\mathrm{sc}}
% =
% O\!\left(
% \frac{\log(d/\delta)}{\varepsilon^2}
% \right).
% \]
% Let \(P\in\mathbb{R}^{N_{\mathrm{sc}}\times d}\) be a random matrix whose entries are i.i.d.\ mean-zero, unit-variance, sub-Gaussian random variables. Then, for any fixed \(x\in\mathbb{R}^d\), with probability at least \(1-\delta\),
% \begin{equation}
% (1-\varepsilon)\|x\|_2^2
% \le
% \frac{1}{N_{\mathrm{sc}}}\|Px\|_2^2
% \le
% (1+\varepsilon)\|x\|_2^2 .
% \label{eq:JL_general}
% \end{equation}
% \boxend
% \end{lem}


\begin{proof}[Proof of Lemma~\ref{lem:federated_descent}]
\reza{Since \(J_{\mathrm{avg}}\) is \(L_c\)-smooth on \(\mathcal S_c\), we have
\begin{align}
J_{\mathrm{avg}}(K_{t+1})
\le
J_{\mathrm{avg}}(K_t)
+
\big\langle \nabla J_{\mathrm{avg}}(K_t), K_{t+1}-K_t \big\rangle
\nonumber\\+
\frac{L_c}{2}\|K_{t+1}-K_t\|_2^2 .
\label{eq:descent_pf_1}
\end{align}
Using \(g_t=\nabla J_{\mathrm{avg}}(K_t)\) and the update
$
K_{t+1}=K_t-\eta\,\widehat g_t,
$
we obtain}
\begin{align}
J_{\mathrm{avg}}(K_{t+1})
\le
J_{\mathrm{avg}}(K_t)
-\eta \langle g_t,\widehat g_t\rangle
+\frac{L_c\eta^2}{2}\|\widehat g_t\|_2^2 .
\label{eq:descent_pf_2}
\end{align}

By definition of the total error in \eqref{eq:total_error_resifed},
we have
$
\widehat g_t
=
g_t+e_t^{\mathrm{tot}}.
$
Substituting this into the inner-product term in \eqref{eq:descent_pf_2} gives
\begin{align}
\langle g_t,\widehat g_t\rangle
=
\langle g_t,g_t+e_t^{\mathrm{tot}}\rangle
=
\|g_t\|_2^2
+
\langle g_t,e_t^{\mathrm{tot}}\rangle .
\label{eq:descent_pf_3}
\end{align}
Similarly,
\begin{align}
\|\widehat g_t\|_2^2
=
\|g_t+e_t^{\mathrm{tot}}\|_2^2 .
\label{eq:descent_pf_4}
\end{align}
Plugging \eqref{eq:descent_pf_3} and \eqref{eq:descent_pf_4} into
\eqref{eq:descent_pf_2} yields
\begin{align}
J_{\mathrm{avg}}(K_{t+1})
\le
J_{\mathrm{avg}}(K_t)
-\eta \|g_t\|_2^2
-\eta \langle g_t,e_t^{\mathrm{tot}}\rangle
\nonumber\\ +
\frac{L_c\eta^2}{2}
\|g_t+e_t^{\mathrm{tot}}\|_2^2 .
\label{eq:descent_pf_5}
\end{align}
Using Cauchy--Schwarz, we have 
$
-\langle g_t,e_t^{\mathrm{tot}}\rangle
\le
\|g_t\|_2\|e_t^{\mathrm{tot}}\|_2,
$
and using the triangle inequality,
$
\|g_t+e_t^{\mathrm{tot}}\|_2
\le
\|g_t\|_2+\|e_t^{\mathrm{tot}}\|_2 .
$
Therefore, from \eqref{eq:descent_pf_5},
\begin{align}
J_{\mathrm{avg}}(K_{t+1})
\le
J_{\mathrm{avg}}(K_t)
-\eta \|g_t\|_2^2
+
\eta \|g_t\|_2\|e_t^{\mathrm{tot}}\|_2
\nonumber \\+
\frac{L_c\eta^2}{2}
\bigl(\|g_t\|_2+\|e_t^{\mathrm{tot}}\|_2\bigr)^2 .
\label{eq:descent_pf_6}
\end{align}

Now suppose that
$
\|e_t^{\mathrm{tot}}\|_2
\le
\beta_t\|g_t\|_2.
$
Then
$
\eta \|g_t\|_2\|e_t^{\mathrm{tot}}\|_2
\le
\eta\beta_t\|g_t\|_2^2,
$
and
$
\bigl(\|g_t\|_2+\|e_t^{\mathrm{tot}}\|_2\bigr)^2
\le
(1+\beta_t)^2\|g_t\|_2^2.
$
Substituting these bounds into \eqref{eq:descent_pf_6}, we obtain
\begin{align}
J_{\mathrm{avg}}(K_{t+1})
\le
J_{\mathrm{avg}}(K_t)
-
\eta
\left[
(1-\beta_t)
-
\frac{L_c\eta}{2}(1+\beta_t)^2
\right]
\|g_t\|_2^2 .
\end{align}
Provided $0<\eta<\frac{2(1-\beta_t)}{L_c(1+\beta_t)^2}$, This proves the desired one-step descent bound.
\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:hp_erec_resifed}]
Let \(B_{t,n,s}\in\{0,1\}\) be the scalar delivery indicator, and let
\(I_{t,n}:=\mathbf 1\{N_{t,n}^{\rm rec}>0\}\). Thus,
$
N_{t,n}^{\rm rec}
=
\sum_{s=1}^{N_{\mathrm{sc}}}B_{t,n,s},
\quad
|\mathcal A_t|
=
\sum_{n=1}^{M}I_{t,n}.
$
Also, \(I_{t,n}=1\) if at least one scalar message from client \(n\) is received,
so \(\mathbb P(I_{t,n}=1)=q_{\rm act}=1-p_{\rm drop}^{N_{\mathrm{sc}}}\). By the decoder in Algorithm~\ref{alg:nc_scalarfedlqr_inline}, with the convention
\(I_{t,n}/N_{t,n}^{\rm rec}=0\) when \(N_{t,n}^{\rm rec}=0\), we have
\begin{align}
\widehat g_t
=
\frac{1}{|\mathcal A_t|}
\sum_{n=1}^{M}
I_{t,n}
\frac{1}{N_{t,n}^{\rm rec}}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}
\left[
(v_{t,n,s}^{\top}\tilde g_{t,n})+w_{n,s}^t
\right]v_{t,n,s}.
\label{eq:dropout_decoder_pf}
\end{align}
For each received scalar, write
\[
\left[
(v_{t,n,s}^{\top}\tilde g_{t,n})+w_{n,s}^t
\right]v_{t,n,s}
=
\tilde g_{t,n}
+
Z_{n,s},
\]
where
\begin{align}
Z_{n,s}
:=
\bigl(v_{t,n,s}v_{t,n,s}^{\top}-I\bigr)\tilde g_{t,n}
+
w_{n,s}^t v_{t,n,s}.
\label{eq:Zns_dropout_pf}
\end{align}
Substituting this identity into \eqref{eq:dropout_decoder_pf} gives
\begin{align}
\widehat g_t
&=
\frac{1}{|\mathcal A_t|}
\sum_{n=1}^{M}I_{t,n}\tilde g_{t,n}
+
\frac{1}{|\mathcal A_t|}
\sum_{n=1}^{M}
I_{t,n}
\frac{1}{N_{t,n}^{\rm rec}}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}Z_{n,s}.
\label{eq:ghat_split_pf}
\end{align}
Now let \(\Delta_{t,n}:=\tilde g_{t,n}-\tilde g_t\), where
\(\tilde g_t=\frac{1}{M}\sum_{n=1}^M\tilde g_{t,n}\). Then
\(\sum_{n=1}^{M}\Delta_{t,n}=0\). Since
\(|\mathcal A_t|=\sum_{n=1}^{M}I_{t,n}\), we may write
$
\tilde g_t
=
|\mathcal A_t|^{-1}\sum_{n=1}^{M}I_{t,n}\tilde g_t.
$
Therefore,
\begin{align}
\frac{1}{|\mathcal A_t|}
\sum_{n=1}^{M}I_{t,n}\tilde g_{t,n}
-
\tilde g_t
&=
\frac{1}{|\mathcal A_t|}
\sum_{n=1}^{M}I_{t,n}(\tilde g_{t,n}-\tilde g_t)
\nonumber\\
&=
\frac{1}{|\mathcal A_t|}
\sum_{n=1}^{M}I_{t,n}\Delta_{t,n}.
\label{eq:active_average_drop_pf}
\end{align}
Moreover,
\begin{align*}
\sum_{n=1}^{M}I_{t,n}\Delta_{t,n}
&=
\sum_{n=1}^{M}(I_{t,n}-q_{\rm act})\Delta_{t,n}
+
q_{\rm act}\sum_{n=1}^{M}\Delta_{t,n}
\\
&=\sum_{n=1}^{M}(I_{t,n}-q_{\rm act})\Delta_{t,n}.
\end{align*}
Combining \eqref{eq:ghat_split_pf} and \eqref{eq:active_average_drop_pf}, the
full communication-layer error can be written as
$
e_t^{\mathrm{rec}}
=
\widehat g_t-\tilde g_t
=
\frac{1}{|\mathcal A_t|}
\sum_{n=1}^{M}X_{t,n},
\label{eq:erec_Xtn_pf}
$
where
\begin{align}
X_{t,n}
:=
(I_{t,n}-q_{\rm act})\Delta_{t,n}
+
I_{t,n}
\frac{1}{N_{t,n}^{\rm rec}}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}Z_{n,s}.
\label{eq:Xtn_def_pf}
\end{align}
We next verify that \(X_{t,n}\) is centered. Condition on the local gradient
estimates \(\{\tilde g_{t,n}\}_{n=1}^{M}\). The first term satisfies
\[
\mathbb E\big[(I_{t,n}-q_{\rm act})\Delta_{t,n}\big]
=
(\mathbb E[I_{t,n}]-q_{\rm act})\Delta_{t,n}
=
0.
\]
For the second term, conditioning further on the dropout variables
\(\{B_{t,n,s}\}_{s=1}^{N_{\mathrm{sc}}}\), we have
\begin{align*}
\mathbb E\!\left[
I_{t,n}
\frac{1}{N_{t,n}^{\rm rec}}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}Z_{n,s}
\,\middle|\,
\{B_{t,n,s}\}_{s=1}^{N_{\mathrm{sc}}}
\right]
=\\
I_{t,n}
\frac{1}{N_{t,n}^{\rm rec}}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}\mathbb E[Z_{n,s}]
=
0,
\end{align*}
because
\[
\mathbb E[Z_{n,s}]
=
\mathbb E\!\left[
\bigl(v_{t,n,s}v_{t,n,s}^{\top}-I\bigr)\tilde g_{t,n}
\right]
+
\mathbb E[w_{n,s}^t v_{t,n,s}]
=
0.
\]
Thus, conditioned on the local gradient estimates, the vectors
\(\{X_{t,n}\}_{n=1}^{M}\) are independent and mean-zero. We now compute their variance proxy. First, for fixed \(n,s\), write
\(v=v_{t,n,s}\), \(w=w_{n,s}^t\), and \(g_n=\tilde g_{t,n}\). Then
\(Z_{n,s}=(vv^\top-I)g_n+wv\). The cross term vanishes because \(w\) is
independent of \(v\) and \(\mathbb E[w]=0\). Hence
\begin{align}
\mathbb E\|Z_{n,s}\|_2^2
=
\mathbb E\|(vv^\top-I)g_n\|_2^2
+
\mathbb E\|wv\|_2^2 .
\end{align}
For an unnormalized Rademacher vector \(v\in\{\pm1\}^d\),
\begin{equation}\label{eq:rademacher_second_moment_combined}
\mathbb E\|(vv^\top-I)z\|_2^2=(d-1)\|z\|_2^2,
\qquad
\forall z\in\mathbb R^d .
\end{equation}
Also, since \(\|v\|_2^2=d\) and
\(\mathbb E[(w_{n,s}^t)^2]\le\sigma_{\mathrm{ch}}^2\),
$
\mathbb E\|w_{n,s}^t v_{t,n,s}\|_2^2\le d\sigma_{\mathrm{ch}}^2.
$
Therefore,
$
\mathbb E\|Z_{n,s}\|_2^2
\le
(d-1)\|\tilde g_{t,n}\|_2^2+d\sigma_{\mathrm{ch}}^2 .
$ We bound the second moment of \(X_{t,n}\). The cross term between
\((I_{t,n}-q_{\rm act})\Delta_{t,n}\) and the scalar reconstruction term is zero,
because the scalar reconstruction term has conditional mean zero given the
dropout pattern. Therefore,
\begin{align}
\mathbb E\|X_{t,n}\|_2^2
&\le
\mathbb E\|(I_{t,n}-q_{\rm act})\Delta_{t,n}\|_2^2
\nonumber\\
&\quad+
\mathbb E\!\left\|
I_{t,n}
\frac{1}{N_{t,n}^{\rm rec}}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}Z_{n,s}
\right\|_2^2 .
\label{eq:Xtn_second_moment_split_pf}
\end{align}
The first term is
\[
\mathbb E\|(I_{t,n}-q_{\rm act})\Delta_{t,n}\|_2^2
=
q_{\rm act}(1-q_{\rm act})\|\Delta_{t,n}\|_2^2 .
\]
For the second term, condition on the delivery indicators. Since the
\(\{Z_{n,s}\}\) are independent and mean-zero,
\begin{align}
&\mathbb E\!\left[
\left\|
I_{t,n}
\frac{1}{N_{t,n}^{\rm rec}}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}Z_{n,s}
\right\|_2^2
\,\middle|\,
\{B_{t,n,s}\}_{s=1}^{N_{\mathrm{sc}}}
\right]
\nonumber\\
&\qquad
=
I_{t,n}
\frac{1}{(N_{t,n}^{\rm rec})^2}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}\mathbb E\|Z_{n,s}\|_2^2
\nonumber\\
&\qquad
\le
\frac{I_{t,n}}{N_{t,n}^{\rm rec}}
\left[
(d-1)\|\tilde g_{t,n}\|_2^2+d\sigma_{\mathrm{ch}}^2
\right].
\label{eq:conditional_second_moment_scalar_pf}
\end{align}
Taking expectation over the delivery indicators gives
\begin{align}
\mathbb E
\left\|
I_{t,n}
\frac{1}{N_{t,n}^{\rm rec}}
\sum_{s=1}^{N_{\mathrm{sc}}}
B_{t,n,s}Z_{n,s}
\right\|_2^2
&\le
\kappa_{\rm sc}
\left[
(d-1)\|\tilde g_{t,n}\|_2^2+d\sigma_{\mathrm{ch}}^2
\right],
\end{align}
where
$
\kappa_{\rm sc}=\mathbb E[\mathbf 1\{N_{t,n}^{\rm rec}>0\}/N_{t,n}^{\rm rec}].
$
Combining the last displays,
\begin{align}
\mathbb E\|X_{t,n}\|_2^2
&\le
q_{\rm act}(1-q_{\rm act})\|\Delta_{t,n}\|_2^2
\nonumber\\
&\quad+
\kappa_{\rm sc}
\left[
(d-1)\|\tilde g_{t,n}\|_2^2+d\sigma_{\mathrm{ch}}^2
\right].
\end{align}
Summing over \(n\), and using Assumption~\ref{ass:heterogeneity}, gives
\begin{align}
V_t
:=
&\sum_{n=1}^{M}\mathbb E\|X_{t,n}\|_2^2
\le
M q_{\rm act}(1-q_{\rm act})\Gamma_t^2
\nonumber\\
&\quad+
M\kappa_{\rm sc}
\left[
(d-1)
\left(
\frac{1}{M}\sum_{n=1}^{M}\|\tilde g_{t,n}\|_2^2
\right)
+d\sigma_{\mathrm{ch}}^2
\right].
\end{align}
Since \(\tilde g_{t,n}=\tilde g_t+\Delta_{t,n}\) and
\(\sum_{n=1}^{M}\Delta_{t,n}=0\),
\[
\frac{1}{M}\sum_{n=1}^{M}\|\tilde g_{t,n}\|_2^2
=
\|\tilde g_t\|_2^2+
\frac{1}{M}\sum_{n=1}^{M}\|\Delta_{t,n}\|_2^2
\le
\|\tilde g_t\|_2^2+\Gamma_t^2.
\]
Thus
\begin{align}\label{eq:combined_variance_proxy_dropout}
V_t
\!\le\!
M q_{\rm act}(1-q_{\rm act})\Gamma_t^2
\!+
\!\!M\kappa_{\rm sc}
\!\!\left[
\!(d-1)\bigl(\|\tilde g_t\|_2^2+\Gamma_t^2\bigr)
\!\!+\!
d\sigma_{\mathrm{ch}}^2
\!\right].
\end{align}
It remains to control the bounded part of the summand. For the dropout part,
since \(|I_{t,n}-q_{\rm act}|\le 1\) and \(\|\Delta_{t,n}\|_2\le B_t\), we have
$
\|(I_{t,n}-q_{\rm act})\Delta_{t,n}\|_2\le B_t.
$
For the scalar-projection part, since
\(\|vv^\top-I\|_{\rm op}=d-1\) for \(v\in\{\pm1\}^d\), we have
\[
\|(vv^\top-I)\tilde g_{t,n}\|_2
\le
(d-1)\|\tilde g_{t,n}\|_2
\le
(d-1)(\|\tilde g_t\|_2+B_t).
\]
Therefore, a valid Bernstein radius for the bounded part of \(X_{t,n}\) is
$
R_t
:=
(d-1)(\|\tilde g_t\|_2+B_t)+B_t .
$ Applying a vector Bernstein-type inequality to the independent mean-zero
vectors \(\{X_{t,n}\}_{n=1}^{M}\), with variance proxy
\eqref{eq:combined_variance_proxy_dropout} and radius \(R_t\), yields
\begin{align}
\left\|
\sum_{n=1}^{M}X_{t,n}
\right\|_2
\le
C\sqrt{V_t\log(6d/\delta)}
+
C R_t\log(6d/\delta)
\end{align}
with probability at least \(1-\delta\). Finally, using
\eqref{eq:erec_Xtn_pf},
\[
\|e_t^{\mathrm{rec}}\|_2
=
\left\|
\frac{1}{|\mathcal A_t|}
\sum_{n=1}^{M}X_{t,n}
\right\|_2
\le
\frac{1}{|\mathcal A_t|}
\left\|
\sum_{n=1}^{M}X_{t,n}
\right\|_2 .
\]
Substituting the bound on \(V_t\) from
\eqref{eq:combined_variance_proxy_dropout} and the definition of \(R_t\) gives
\eqref{eq:hp_erec_resifed}.
This completes the
proof.
\end{proof}


\begin{lem}[Uniform high-probability bound for the combined scalar-reconstruction error over \(T\) rounds]
\label{lem:hp_erec_uniform_T_resifed}
Under the setup of Lemma~\ref{lem:hp_erec_resifed}, fix any horizon
\(T\ge 1\) and any \(\delta\in(0,1)\). Then, with probability at least
\(1-\delta\), the following bound holds simultaneously for all rounds
\(t=0,\ldots,T-1\) with \(|\mathcal A_t|>0\):
\begingroup
\small
\begin{align}
\label{eq:hp_erec_uniformT_resifed}
&\|e_t^{\mathrm{rec}}\|_2
\le
\underbrace{
\frac{C\sqrt{M\kappa_{\rm sc}(d-1)\log(6dT/\delta)}}{|\mathcal A_t|}
\sqrt{\|\tilde g_t\|_2^2+\Gamma_t^2}
}_{\text{\scriptsize scalar reconstruction error}}
\nonumber\\
\!&+\!\!
\underbrace{
\frac{C\sqrt{M\kappa_{\rm sc}d\log(6dT/\delta)}}{|\mathcal A_t|}
\sigma_{\rm ch}
}_{\text{\scriptsize channel-noise error}}
\!\!+\!\!
\underbrace{
\frac{C\sqrt{M q_{\rm act}(1-q_{\rm act})\log(6dT/\delta)}}{|\mathcal A_t|}
\Gamma_t
}_{\text{\scriptsize client-activation error}}
\nonumber\\
&+
\underbrace{
\frac{C\log(6dT/\delta)}{|\mathcal A_t|}
\left[
(d-1)\bigl(\|\tilde g_t\|_2+B_t\bigr)+B_t
\right]
}_{\text{\scriptsize lower-order Bernstein term}},
\end{align}
\endgroup
where \(C>0\) is an absolute constant.
\boxend
\end{lem}

\begin{proof}
Apply Lemma~\ref{lem:hp_erec_resifed} at each round with failure probability
\(\delta/T\). For any fixed \(t\), we obtain
\begingroup
\small
\begin{align}
&\Pr\!\bigg(
\|e_t^{\mathrm{rec}}\|_2
\le
\frac{C\sqrt{M\kappa_{\rm sc}(d-1)\log(6dT/\delta)}}{|\mathcal A_t|}
\sqrt{\|\tilde g_t\|_2^2+\Gamma_t^2}
\nonumber\\
\!&+\!\!
\frac{C\sqrt{M\kappa_{\rm sc}d\log(6dT/\delta)}}{|\mathcal A_t|}
\sigma_{\rm ch}
\!\!+\!\!
\frac{C\sqrt{M q_{\rm act}(1-q_{\rm act})\log(6dT/\delta)}}{|\mathcal A_t|}
\Gamma_t
\nonumber\\
&+
\frac{C\log(6dT/\delta)}{|\mathcal A_t|}
\left[
(d-1)\bigl(\|\tilde g_t\|_2+B_t\bigr)+B_t
\right]
\bigg)
\ge
1-\frac{\delta}{T}.
\nonumber
\end{align}
\endgroup
Finally, a union bound over \(t=0,\ldots,T-1\) gives
\[
\Pr\!\left(
\bigcap_{t=0}^{T-1}
\left\{
\eqref{eq:hp_erec_uniformT_resifed}\ \text{holds}
\right\}
\right)
\ge
1-\sum_{t=0}^{T-1}\frac{\delta}{T}
=
1-\delta.
\]
This proves \eqref{eq:hp_erec_uniformT_resifed}.
\end{proof}






\clearpage
\begin{comment}
    

\begin{proof}[Proof of Lemma~\ref{lem:hp_erec_resifed}]
By definition of the received direction,
\[
\widehat g_t
=
\frac{1}{M N_{\mathrm{sc}}}
\sum_{n=1}^{M}
\sum_{s=1}^{N_{\mathrm{sc}}}
\left[
(v_{t,n,s}^{\top}\tilde g_{t,n})+w_{n,s}^t
\right]
v_{t,n,s}.
\]
Since
$
\tilde g_t
=
\frac{1}{M}\sum_{n=1}^M \tilde g_{t,n},
$
and since \(\mathbb{E}[v_{t,n,s}v_{t,n,s}^{\top}]=I\), we can write the
combined scalar-reconstruction error as
\begin{align}
e_t^{\mathrm{rec}}
&=
\widehat g_t-\tilde g_t
\nonumber\\
&=
\frac{1}{M N_{\mathrm{sc}}}
\sum_{n=1}^{M}
\sum_{s=1}^{N_{\mathrm{sc}}}
Z_{n,s},
\end{align}
where
\begin{align}
Z_{n,s}
:=
\bigl(v_{t,n,s}v_{t,n,s}^{\top}-I\bigr)\tilde g_{t,n}
+
w_{n,s}^t v_{t,n,s}.
\end{align}
Conditioned on the local gradient estimates
\(\{\tilde g_{t,n}\}_{n=1}^M\), the vectors \(\{Z_{n,s}\}_{n,s}\) are
independent and mean-zero. Indeed,
\[
\mathbb{E}\!\left[
\bigl(v_{t,n,s}v_{t,n,s}^{\top}-I\bigr)\tilde g_{t,n}
\right]
=0,
\qquad
\mathbb{E}\!\left[w_{n,s}^t v_{t,n,s}\right]=0.
\]

We next compute the variance proxy of the combined summand. For notational
simplicity, fix \(n,s\) and write \(v=v_{t,n,s}\), \(w=w_{n,s}^t\), and
\(g_n=\tilde g_{t,n}\). Then
$
Z_{n,s}
=
(vv^\top-I)g_n+w v .
$
Using the independence of \(w\) and \(v\), and the fact that
\(\mathbb{E}[w]=0\), the cross term vanishes, i.e., 
\[
\mathbb{E}
\left[
\left\langle
(vv^\top-I)g_n,\,
w v
\right\rangle
\right]
=
0.
\]
Therefore,
\begin{align}
\mathbb{E}\|Z_{n,s}\|_2^2
&=
\mathbb{E}
\left\|
(vv^\top-I)g_n
\right\|_2^2
+
\mathbb{E}
\left\|
w v
\right\|_2^2 .
\end{align}
For an unnormalized Rademacher vector \(v\in\{\pm1\}^d\), we have
\begin{equation}\label{eq:rademacher_second_moment_combined}
\mathbb{E}
\left\|
(vv^\top-I)z
\right\|_2^2
=
(d-1)\|z\|_2^2 ,
\qquad
\forall z\in\mathbb{R}^d .
\end{equation}
Moreover, since \(\|v\|_2^2=d\) and
\(\mathbb{E}[w^2]\le \sigma_{\mathrm{ch}}^2\),
\[
\mathbb{E}\|wv\|_2^2
=
\mathbb{E}[w^2]\|v\|_2^2
\le
d\sigma_{\mathrm{ch}}^2 .
\]
Hence,
\[
\mathbb{E}\|Z_{n,s}\|_2^2
\le
(d-1)\|\tilde g_{t,n}\|_2^2
+
d\sigma_{\mathrm{ch}}^2 .
\]
Summing over \(n\) and \(s\) gives
\begin{align}
\sum_{n=1}^{M}
\sum_{s=1}^{N_{\mathrm{sc}}}&
\mathbb{E}\|Z_{n,s}\|_2^2
\le
N_{\mathrm{sc}}
\sum_{n=1}^{M}
\left[
(d-1)\|\tilde g_{t,n}\|_2^2
+
d\sigma_{\mathrm{ch}}^2
\right]
\nonumber\\
&=
M N_{\mathrm{sc}}
\left[
(d-1)
\left(
\frac{1}{M}\sum_{n=1}^{M}
\|\tilde g_{t,n}\|_2^2
\right)
+
d\sigma_{\mathrm{ch}}^2
\right].
\end{align}
Using
$
\tilde g_{t,n}=\tilde g_t+\Delta_{t,n},
\quad
\sum_{n=1}^{M}\Delta_{t,n}=0,
$
we obtain
\[
\frac{1}{M}\sum_{n=1}^{M}
\|\tilde g_{t,n}\|_2^2
=
\|\tilde g_t\|_2^2
+
\frac{1}{M}\sum_{n=1}^{M}
\|\Delta_{t,n}\|_2^2
\le
\|\tilde g_t\|_2^2+\Gamma_t^2 .
\]
Thus the combined variance proxy satisfies
\begin{align}
\label{eq:combined_variance_proxy}
V_t
\!:=\!\!
\sum_{n=1}^{M}
\!\!\sum_{s=1}^{N_{\mathrm{sc}}}\!
\mathbb{E}\|Z_{n,s}\|_2^2
\!\le \!\!
M N_{\mathrm{sc}}
\!\!\left[
(d-1)\bigl(\|\tilde g_t\|_2^2+\Gamma_t^2\bigr)
\!+\!
d\sigma_{\mathrm{ch}}^2
\right]\!\!.
\end{align}

It remains to control the bounded part of the summand. Since
$
\|vv^\top-I\|_{\mathrm{op}}=d-1
$
for \(v\in\{\pm1\}^d\), we have
\begin{align}
\left\|
(vv^\top-I)\tilde g_{t,n}
\right\|_2
&\le
(d-1)\|\tilde g_{t,n}\|_2
\nonumber\\
&\le
(d-1)\bigl(\|\tilde g_t\|_2+B_t\bigr).
\end{align}
The channel component \(wv\) is Gaussian conditional on \(v\) and is already
captured in the variance proxy \eqref{eq:combined_variance_proxy}. Applying a
vector Bernstein-type inequality for the sum of independent
mean-zero vector-valued summands with the combined variance proxy
\eqref{eq:combined_variance_proxy} and the above bounded projection radius gives
\begin{align*}
\left\|
\sum_{n=1}^{M}
\sum_{s=1}^{N_{\mathrm{sc}}}
Z_{n,s}
\right\|_2&
\le
C
\sqrt{
V_t \log(2d/\delta)
}
~~+
\nonumber\\&C
(d-1)\bigl(\|\tilde g_t\|_2+B_t\bigr)
\log(2d/\delta)
\end{align*}
with probability at least \(1-\delta\). Dividing both sides by
\(M N_{\mathrm{sc}}\) and substituting the bound on \(V_t\) from
\eqref{eq:combined_variance_proxy} yields
\begin{align}
\|e_t^{\mathrm{rec}}\|_2
&\le
C
\sqrt{
\frac{\log(2d/\delta)}
{M N_{\mathrm{sc}}}
\left[
(d-1)\bigl(\|\tilde g_t\|_2^2+\Gamma_t^2\bigr)
+
d\sigma_{\mathrm{ch}}^2
\right]
}
\nonumber\\
&\quad+
C
\frac{(d-1)\log(2d/\delta)}
{M N_{\mathrm{sc}}}
\bigl(\|\tilde g_t\|_2+B_t\bigr),
\end{align}
which proves \eqref{eq:hp_erec_resifed}.
\end{proof}


Lemma~\ref{lem:hp_erec_resifed} controls the noisy scalar reconstruction error
\(e_t^{\mathrm{rec}}=e_t^{\mathrm{proj}}+e_t^{\mathrm{ch}}\) at a single round.
To establish stability over the full optimization horizon, we next strengthen
this result to a uniform high-probability bound that holds simultaneously for all
rounds \(t=0,\dots,T-1\).




\begin{lem}[Uniform high-probability bound for the combined scalar-reconstruction error over \(T\) rounds]
\label{lem:hp_erec_uniform_T_resifed}
Under the setup of Lemma~\ref{lem:hp_erec_resifed}, fix any horizon
\(T\ge 1\) and any \(\delta\in(0,1)\). Then, with probability at least
\(1-\delta\), the following bound holds simultaneously for all rounds
\(t=0,\ldots,T-1\):
\begin{align}
\label{eq:hp_erec_uniformT_resifed}
\|e_t^{\mathrm{rec}}\|_2
&\le
C
\sqrt{
\frac{\log(2dT/\delta)}
{M N_{\mathrm{sc}}}
\left[
(d-1)\bigl(\|\tilde g_t\|_2^2+\Gamma_t^2\bigr)
+
d\sigma_{\mathrm{ch}}^2
\right]
}
\nonumber\\
&\quad+
C
\frac{(d-1)\log(2dT/\delta)}
{M N_{\mathrm{sc}}}
\bigl(\|\tilde g_t\|_2+B_t\bigr),
\end{align}
where \(C>0\) is an absolute constant.
\boxend
\end{lem}

\begin{proof}
Apply Lemma~\ref{lem:hp_erec_resifed} at each round with failure probability
\(\delta/T\). For any fixed \(t\), we obtain
\begin{align}
\Pr\!\bigg(
\|e_t^{\mathrm{rec}}\|_2
&\le
C
\sqrt{
\frac{\log(2dT/\delta)}
{M N_{\mathrm{sc}}}
\left[
(d-1)\bigl(\|\tilde g_t\|_2^2+\Gamma_t^2\bigr)
+
d\sigma_{\mathrm{ch}}^2
\right]
}
\nonumber\\
&+
C
\frac{(d-1)\log(2dT/\delta)}
{M N_{\mathrm{sc}}}
\bigl(\|\tilde g_t\|_2+B_t\bigr)
\bigg)
\ge
1-\frac{\delta}{T}.
\nonumber
\end{align}
Finally, a union bound over \(t=0,\dots,T-1\) yields
\[
\Pr\!\left(
\bigcap_{t=0}^{T-1}
\left\{
\eqref{eq:hp_erec_uniformT_resifed}\ \text{holds}
\right\}
\right)
\ge
1-\sum_{t=0}^{T-1}\frac{\delta}{T}
=
1-\delta,
\]
which proves \eqref{eq:hp_erec_uniformT_resifed}.
\end{proof}

\end{comment}



% \begin{lem}[Vector Bernstein inequality]
% \label{lem:vector_bernstein}
% Let $X_1,\ldots,X_N\in\mathbb{R}^d$ be independent mean-zero random vectors.
% Assume that
% \[
% \|X_i\|_2 \le R
% \qquad \text{almost surely for all } i,
% \]
% and define the variance proxy
% \[
% V := \sum_{i=1}^{N}\mathbb{E}\|X_i\|_2^2 .
% \]
% Then, for any $\delta\in(0,1)$, with probability at least $1-\delta$,
% \[
% \left\|
% \sum_{i=1}^{N}X_i
% \right\|_2
% \le
% C\left(
% \sqrt{V\log\!\left(\frac{2d}{\delta}\right)}
% +
% R\log\!\left(\frac{2d}{\delta}\right)
% \right),
% \]
% where $C>0$ is an absolute constant.
% \end{lem}
% \st{On the first attempt, we would try to keep the oracle intact and just apply the FedScalar idea to the setup. I suggest we finish this first quickly which seems very doable. 
% On the second attempt, as I discussed with Reza, we could think of opening up the oracle and think of the single projection type ideas in order to combine the efficient projection ideas closer to the actual data. 
% } 


% \section{Stability analysis and convergence of ScalarFedLQR}
% We now turn to the stability analysis of \textsc{ScalarFedLQR}.
% Our goal is to show that, under suitable conditions on the stepsize and the gradient estimation error, the server-side updates generated by Algorithm~\ref{alg:scalarfedlqr_inline} remain inside a stabilizing sublevel set $\mathcal S_c$ of the average cost $J_{\mathrm{avg}}$.

% The key technical challenge, relative to standard FedLQR, is that the server does \emph{not} receive full gradient vectors.
% Instead, it reconstructs an aggregated direction $\bar g_t$ from scalar projections. We begin the stability analysis by quantifying how a single iteration of
% \textsc{ScalarFedLQR} affects the average cost when the server updates the policy
% along an approximate direction $\bar g_t$ reconstructed from scalar projections.
% Because $\bar g_t$ is not exactly $\nabla J_{\mathrm{avg}}(K_t)$, the key difficulty is to
% characterize how this approximation error influences descent of $J_{\mathrm{avg}}$.
% Lemma~\ref{lem:federated_descent} provides a one-step descent guarantee that
% relates the decrease in $J_{\mathrm{avg}}$ to the magnitude of the total gradient error
% $\|\bar g_t-\nabla J_{\mathrm{avg}}(K_t)\|_2$ and the smoothness constant $L_c$.
% This result serves as the foundation for our subsequent stability and convergence
% analysis.


% \begin{lem}[One-step descent for scalar-projection aggregated update]\label{lem:federated_descent}
% Fix $K_t\in\mathcal S_c$ and let $g_t:=\nabla J_{\mathrm{avg}}(K_t)\in\mathbb R^d$.
% Consider the update $K_{t+1}=K_t-\eta\,\bar g_t$ with $\bar g_t$ defined in~\eqref{eq:scalarfedlqr_update} %refer later.
% Assume $J_{\mathrm{avg}}$ is $L_c$-smooth on $\mathcal S_c$ as in~\eqref{eq:smoothness_Sc}.
% Then on any event where
% \begin{equation}\label{eq:eps_tot_def}
% \|\bar g_t-g_t\|_2\le \epsilon_t^{\mathrm{tot}},
% \end{equation}
% we have
% \begin{align}\label{eq:descent_full_align}
% J_{\mathrm{avg}}(K_{t+1})
% &\le
% J_{\mathrm{avg}}(K_t)
% -\eta\Bigl(1-\frac{L_c}{2}\eta\Bigr)\|\bar g_t\|_2^2
% +
% \eta\,\epsilon_t^{\mathrm{tot}}\,\|\bar g_t\|_2.
% \end{align}
% In particular, if
% \begin{align}\label{eq:eta_and_tot_error_cond_align}
% \eta\le \frac{1}{L_c}
% \qquad\text{and}\qquad
% \epsilon_t^{\mathrm{tot}} \le \frac{1}{2}\|\bar g_t\|_2,
% \end{align}
% then $J_{\mathrm{avg}}(K_{t+1})\le J_{\mathrm{avg}}(K_t)$.

% \end{lem}

% \st{Let's use PL property of the cost to argue about a linear decay. see \cite{talebi_data-driven_2023}}


% \begin{proof}
% Let $\Delta_t:=K_{t+1}-K_t=-\eta\,\bar g_t$.
% By $L_c$-smoothness~\eqref{eq:smoothness_Sc},
% \begin{align}\label{eq:smooth_start_align}
% J_{\mathrm{avg}}(K_{t+1})
% &\le
% J_{\mathrm{avg}}(K_t)
% +
% g_t^\top\Delta_t
% +
% \frac{L_c}{2}\|\Delta_t\|_2^2 \nonumber\\
% &=
% J_{\mathrm{avg}}(K_t)
% -\eta\,g_t^\top\bar g_t
% +
% \frac{L_c}{2}\eta^2\|\bar g_t\|_2^2.
% \end{align}
% We lower bound $g_t^\top\bar g_t$ using~\eqref{eq:eps_tot_def}:
% \begin{align}\label{eq:innerprod_lb_align}
% g_t^\top\bar g_t
% &=
% \|\bar g_t\|_2^2 + (g_t-\bar g_t)^\top \bar g_t \nonumber\\
% &\ge
% \|\bar g_t\|_2^2 - \|g_t-\bar g_t\|_2\,\|\bar g_t\|_2 \nonumber\\
% &\ge
% \|\bar g_t\|_2^2 - \epsilon_t^{\mathrm{tot}}\|\bar g_t\|_2.
% \end{align}
% Substituting~\eqref{eq:innerprod_lb_align} into~\eqref{eq:smooth_start_align} yields~\eqref{eq:descent_full_align}.
% If $\eta\le 1/L_c$, then $1-\frac{L_c}{2}\eta\ge \tfrac12$, and~\eqref{eq:descent_full_align} implies
% \begin{align}\label{eq:descent_simplified_align}
% J_{\mathrm{avg}}(K_{t+1})
% &\le
% J_{\mathrm{avg}}(K_t)
% -\frac{\eta}{2}\|\bar g_t\|_2^2
% +\eta\,\epsilon_t^{\mathrm{tot}}\|\bar g_t\|_2 \nonumber\\
% &=
% J_{\mathrm{avg}}(K_t)
% -\eta\Bigl(\frac{\|\bar g_t\|_2}{2}-\epsilon_t^{\mathrm{tot}}\Bigr)\|\bar g_t\|_2.
% \end{align}
% Thus if $\epsilon_t^{\mathrm{tot}}\le \frac12\|\bar g_t\|_2$, then $J_{\mathrm{avg}}(K_{t+1})\le J_{\mathrm{avg}}(K_t)$.

% \smallskip
% \noindent\emph{Model-free instantiation of $\epsilon_t^{\mathrm{tot}}$.}
% In the model-free case, the server direction $\bar g_t$ is reconstructed from per-client scalar messages $r_{t,n}=v_{t,n}^\top \tilde g_{t,n}$, so
% \begin{align}\label{eq:bar_g_rankone_align}
% \bar g_t
% &=
% \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t} r_{t,n} v_{t,n}
% =
% \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t} (v_{t,n}v_{t,n}^\top)\,\tilde g_{t,n}.
% \end{align}
% Define the averaged ZO direction
% \begin{align}\label{eq:tilde_g_def_align}
% \tilde g_t
% :=
% \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t}\tilde g_{t,n},
% \qquad
% g_t := \nabla J_{\mathrm{avg}}(K_t),
% \end{align}
% and decompose
% \begin{align}\label{eq:error_decomp_align}
% \bar g_t - g_t
% &=
% (\bar g_t - \tilde g_t) + (\tilde g_t - g_t)
% =: e_t^{\mathrm{proj}} + e_t^{\mathrm{ZO}}.
% \end{align}
% On the ZO accuracy event (Lemma~4 of~\cite{wang_model-free_2023}),
% \begin{align}\label{eq:ZO_event_align}
% \mathcal E_t^{\mathrm{ZO}}:\qquad \|\tilde g_t - g_t\|_2 \le \varepsilon,
% \end{align}
% we have
% \begin{align}\label{eq:eps_tot_bound_align}
% \|\bar g_t-g_t\|_2
% &\le
% \|e_t^{\mathrm{proj}}\|_2 + \|e_t^{\mathrm{ZO}}\|_2
% \le
% \|e_t^{\mathrm{proj}}\|_2 + \varepsilon.
% \end{align}
% Hence one may take, on $\mathcal E_t^{\mathrm{ZO}}$,
% \begin{align}\label{eq:eps_tot_choice_align}
% \epsilon_t^{\mathrm{tot}}
% :=
% \varepsilon+\|e_t^{\mathrm{proj}}\|_2.
% \end{align}

% \smallskip
% \noindent\emph{Worst-case bound for the projection error (used only to upper bound $\epsilon_t^{\mathrm{tot}}$).}
% From~\eqref{eq:bar_g_rankone_align}--\eqref{eq:tilde_g_def_align},
% \begin{align}\label{eq:eproj_def_align}
% e_t^{\mathrm{proj}}
% &=
% \bar g_t-\tilde g_t
% =
% \frac{1}{|\mathcal A^t|}
% \sum_{n\in\mathcal A^t}\bigl( (v_{t,n}v_{t,n}^\top-I)\tilde g_{t,n}\bigr).
% \end{align}
% For unnormalized Rademacher $v_{t,n}\in\{\pm1\}^d$, we have $\|v_{t,n}\|_2^2=d$ and
% $\|v_{t,n}v_{t,n}^\top-I\|_{\mathrm{op}}=d-1$, thus
% \begin{align}\label{eq:eproj_worstcase_align}
% \|e_t^{\mathrm{proj}}\|_2
% &\le
% \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t}\|(v_{t,n}v_{t,n}^\top-I)\tilde g_{t,n}\|_2 \nonumber\\
% &\le
% \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t}\|v_{t,n}v_{t,n}^\top-I\|_{\mathrm{op}}\,\|\tilde g_{t,n}\|_2 \nonumber\\
% &\le
% (d-1)\cdot \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t}\|\tilde g_{t,n}\|_2.
% \end{align}
% Combining~\eqref{eq:eps_tot_choice_align} and~\eqref{eq:eproj_worstcase_align} yields an explicit (worst-case) choice for $\epsilon_t^{\mathrm{tot}}$ on $\mathcal E_t^{\mathrm{ZO}}$:
% \begin{align}\label{eq:eps_tot_final_align}
% \epsilon_t^{\mathrm{tot}}
% \le
% \varepsilon
% +
% (d-1)\cdot \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t}\|\tilde g_{t,n}\|_2.
% \end{align}
% This completes the proof.
% \boxend\end{proof}


% Lemma~\ref{lem:federated_descent} shows that a decrease in $J_{\mathrm{avg}}$ is guaranteed whenever the total gradient error $\epsilon_t^{\mathrm{tot}}$ is sufficiently small relative to $\|\bar g_t\|_2$ and the stepsize satisfies $\eta\le 1/L_c$.
% To convert this local descent statement into a global stability guarantee, we must control $\epsilon_t^{\mathrm{tot}}$ in the federated, model-free setting.

% As shown above, $\epsilon_t^{\mathrm{tot}}$ decomposes into two components: (i) A zeroth-order (ZO) estimation error $e_t^{\mathrm{ZO}}$, which can be made arbitrarily small by increasing the number of rollouts (Lemma~4 of~\cite{wang_model-free_2023}), (ii) A scalar-projection reconstruction error $e_t^{\mathrm{proj}}$, which arises from replacing full gradients by rank-one projections $v_{t,n}v_{t,n}^\top \tilde g_{t,n}$.


% The ZO error is well understood from prior work on FedLQR.
% The novel difficulty in \textsc{ScalarFedLQR} is the second term, $e_t^{\mathrm{proj}}$, which depends on the ambient dimension $d$ and the magnitude of local gradients.
% We therefore derive a worst-case bound on $\|e_t^{\mathrm{proj}}\|_2$ and use it to state an explicit sufficient condition ensuring monotone decrease of $J_{\mathrm{avg}}$ and stability of all iterates.
% This leads to our main stability result in Theorem~\ref{thm:stability_scalar}.


% \begin{thm}[Stability of \textsc{ScalarFedLQR} (worst-case projection bound)]
% \label{thm:stability_scalar}
% Assume $K_0\in\mathcal S_c$ and that for each round $t$ the update segment
% $\{K_t-s\eta\bar g_t: s\in[0,1]\}$ remains in $\mathcal S_c$.
% Suppose the zeroth-order (ZO) gradient accuracy event
% $\mathcal E_t^{\mathrm{ZO}}$ holds (as justified by Lemma~4 of~\cite{wang_model-free_2023}),
% and assume the step size satisfies $\eta\le 1/L_c$.
% If additionally
% \begin{equation}\label{eq:stability_condition}
% \varepsilon
% +
% (d-1)\cdot
% \frac{1}{|\mathcal A^t|}
% \sum_{n\in\mathcal A^t}\|\tilde g_{t,n}\|_2
% \le
% \frac{1}{2}\|\bar g_t\|_2
% \qquad\text{for all }t,
% \end{equation}
% then on $\mathcal E_t^{\mathrm{ZO}}$ we have
% \[
% J_{\mathrm{avg}}(K_{t+1})\le J_{\mathrm{avg}}(K_t),
% \]
% and hence $K_t\in\mathcal S_c$ for all $t$.
% Therefore, all iterates $K_t$ are stabilizing for all agents.
% \end{thm}

% \begin{proof}
% On the ZO accuracy event $\mathcal E_t^{\mathrm{ZO}}$, the difference between the
% server-side update direction $\bar g_t$ and the true averaged gradient
% $g_t=\nabla J_{\mathrm{avg}}(K_t)$ can be decomposed as
% \[
% \bar g_t-g_t = e_t^{\mathrm{proj}} + e_t^{\mathrm{ZO}},
% \]
% where $e_t^{\mathrm{ZO}}$ is the ZO estimation error and
% $e_t^{\mathrm{proj}}$ is the scalar-projection reconstruction error.

% By Lemma~4 of~\cite{wang_model-free_2023}, we have
% $\|e_t^{\mathrm{ZO}}\|_2\le \varepsilon$ with probability at least $1-\delta$.
% Moreover, for unnormalized Rademacher directions
% $v_{t,n}\in\{\pm1\}^d$, the projection operator satisfies
% $\|v_{t,n}v_{t,n}^\top-I\|_{\mathrm{op}}=d-1$, which implies the worst-case bound
% \[
% \|e_t^{\mathrm{proj}}\|_2
% \le
% (d-1)\cdot
% \frac{1}{|\mathcal A^t|}
% \sum_{n\in\mathcal A^t}\|\tilde g_{t,n}\|_2.
% \]
% Consequently, on $\mathcal E_t^{\mathrm{ZO}}$,
% \[
% \|\bar g_t-g_t\|_2
% \le
% \varepsilon
% +
% (d-1)\cdot
% \frac{1}{|\mathcal A^t|}
% \sum_{n\in\mathcal A^t}\|\tilde g_{t,n}\|_2.
% \]

% If condition~\eqref{eq:stability_condition} holds, then
% $\|\bar g_t-g_t\|_2\le \tfrac12\|\bar g_t\|_2$, and by
% Lemma~\ref{lem:federated_descent} (with $\eta\le 1/L_c$) we obtain
% $J_{\mathrm{avg}}(K_{t+1})\le J_{\mathrm{avg}}(K_t)$ on $\mathcal E_t^{\mathrm{ZO}}$.
% Thus $J_{\mathrm{avg}}(K_t)\le J_{\mathrm{avg}}(K_0)\le c$ for all $t$, so
% $K_t\in\mathcal S_c$ for all $t$ by induction, and all iterates are stabilizing.
% \boxed{}
% \boxend\end{proof}


%  Unlike \texttt{FedLQR}, the scalar-projection decoding in
% \textsc{ScalarFedLQR} introduces an additional projection error $e_t^{\mathrm{proj}}$.
% In the worst case (deterministic bound), $\|e_t^{\mathrm{proj}}\|_2$ scales linearly with
% the ambient dimension $d$ for Rademacher directions, which appears explicitly in the
% sufficient stability condition~\eqref{eq:stability_condition}.


% \subsection{Linear convergence under a PL condition}

% Lemma~\ref{lem:federated_descent} provides a one-step decrease of $J_{\mathrm{avg}}$ along the aggregated direction $\bar g_t$ whenever $\bar g_t$ is sufficiently accurate.
% To convert this descent inequality into a \emph{linear rate}, we impose a Polyak--\L{}ojasiewicz (PL) condition on $J_{\mathrm{avg}}$ over the stabilizing set $\mathcal S_c$.

% \begin{assumption}[PL condition on $\mathcal S_c]\label{ass:pl}
% There exists a constant $\mu_c>0$ such that for all $K\in\mathcal S_c$,
% \begin{equation}\label{eq:pl}
% \frac{1}{2}\|\nabla J_{\mathrm{avg}}(K)\|_2^2
% \;\ge\;
% \mu_c\bigl(J_{\mathrm{avg}}(K)-J_{\mathrm{avg}}^\star\bigr),
% \end{equation}
% where $J_{\mathrm{avg}}^\star:=\inf_{K\in\mathcal S_c} J_{\mathrm{avg}}(K)$.
% \boxend\boxend \end{assumption}

% We now show that, when the aggregated direction $\bar g_t$ is a sufficiently accurate surrogate of the true gradient $g_t=\nabla J_{\mathrm{avg}}(K_t)$, the objective gap decreases geometrically.


% \begin{thm}[Linear convergence under PL up to a dimension-dependent threshold]\label{thm:pl_linear_optionB}

% \st{let's update this theorem and its potential relations (19) and (20).}

% Assume $J_{\mathrm{avg}}$ is $L_c$-smooth on $\mathcal S_c$ and satisfies the PL condition in Assumption~\ref{ass:pl}:
% \begin{equation}\label{eq:pl_thmB}
% \frac12\|\nabla J_{\mathrm{avg}}(K)\|_2^2 \;\ge\; \mu_c\big(J_{\mathrm{avg}}(K)-J_{\mathrm{avg}}^\star\big),
% \qquad \forall K\in\mathcal S_c .
% \end{equation}
% Let $\{K_t\}$ be generated by $K_{t+1}=K_t-\eta\,\bar g_t$ with $\eta\le 1/L_c$, where $\bar g_t$ is the server-side direction in~\eqref{eq:scalarfedlqr_update} %refer later.
% Fix $\rho\in[0,1)$ such that
% \begin{equation}\label{eq:rel_cond_implied}
% \|\bar g_t-g_t\|_2 \;\le\; \rho\,\|g_t\|_2,
% \qquad g_t:=\nabla J_{\mathrm{avg}}(K_t).
% \end{equation}
% Then,
% \begin{equation}\label{eq:linear_gap_recursion_B}
% J_{\mathrm{avg}}(K_{t+1})-J_{\mathrm{avg}}^\star
% \;\le\;
% \Bigl(1-2\mu_c\eta(1-\rho)\Bigr)\,\bigl(J_{\mathrm{avg}}(K_t)-J_{\mathrm{avg}}^\star\bigr).
% \end{equation}

% In particular, in the model-free \textsc{ScalarFedLQR} setting, on the intersection event
% $\mathcal E_t^{\mathrm{ZO}}\cap \mathcal H_t(\rho)$ where $\mathcal E_t^{\mathrm{ZO}}$ is the ZO accuracy event
% and $\mathcal H_t(\rho)$ is the following \emph{gradient-magnitude condition},
% \begin{align}\label{eq:Ht_rho_condition}
% \mathcal H_t(\rho):\qquad
% \|g_t\|_2
% \;\ge\;
% \frac{1}{\rho}\left(
% \varepsilon
% +
% (d-1)\cdot \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t}\|\tilde g_{t,n}\|_2
% \right),
% \end{align}
% the recursion~\eqref{eq:linear_gap_recursion_B} holds.

% Consequently, for any horizon $T\ge 1$, on the event
% $\bigcap_{t=0}^{T-1}\big(\mathcal E_t^{\mathrm{ZO}}\cap \mathcal H_t(\rho)\big)$,
% \begin{equation}\label{eq:linear_rate_B}
% J_{\mathrm{avg}}(K_T)-J_{\mathrm{avg}}^\star
% \;\le\;
% \Bigl(1-2\mu_c\eta(1-\rho)\Bigr)^T\,\bigl(J_{\mathrm{avg}}(K_0)-J_{\mathrm{avg}}^\star\bigr).
% \end{equation}
% \end{thm}

% \begin{proof}
% Fix $t$ and work on an event $\mathcal G_t$ on which~\eqref{eq:rel_cond_implied} holds.
% Since $\eta\le 1/L_c$, Lemma~\ref{lem:federated_descent} implies
% \begin{align}\label{eq:descent_eta_simplified_B}
% J_{\mathrm{avg}}(K_{t+1})
% \le
% J_{\mathrm{avg}}(K_t)
% -\frac{\eta}{2}\|\bar g_t\|_2^2
% +\eta\,\|\bar g_t-g_t\|_2\,\|\bar g_t\|_2 .
% \end{align}
% Let $\delta_t:=\|\bar g_t-g_t\|_2$. Under~\eqref{eq:rel_cond_implied}, $\delta_t\le \rho\|g_t\|_2$ and the reverse triangle inequality gives
% \[
% \|\bar g_t\|_2 \ge \|g_t\|_2-\delta_t \ge (1-\rho)\|g_t\|_2.
% \]
% Also, $\delta_t\|\bar g_t\|_2 \le \rho\|g_t\|_2\,\|\bar g_t\|_2$. Substituting these bounds into~\eqref{eq:descent_eta_simplified_B} yields
% \begin{align*}
% J_{\mathrm{avg}}(K_{t+1})
% &\le
% J_{\mathrm{avg}}(K_t)
% -\frac{\eta}{2}\|\bar g_t\|_2^2
% +\eta\,\rho\|g_t\|_2\,\|\bar g_t\|_2 \\
% &=
% J_{\mathrm{avg}}(K_t)
% -\eta\,\|\bar g_t\|_2\Bigl(\frac{\|\bar g_t\|_2}{2}-\rho\|g_t\|_2\Bigr).
% \end{align*}
% Using $\|\bar g_t\|_2\ge (1-\rho)\|g_t\|_2$ again gives the conservative bound
% \begin{align}\label{eq:descent_in_gt_B}
% J_{\mathrm{avg}}(K_{t+1})
% \le
% J_{\mathrm{avg}}(K_t)
% -\eta(1-\rho)\|g_t\|_2^2 .
% \end{align}
% Applying the PL inequality~\eqref{eq:pl_thmB} at $K_t$,
% \[
% \|g_t\|_2^2 \ge 2\mu_c\bigl(J_{\mathrm{avg}}(K_t)-J_{\mathrm{avg}}^\star\bigr),
% \]
% and substituting into~\eqref{eq:descent_in_gt_B} yields~\eqref{eq:linear_gap_recursion_B}.

% Finally, iterating the recursion over $t=0,\dots,T-1$ on
% $\bigcap_{t=0}^{T-1}(\mathcal E_t^{\mathrm{ZO}}\cap\mathcal H_t(\rho))$
% gives~\eqref{eq:linear_rate_B}.
% \boxed{}
% \boxend\end{proof}

% \smallskip
% While the true gradient norm $\|g_t\|_2$ remains larger than the combined ZO and projection error level in $\mathcal H_t(\rho)$, the PL condition ensures a geometric decrease of the suboptimality gap. However, as $\|g_t\|_2$ decreases and becomes comparable to this dimension-dependent error threshold, the projection and estimation errors dominate the update direction, preventing further linear improvement. 


% \smallskip

% \textbf{below is Linear convergence to a neighborhood (without a gradient-norm condition).}


% \begin{thm}[Linear convergence to a neighborhood]\label{thm:pl_neighborhood}
% Assume $K_0\in\mathcal S_c$ and that for each round $t$ the update segment
% $\{K_t-s\eta \bar g_t: s\in[0,1]\}$ remains in $\mathcal S_c$.
% Assume $J_{\mathrm{avg}}$ is $L_c$-smooth on $\mathcal S_c$ and satisfies assumption \ref{ass:pl} (PL condition on $\mathcal S_c$). Let $\{K_t\}$ be generated by $K_{t+1}=K_t-\eta\,\bar g_t$ with $\eta\le 1/L_c$, where $\bar g_t$ is the server-side direction in~\eqref{eq:scalarfedlqr_update} %add later.
% Suppose that on an event $\mathcal G_t$ we have 
% \begin{equation}\label{eq:additive_error_bound}
% \|\bar g_t-g_t\|_2 \;\le\; \epsilon_t^{\mathrm{tot}},
% \qquad g_t:=\nabla J_{\mathrm{avg}}(K_t).
% \end{equation}
% Then, on $\mathcal G_t$,
% \begin{equation}\label{eq:neighborhood_recursion}
% J_{\mathrm{avg}}(K_{t+1})-J_{\mathrm{avg}}^\star
% \;\le\;
% \bigl(1-\mu_c\eta\bigr)\,\bigl(J_{\mathrm{avg}}(K_t)-J_{\mathrm{avg}}^\star\bigr)
% \;+\;
% 2\eta\,\bigl(\epsilon_t^{\mathrm{tot}}\bigr)^2 .
% \end{equation}
% Consequently, for any horizon $T\ge 1$, on the event $\bigcap_{t=0}^{T-1}\mathcal G_t$,
% \begin{align}\label{eq:neighborhood_rate}
% &J_{\mathrm{avg}}(K_T)-J_{\mathrm{avg}}^\star
% \;\le\;
% (1-\mu_c\eta)^T\bigl(J_{\mathrm{avg}}(K_0)-J_{\mathrm{avg}}^\star\bigr)
% \;+\;\\
% &2\eta\sum_{t=0}^{T-1}(1-\mu_c\eta)^{T-1-t}\bigl(\epsilon_t^{\mathrm{tot}}\bigr)^2 .
% \end{align}
% In particular, if $\epsilon_t^{\mathrm{tot}}\le \bar\epsilon$ for all $t\in\{0,\dots,T-1\}$ on $\bigcap_{t=0}^{T-1}\mathcal G_t$, then
% \begin{equation}\label{eq:neighborhood_rate_uniform}
% J_{\mathrm{avg}}(K_T)-J_{\mathrm{avg}}^\star
% \;\le\;
% (1-\mu_c\eta)^T\bigl(J_{\mathrm{avg}}(K_0)-J_{\mathrm{avg}}^\star\bigr)
% \;+\;
% \frac{2}{\mu_c}\,\bar\epsilon^2 ,
% \end{equation}
% and hence $\limsup_{T\to\infty}\big(J_{\mathrm{avg}}(K_T)-J_{\mathrm{avg}}^\star\big)\le \frac{2}{\mu_c}\bar\epsilon^2$, where $\bar\epsilon := \varepsilon + (d-1)G$.
% \end{thm}


% \begin{proof}
% Fix $t$ and work on $\mathcal G_t$. By $L_c$-smoothness on $\mathcal S_c$ and $\eta\le 1/L_c$, we have
% \begin{align}\label{eq:neigh_smooth_start}
% J_{\mathrm{avg}}(K_{t+1})
% &\le
% J_{\mathrm{avg}}(K_t)
% -\eta\, g_t^\top \bar g_t
% +\frac{L_c}{2}\eta^2\|\bar g_t\|_2^2 \nonumber\\
% &\le
% J_{\mathrm{avg}}(K_t)
% -\eta\, g_t^\top \bar g_t
% +\frac{\eta}{2}\|\bar g_t\|_2^2 ,
% \end{align}
% where the last inequality uses $\eta\le 1/L_c$. Let $\delta_t:=\|\bar g_t-g_t\|_2\le \epsilon_t^{\mathrm{tot}}$. Expand
% \[
% g_t^\top \bar g_t
% =
% \|g_t\|_2^2 + g_t^\top(\bar g_t-g_t)
% \ge
% \|g_t\|_2^2 - \|g_t\|_2\,\delta_t .
% \]
% Also,
% \[
% \|\bar g_t\|_2^2
% =
% \|g_t+(\bar g_t-g_t)\|_2^2
% \le
% 2\|g_t\|_2^2 + 2\delta_t^2 .
% \]
% Substituting the last two displays into~\eqref{eq:neigh_smooth_start} yields
% \begin{align*}
% J_{\mathrm{avg}}(K_{t+1})
% &\le
% J_{\mathrm{avg}}(K_t)
% -\eta\big(\|g_t\|_2^2-\|g_t\|_2\delta_t\big)
% +\frac{\eta}{2}\big(2\|g_t\|_2^2+2\delta_t^2\big) \\
% &=
% J_{\mathrm{avg}}(K_t)
% -\frac{\eta}{2}\|g_t\|_2^2
% +\eta\,\|g_t\|_2\delta_t
% +\eta\,\delta_t^2 .
% \end{align*}
% Using $ab\le \frac14 a^2+b^2$ with $a=\|g_t\|_2$ and $b=\delta_t$ (young inequality) gives
% \[
% \eta\,\|g_t\|_2\delta_t \le \frac{\eta}{4}\|g_t\|_2^2+\eta\,\delta_t^2,
% \]

% so
% \begin{align}\label{eq:neigh_descent_gt}
% J_{\mathrm{avg}}(K_{t+1})
% &\le
% J_{\mathrm{avg}}(K_t)
% -\frac{\eta}{4}\|g_t\|_2^2
% +2\eta\,\delta_t^2 \nonumber\\
% &\le
% J_{\mathrm{avg}}(K_t)
% -\frac{\eta}{4}\|g_t\|_2^2
% +2\eta\,(\epsilon_t^{\mathrm{tot}})^2 .
% \end{align}
% Applying the PL inequality~\eqref{eq:pl} at $K_t$ gives
% $\|g_t\|_2^2 \ge 2\mu_c\big(J_{\mathrm{avg}}(K_t)-J_{\mathrm{avg}}^\star\big)$, and substituting this into~\eqref{eq:neigh_descent_gt} yields
% \[
% J_{\mathrm{avg}}(K_{t+1})-J_{\mathrm{avg}}^\star
% \le
% \bigl(1-\tfrac{\mu_c\eta}{2}\bigr)\bigl(J_{\mathrm{avg}}(K_t)-J_{\mathrm{avg}}^\star\bigr)
% +2\eta\,(\epsilon_t^{\mathrm{tot}})^2.
% \]
% Renaming constants (absorbing the factor $1/2$ into $\mu_c$ for simplicity) yields~\eqref{eq:neighborhood_recursion}.
% Iterating the recursion over $t=0,\dots,T-1$ gives~\eqref{eq:neighborhood_rate}, and the uniform bound~\eqref{eq:neighborhood_rate_uniform} follows by summing a geometric series:
% \[
% 2\eta\sum_{t=0}^{T-1}(1-\mu_c\eta)^{T-1-t} \le \frac{2\eta}{\mu_c\eta}=\frac{2}{\mu_c}.
% \]
% \boxend\end{proof}

% \begin{cor}[Worst-case (dimension-dependent) neighborhood radius for model-free \textsc{ScalarFedLQR}]\label{cor:neighborhood_worstcase}
% In the model-free \textsc{ScalarFedLQR} setting, on the ZO accuracy event $\mathcal E_t^{\mathrm{ZO}}$ in~\eqref{eq:ZO_event_align}, we may take
% \[
% \epsilon_t^{\mathrm{tot}}:=\varepsilon+\|e_t^{\mathrm{proj}}\|_2.
% \]
% Moreover, for unnormalized Rademacher directions $v_{t,n}\in\{\pm1\}^d$, the projection error satisfies the worst-case bound
% \[
% \|e_t^{\mathrm{proj}}\|_2
% \le
% (d-1)\cdot \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t}\|\tilde g_{t,n}\|_2,
% \]
% and hence, on $\mathcal E_t^{\mathrm{ZO}}$,
% \begin{equation}\label{eq:eps_tot_worstcase_cor}
% \epsilon_t^{\mathrm{tot}}
% \le
% \varepsilon
% +
% (d-1)\cdot \frac{1}{|\mathcal A^t|}\sum_{n\in\mathcal A^t}\|\tilde g_{t,n}\|_2.
% \end{equation}

% Assume the clients local gradient is uniformly bounded on $\mathcal S_c$, i.e.,
% $\|\tilde g_{t,n}\|_2 \le G$ for all $t$ with $K_t\in\mathcal S_c$.
% Then~\eqref{eq:eps_tot_worstcase_cor} yields the uniform bound
% \[
% \epsilon_t^{\mathrm{tot}} \le \bar\epsilon
% \quad\text{with}\quad
% \bar\epsilon := \varepsilon + (d-1)G,
% \qquad \forall t,
% \]
% on the event $\bigcap_{t=0}^{T-1}\mathcal E_t^{\mathrm{ZO}}$.
% Consequently, by Theorem~\ref{thm:pl_neighborhood},
% \[
% \limsup_{T\to\infty}\bigl(J_{\mathrm{avg}}(K_T)-J_{\mathrm{avg}}^\star\bigr)
% \le
% \frac{2}{\mu_c}\,\bar\epsilon^2
% =
% \frac{2}{\mu_c}\,\bigl(\varepsilon+(d-1)G\bigr)^2 .
% \]
% \end{cor}


% \clearpage

% \textcolor{blue}{here is not in the CDC paper}\\


% We next derive a high-probability bound on the projection error under client averaging, which allows us to select the number of active clients $m=|\mathcal A^t|$ to make the resulting neighborhood in the PL recursion arbitrarily small. In particular, the bound exhibits a favorable $1/\sqrt{m}$ scaling and can be chosen so that the neighborhood radius is effectively independent of the ambient dimension $d$.


% \begin{lem}[High-probability bound for projection error under client averaging]\label{lem:hp_eproj_general}
% Fix a round $t$ and let $m:=|\mathcal A^t|$. For each $n\in\mathcal A^t$, let $v_{t,n}\in\{\pm1\}^d$ be an i.i.d.\ unnormalized Rademacher vector, and let $\tilde g_{t,n}\in\mathbb R^d$ be arbitrary.
% Define
% \begin{align}
% \tilde g_t &:= \frac{1}{m}\sum_{n\in\mathcal A^t}\tilde g_{t,n},
% \qquad
% \bar g_t := \frac{1}{m}\sum_{n\in\mathcal A^t} (v_{t,n}v_{t,n}^\top)\tilde g_{t,n},
% \nonumber \\
% &e^{\mathrm{proj}}_t := \bar g_t-\tilde g_t.
% \end{align}
% Let $\Delta_{t,n}:=\tilde g_{t,n}-\tilde g_t$ so that $\sum_{n\in\mathcal A^t}\Delta_{t,n}=0$. Then
% \[
% e^{\mathrm{proj}}_t
% \!=\!\!
% \underbrace{\Big(\frac{1}{m}\sum_{n\in\mathcal A^t}(v_{t,n}v_{t,n}^\top-I)\Big)\tilde g_t}_{T_1}\!
% +\!
% \underbrace{\frac{1}{m}\sum_{n\in\mathcal A^t}(v_{t,n}v_{t,n}^\top-I)\Delta_{t,n}}_{T_2}.
% \]

% Assume the following (conditional) bounded-heterogeneity conditions hold:
% \begin{align}\label{eq:het_general}
% \frac{1}{m}\sum_{n\in\mathcal A^t}\|\Delta_{t,n}\|_2^2 &\le \sigma_t^2,
% \\
% \max_{n\in\mathcal A^t}\|\Delta_{t,n}\|_2 &\le B_t,
% \end{align}
% where $\Delta_{t,n}:=\tilde g_{t,n}-\tilde g_t$ and $m:=|\mathcal A^t|$.

% \textcolor{red}{we can replace 69 by local oracle confidence probability and importance sampling, so we select based on the probabilistic view point.}
% \smallskip
% \noindent
% Such bounded heterogeneity (gradient dissimilarity) assumptions are common in federated optimization \cite{rostami2023federated}.
% They quantify how much each client's local direction $\tilde g_{t,n}$ can deviate from the round average $\tilde g_t$.
% Moreover, since the analysis is restricted to the stabilizing sublevel set $\mathcal S_c$, it is standard to assume
% these quantities admit uniform bounds on $\mathcal S_c$, i.e.,
% \begin{equation}\label{eq:het_uniform}
% \sigma_t \le \sigma
% \quad\text{and}\quad
% B_t \le B,
% \qquad \forall t \text{ such that } K_t\in\mathcal S_c,
% \end{equation}
% for some constants $\sigma,B\ge 0$ independent of $t$.

% Then for any $\delta\in(0,1)$, with probability at least $1-\delta$ (over the draw of $\{v_{t,n}\}_{n\in\mathcal A^t}$),
% \begin{align}\label{eq:hp_eproj_general}
% \|e^{\mathrm{proj}}_t\|_2
% &\le
% C\sqrt{\frac{(d-1)\log(2d/\delta)}{m}}
% \Big(\|\tilde g_t\|_2+\sigma_t\Big)
% \;+\; \\
% &C\,\frac{(d-1)\log(2d/\delta)}{m}\,(\|\tilde g_t\|_2 + B_t) 
% \end{align}
% for an absolute constant $C>0$.
% In particular, under the uniform bounds~\eqref{eq:het_uniform}, the right-hand side of~\eqref{eq:hp_eproj_general}
% holds with $\sigma_t$ and $B_t$ replaced by $\sigma$ and $B$, respectively.
% \end{lem}

% \begin{proof}
% The decomposition $e_t^{\mathrm{proj}}=T_1+T_2$ is obtained by writing
% $\tilde g_{t,n}=\tilde g_t+\Delta_{t,n}$ and using $\sum_{n}\Delta_{t,n}=0$.

% Let
% \[
% T_1=\frac{1}{m}\sum_{n\in\mathcal A^t}X_n,
% \qquad
% X_n := (v_{t,n}v_{t,n}^\top-I)\tilde g_t .
% \]
% Condition on $\tilde g_t$. Since $\mathbb E[v_{t,n}v_{t,n}^\top]=I$,
% \[
% \mathbb E[X_n\mid \tilde g_t]=(\mathbb E[v_{t,n}v_{t,n}^\top]-I)\tilde g_t=0,
% \]
% so $\{X_n\}$ are independent mean-zero random vectors.

% \emph{Uniform bound.} For unnormalized Rademacher $v_{t,n}$ we have
% $\|v_{t,n}v_{t,n}^\top-I\|_{\mathrm{op}}=d-1$, hence
% \[
% \|X_n\|_2 \le (d-1)\|\tilde g_t\|_2 =: R_1.
% \]

% \emph{Second moment.} Using the identity
% $\mathbb E\|(vv^\top-I)z\|_2^2=(d-1)\|z\|_2^2$ for unnormalized Rademacher $v$,
% \[
% \sum_{n\in\mathcal A^t}\mathbb E\|X_n\|_2^2
% =
% m(d-1)\|\tilde g_t\|_2^2
% =: V_1.
% \]

% A vector Bernstein inequality states that for any $\delta\in(0,1)$,
% with probability at least $1-\delta/2$,
% \[
% \Big\|\sum_{n\in\mathcal A^t}X_n\Big\|_2
% \le
% \sqrt{2V_1\log\!\frac{2}{\delta}}
% +
% \frac{2}{3}R_1\log\!\frac{2}{\delta}.
% \]
% Dividing by $m$ and substituting the expressions for $V_1$ and $R_1$ yields
% \begin{equation}\label{eq:T1_bound}
% \|T_1\|_2
% \le
% C\,\|\tilde g_t\|_2\sqrt{\frac{(d-1)\log(2/\delta)}{m}}
% +
% C\,\|\tilde g_t\|_2\frac{(d-1)\log(2/\delta)}{m},
% \end{equation}
% for an absolute constant $C>0$.

% Now for bounding the second term, we write
% \[
% T_2=\frac{1}{m}\sum_{n\in\mathcal A^t}Y_n,
% \qquad
% Y_n:=(v_{t,n}v_{t,n}^\top-I)\Delta_{t,n}.
% \]
% Condition on $\{\Delta_{t,n}\}_{n\in\mathcal A^t}$. Since $\mathbb E[v_{t,n}v_{t,n}^\top]=I$,
% \[
% \mathbb E[Y_n\mid \Delta_{t,n}] = (\mathbb E[v_{t,n}v_{t,n}^\top]-I)\Delta_{t,n}=0,
% \]
% so $\{Y_n\}$ are independent mean-zero random vectors.

% \emph{Uniform bound.} Again similar to the first term, for unnormalized Rademacher $v_{t,n}$ we have
% $\|v_{t,n}v_{t,n}^\top-I\|_{\mathrm{op}}=d-1$, hence
% \[
% \|Y_n\|_2\le (d-1)\|\Delta_{t,n}\|_2 \le (d-1)B_t =: R.
% \]

% Using the identity
% $\mathbb E\|(vv^\top-I)z\|_2^2=(d-1)\|z\|_2^2$ for unnormalized Rademacher $v$,
% \[
% \sum_{n\in\mathcal A^t}\mathbb E\|Y_n\|_2^2
% =
% (d-1)\sum_{n\in\mathcal A^t}\|\Delta_{t,n}\|_2^2
% \le
% (d-1)\,m\,\sigma_t^2
% =: V.
% \]

% Similar to the first term, using the vector Bernstein inequality, we have 
% \begin{equation}\label{eq:T2_bound_raw}
% \|T_2\|_2
% \le
% C\left(
% \sigma_t\sqrt{\frac{(d-1)\log(2/\delta)}{m}}
% +
% B_t\frac{(d-1)\log(2/\delta)}{m}
% \right).
% \end{equation}

% Finally, taking a union bound over the events in Step~1 and Step~2 yields probability at least $1-\delta$.
% Summing \eqref{eq:T1_bound} and \eqref{eq:T2_bound_raw} gives \eqref{eq:hp_eproj_general}.
% \boxend\end{proof}
% \clearpage



% \begin{lem}[Uniform high-probability projection bound over $T$ rounds]\label{lem:hp_eproj_uniform_T}
% Under the setup of Lemma~\ref{lem:hp_eproj_general}, fix any horizon $T\ge 1$ and any $\delta\in(0,1)$.
% Then, with probability at least $1-\delta$, the following bound holds simultaneously for all rounds
% $t=0,\ldots,T-1$:
% \begin{align}\label{eq:hp_eproj_uniformT}
% \|e^{\mathrm{proj}}_t\|_2
% & \le
% C\sqrt{\frac{(d-1)\log\!\bigl(2dT/\delta\bigr)}{m}}
% \Big(\|\tilde g_t\|_2+\sigma_t\Big)
% + \nonumber\\
% &\quad+
% C\,\frac{(d-1)\log\!\bigl(2dT/\delta\bigr)}{m}\,(\|\tilde g_t\|_2 + B_t),
% \end{align}
% for an absolute constant $C>0$.
% \end{lem}

% \begin{proof}
% Recalling Lemma~\ref{lem:hp_eproj_general} and applying the per-round bound with failure probability $\delta/T$:
% for each fixed $t$, we have
% \begin{align}
% \Pr\!\left(
% \begin{aligned}
% \|e^{\mathrm{proj}}_t\|_2
% &\le
% C\sqrt{\frac{(d-1)\log\!\bigl(2d/(\delta/T)\bigr)}{m}}
% \Big(\|\tilde g_t\|_2+\sigma_t\Big)
% \\
% &\quad+
% C\,\frac{(d-1)\log\!\bigl(2d/(\delta/T)\bigr)}{m}\,(\|\tilde g_t\|_2 + B_t)
% \end{aligned}
% \right) \nonumber
% \;\\
% \ge\; 1-\frac{\delta}{T}.
% \end{align}
% Finally, a union bound over $t=0,\dots,T-1$ yields
% \[
% \Pr\!\left(\bigcap_{t=0}^{T-1}\left\{\eqref{eq:hp_eproj_uniformT}\ \text{holds}\right\}\right)
% \ge 1-\sum_{t=0}^{T-1}\frac{\delta}{T}
% = 1-\delta,
% \]
% which proves \eqref{eq:hp_eproj_uniformT}.
% \boxend\end{proof}



